Enhancing Inductive Entailment Proofs in Separation Logic with Lemma Synthesis

This paper presents an approach to lemma synthesis to support advanced inductive entailment procedures based on separation logic. We first propose a mechanism where lemmas are automatically proven and systematically applied. The lemmas may include universal guard and/or unknown predicate. While the former is critical for expressivity, the latter is essential for supporting relationships between multiple predicates. We further introduce lemma synthesis to support (i) automated inductive reasoning together with frame inference and (ii) theorem exploration. For (i) we automatically discover and prove auxiliary lemmas during an inductive proof; and for (ii) we automatically generate a useful set of lemmas to relate user-defined or system-generated predicates. We have implemented our proposed approach into an existing verification system and tested its capability in inductive reasoning and theorem exploration. The experimental results show that the enhanced system can automatically synthesize useful lemmas to facilitate reasoning on a broad range of non-trivial inductive proofs.

==> abs-bk.tex <==
%% Lemmas have been widely used to enhance the capability of program verification systems.
%%  However, existing reasoning systems of heap-manipulating programs %% based on
%%  via separation logic
%%  rely on user to supply additional lemmas that
%% might be needed for a proof.
%% In this paper,
%% we present
This paper presents
an approach to lemma synthesis for automation and completeness
of inductive entailment procedures in separation logic.
We propose a
%% lemma mechanism (automated proving and application) %% and lemma synthesis
% with second-order bi-abduction.
mechanism where lemmas are automatically proven and  systematically applied.
%% Our mechanism supports lemmas
Our lemmas can include  {\em universal} guards %%  {\em universal} variables
and {\em unknown} predicates.
While the former is crucial for an expressive power,
the latter is essential to synthesize lemmas with
 newly-inferred predicates.
%% This mechanism takes a
%% conjecture
%% with unknown
%% predicates as input
%% and deploys second-order bi-abductive entailment procedure to prove its soundness
%% and
%% infer definitions of these {\em unknown} predicates,
%% simultaneously.
%% In turn, the proven lemma with synthesized predicates
%% can be automatically applied during program verification.
We further introduce
 lemma synthesis to support
(i)  automated inductive reasoning and (ii) theorem exploration.
%% lemma synthesis to support (i) automated inductive reasoning
%% and (ii) theorem exploration.
Concretely, for (i) we automatically discover and prove
auxiliary lemmas during an inductive proof;
for (ii)  we automatically
 generate a useful set of lemmas to relate %% existing
 user-defined predicates. %% as well as
%% where the auxiliary
%% lemmas can be proven automatically before used. %% using our lemma mechanism.
%% for (ii) we automatically generate a useful set of lemmas to relate %% existing
%% user-defined predicates.
 %% or relate an existing predicate with multiple synthesized predicates to
 %% explicate hiding separation (non-aliasing) pointers.
We have implemented our proposed approach %% lemma synthesis
into an automated verification system
and tested its capability in
inductive reasoning and theorem exploration. %%predicate transformation.
%% detect must-separating
%% pointers of user-defined predicates.
The experimental results show that the enhanced
system can automatically synthesize useful lemmas to facilitate reasoning on
 a new class of sophisticated inductive proofs.
%% the completeness and automation of the verification system.


==> abs-old.tex <==


We present an entailment procedure for 
separation logic with emphasis on user-defined shape predicates.
Our decision procedure supports both valid and invalid proving.
Especially, our entailment procedure supports segmentation folding on the predicates
 and frame inference for modular reasoning.
To enhance the completeness,
our proposal also supports a lemma mechanism as alternative
unfolding on inductive predicates during proof search.
The benefit of the lemma mechanism is twofold. First,
it helps to explore alternative searches beyond definitions of shape predicates.
Second, it supports induction proving while lemma definition works as induction
hypothesis and lemma application makes use of the induction
hypothesis to prove the entailment.
We have implemented the proposal into a tool called {\toolname}
and evaluated the tool on a set of entailment problems and
verification on heap-manipulating programs. The experimental results show
that {\toolname} can solve 96.74\% of the entailment problems
and can discharge all generated entailments effectively and efficiently
during verifying the programs.

\hide{
invariant as exact representative of user-defined predicate
and a reduction of a Separation Logic fragment to a 
 a decidable first-order theory fragment.
Second, we show how to employ this reduction to automatically
 check entailment and satisfiability for separation logic.
Especially, our entailment procedure supports segmentation folding on the predicates
 and frame inference for modular reasoning.
Second, as first-other formulas with exact invariant may consist of disjuncts which exponentially increase the proof search,
we propose sound and complete procedures with approximate mechanisms:
 (1) {\em necessary} invariants - over-approximation with less disjuncts -
  to prove unsatisfiability;
(2) context-sensitive and top-down {\em sufficient} analysis to search a models to prove satisfiability.
Last, we propose a modular and bottom-up analysis to compute those exact and necessary invariants.

UNSAT proving: over-approximate invariant to compute {\em necessary} abstraction.

SAT proving: under-approximation to compute {\em sufficient} abstraction.

\noindent{\bf What? define key words}

\noindent{\bf Significance, Application}

First, 

\noindent{\bf Implementation and Evaluation}

 \begin{verbatim}
  - decision procedure
  - invalid proving with satisfiability
  - 
 \end{verbatim}}


==> conclude-old.tex <==
\noindent{\bf Conclusion.} We have presented a entailment
procedure for an undecidable fragment
of separation logic.
Based on the exact heap
representative, the procedure
can prove both validity and invalidity.
As designed for a powerful decision procedure,
our procedure can support the highest generic level
of inductive shape predicates.
as well as be capable of inferring
residual frame, the heap part does not involve
in the entailment.
Moreover, we have described
a set of inference rules to efficiently
handle segment shape predicates.
We have proposed a new lemma mechanism
with rewrite rule for introduce the cut,
instead of entailment based rule.
We have also implemented a
prototype of our decision
procedure, and have
evaluated on sets of benchmarks
 with complex user-defined predicate usage patterns.
To bridge the gap
of the present solver,
we shall improve it towards synthesizing
on-the-fly and applying necessary lemmas on demand.


==> cover.tex <==
\thispagestyle{empty}

%\begin{titlepage}


\begin{center}

%\vspace{20cm}


 %% {\Large Automated Verification on Heap-Manipulating Programs with Specification Inference}
%% {\Large Automated Complete Specification Discovery with Shape Predicate Synthesis and Beyond}
%% {\Large Automated Verification of Complete Specifications on Heap-Manipulating Programs}
% {\Large Automated Verification of Complete Specification with Shape Inference}
 {\large AUTOMATED VERIFICATION OF \\COMPLETE SPECIFICATION WITH SHAPE INFERENCE}
%% {\Large Automated Verification on Heap-Manipulating Programs with Shape Synthesis}

\vspace{18mm}

%% \begin{center}
%% \includegraphics[width=5cm]{images/NUS_SOC_logo}
%% \end{center}


\vspace{43mm}

{\Large LE QUANG LOC} \\


%\vspace{0.6cm}
%\vspace{2cm}

\vspace{8.5cm}

{\Large 
NATIONAL UNIVERSITY OF SINGAPORE \\
\vspace{1cm} 2014 }

\end{center}

%\end{titlepage} 


==> entail-appr.tex <==
The procedures for entailment and satisfiablity checking in Sec. \ref{sec:ent.exact} is not very efficient at two points. invariant computation is slow to reach a least fixpoint;
invariant of heap predicate formulas consist of disjuncts;
 those  disjuncts increase exponentially when combined in ${\xpure}$.

Our proposal is a combination of underapproximate and overapproximate.

may not terminate.

We propose approximate mechanism: an over-approximation transformation for validity proving
and under-approximation analysis for invalidity proving. over-approximation for efficiency.

 for invalid proving, we propose a context-sensitive
under-approximate analysis to counter-model searching.

Entailment procedure with over-approximation is similar to
  entailment procedure in Sec. \ref{sec:ent.exact} except \form{\entrulen{{XPURE}}}.

Combination of must and may analysis??
\[
\!\frac{\begin{array}{c}\entrulen{\overline{XPURE}-UNSAT}\\
%% \rho{=}[0/\nil]\\
{\neg (\xpureo(\heap_1{\sep}\heap){\wedge}\pure_1) \wedge ({\exists} \myit{V}{\cdot}\pure_2)} \vdash_{pure} \false
\end{array}}
{\entailVVE{\heap_1{\wedge}\pure_1}{\pure_2}{(\heap_1{\wedge}\pure_1, \valid)}}%
\]


DPLL-Based Decision Procedure for Satisfiability??
\[
\!\frac{\begin{array}{c}\entrulen{\overline{XPURE}-SAT}\\
%% \rho{=}[0/\nil]\\
{ \xpureu(\heap_1{\sep}\heap{\wedge}\pure_1 \wedge \neg({\exists} \myit{V}{\cdot}\pure_2))} \vdash_{pure} \true
\end{array}}
{\entailVVE{\heap_1{\wedge}\pure_1}{\pure_2}{(\heap_1{\wedge}\pure_1, \invalid)}}%
\]

put $\neg$ rhs into \form{\xpureu} to drive the counter-model searching
\subsection{$\xpureo$ Reduction}

\subsection{Context-sensitive Analysis for Counter-Model}

DPLL-Based Decision Procedure for Satisfiability

Recursive predicates make the The challenging

The analysis takes a separation logic formula as input and
it can produces three types of results:
\begin{enumerate}
\item It may output "yes" together with a set of concrete models
\item It may output "no"
\item It may not terminate
\end{enumerate}

The analysis keeps track of a set of stack record $\ustack$, each record $\ustate$ is a tuple:
\[
 \ustate: \PName \sep \Val^n \sep \bag \sep \pure
\]



stack $\predstack$


\begin{verbatim}

==============================================
disjuncts

\alpha_1 = inv_u(svs, \alpha, f_1)
\alpha_2 = inv_u(svs, \alpha, f_2)
-------------------------------------------------
inv_u(svs, \alpha, f_1 \/ f_2) ---> \alpha_1 \meet \alpha_2

rearrange

r = inv_u(svs, alpha, h1 /\ rearrange (p, svs \cap fv(h1)) *  h2 /\ rearrange (p, svs \cap fv(h2)))
-----------------------
inv_u (svs, alpha, h1 * h2 /\ p) --> r


spatial conjunction

(B1, \eq_1, \num_1) = inv_u(svs \cap fv(f1), alpha, f1)
(B2, \eq_2, \num_2) = inv_u(svs \cap fv(f2), alpha, f_2)
--------------------------------------------------
inv_u(svs, alpha, f_1 * f_2) ---> (B1 \cup B2, \eq_1 /\ \eq_2, \num_1 /\ \num_2)


normalize
pure has zip x.next, x.val, x.next.next: fully unfold


formula - non-rec

\alpha_1 = extract(h_ptos, \pure)
\alpha_2 = norm(\alpha \meet \alpha_1)
\alpha_i = inv_u(svs, \alpha_2 \meet extract_eqs(h_v_i), h_v_i)
\alpha_3 = \MEET \alpha_i
--------------------------------------------------
inv_u(svs, (baga, \eq, \num), h_vs * h_ptos /\ \pure) ---> \alpha_3


--------------------------------------
formula - mutual-rec


\gamma: mut_rec_view_name * args --> alpha
\fix: \gamma_1 * \gamma_2 --> bool

\alpha_1 = extract(h_ptos, \pure)
\alpha_2 = norm(\alpha \meet \alpha_1)
\alpha_i = inv_u(svs, \alpha_2 \meet extract_eqs(h_v_i), h_v_i): h_v_i is not mut rec

\alpha_j = \gamma(h_v_i, h_v_i_args)


\alpha_3 = \MEET \alpha_i

\gamma1 = \add \gamma \alpha_3
--------------------------------------------------
\gamma: inv_u(svs, (baga, \eq, \num), h_vs * h_ptos /\ \pure) ---> \gamma1: \alpha_3

=================================================


\\check sat
  \alpha = inv-u(\top,lhs)      (reduce(\alpha) |- true).
 ----------------------
  (lhs) ---> SAT.

\check unsat
   \alpha = inv-o(lhs)   reduce(\alpha) |- false
 ----------------------
  (lhs) ---> UNSAT.


===============================

unfold
  f_i in definition of view
  r_i = f_i * lhs |- rhs
  r = LAND r_i
 ----------------------
  (x::view<...> * lhs |- rhs) --> r.

fold
  f_i in definition of view
  r_i =  lhs |- f_i * rhs
  r = SEARCH r_i
 ----------------------
  ( lhs |- x::view<...> * rhs) --> r.


seg-fold-1
  x::p<\vector{v_1}, y> * y ... z |- x::p<\vector{v_3},z> --> x::p<\vector{v_1}, y> *  y ... z |- x::p<\vector{v_4},y>*y::p<\vector{v_5},z>


seg-fold-2
  x::br-of-p * y ... z |- x::p<\vector{v_3},z> --> x::p<\vector{v_1}, y> *  y ... z |- x::p<\vector{v_4},y>*y::p<\vector{v_5},z>



invalid check

   inv-u(fv(rhs), \top,rhs) ==> true
   lsvl=fv(lhs)  lhs_u = inv-u(lsvl,\top,lhs)
   inv-u(lsvl, lhs_u, rhs) ==> false
 ----------------------
  (lhs |- rhs) --> INVALID.


valid check: \emp heap rhs

   inv-o(lhs) ==> rhs_pure
 ----------------------
  (lhs |- emp /\ rhs_pure) --> VALID.
 

\end{verbatim}


==> entail-cycle-pure.tex <==

\hide{ LHS |- RHS
cases:
 -Root matching: (two aux functions)
   1. lhs is an instance of predicate A
      rhs is an instance of predicate B
   2. lhs: node. rhs: predicate.
       fold lhs or lemma synthesis
   3. lhs: predicate . rhs: node.
       unfold lhs or lemma synthesis
 - arg matching (check_seg_split_pred)
   4.  lhs: predicate . rhs: node.
    LEFT ->
    (suppose to ignore this one)}


To support the new mechanism,
we enhance the entailment formalism as follows:
\[
\form{\entailLEM{\G_i}{\D_A}{\heap}{V}{\D_C}{((\D_R,\flow),\G_0})}
\]
with additional \form{\G_i} (\form{\G_o}) be input (output, respectively) sets of lemmas.

In this subsection we will implement the \form{ \synlemma{\G}{\D_{1}}{\pure_1}{\D_2}{\pure_2}{\bowtie}} function.
\btt{syn} checks whether the current entailment contains a sound cyclic proof.
\btt{syn} synthesized and proves lemma through three steps as follows:
\begin{enumerate}
\item Firstly, it synthesizes the lemma.
\[
\begin{array}[t]{c}
  \bar{v}_1 = \FV(\D_1) \qquad \bar{v}_2 = \FV(\D_2) \\
 \lem = \D_{1} \wedge \slice{ \bar{v}_1}{\pure_1} \bowtie \D_{2} \wedge  \slice{ \bar{v}_2}{\pure_2}
\end{array}
\]
Here, \form{\slice{\setvars{w}}{\pure}} is an auxiliary function that
existentially quantifies in {\pure} all free variables that are not in the set \form{\setvars{w}}. 
\item Secondly, it checks whether the new lemma exists, \form{\lookup{\G}{\lem} }.
If \form{\lem} is in \form{\G}, \btt{syn} fails with \form{\bot}.
%\item Last, it proves the lemma with initially performing an progress with unfold, if necessary.
\end{enumerate}


\input{entail-fig-cycle-pure}
 
Case 1: \form{\entrulen{2PRED}}

\form{\D_1 {=} \seppred{\code{P^0}}{r{,}\bar{w_1}}}

\form{\D_2 {=}  \seppred{\code{Q^{0}}}{r{,}\bar{w_2}}}
\[
\begin{array}[t]{c}
   \constr_1'{=} \unfold(\seppred{\code{P^0}}{r{,}\bar{w}_1}
    {\wedge} \slice{ r{::}\bar{w}_1}{\pure_1}{,}
             \code{\seppred{\code{P}}{r{,}\bar{w}_1}}) \\
{\entailLEM{(\G {\cup} \{\lem \})}{\constr_1'}{\heap}{V}
{{\D_2}{\wedge}\slice{ r{::}\bar{w}_2}{\pure_2}}{\textcolor{blue}{\emp}}{\flow}{\G_o}}
\end{array}
\]

Case 2: \form{\entrulen{LSYN-FOLD}}

\form{\D_1 {=} \sepnodeF{r}{c}{p{,}\setvars{w_1}} {\sep} \seppred{\code{P^1}}{p{,}\bar{w_3}}}

\form{\D_2 {=} \seppred{\code{Q^0}}{r{,}\bar{w}_2}}
\[
\begin{array}[t]{c}
   \constr_2'{=} \unfold(\seppred{\code{Q^0}}{r{,}\bar{w}_2}
    {\wedge} \slice{ r{::}\bar{w}_2}{\pure_2}{,}
             \code{\seppred{\code{Q^0}}{r{,}\bar{w}_2}}) \\
{\entailLEM{(\G {\cup} \{\lem \})}{\D_1 {\wedge} \slice{ [r;q]{@}\bar{w}_1@\bar{w}_3}{\pure_1}  }
{\heap}{V}
                {\constr_2'}{\textcolor{blue}{\emp}}{\flow}{\G_o}}
\end{array}
\]

Case 3: \form{\entrulen{LSYN-UNFOLD}}

\form{\D_1 {=} \seppred{\code{P^0}}{r{,}\bar{w_1}}}

\form{\D_2 {=} \seppred{\sepnodeF{r}{c}{p{,}\setvars{w_3}} {\sep} \code{Q^0}}{p{,}\bar{w_2}} }
\[
\begin{array}[t]{c}
   \constr_1'{=} \unfold(\D_1  {\wedge} \slice{ r{::}\bar{w}_1}{\pure_1}{,}
             \code{\seppred{\code{P^0}}{r{,}\bar{w}_1}}) \\
{\entailLEM{(\G {\cup} \{\lem \})}{\constr_1'}{\D_2 {\wedge}\slice{ [r;q]{@}\bar{w}_2@\bar{w}_3}{\pure_2}}
{\heap}{V}
{\textcolor{blue}{\emp}}{\flow}{\G_o}}
\end{array}
\]


==> entail-fig-cycle-pure.tex <==
\begin{figure*}[hbt]
\begin{center}
\begin{minipage}{0.98\textwidth}
\begin{frameit}
%\begin{small}
 \vspace{-2pt}
\[
\renewcommand{\arraystretch}{1.2}
\begin{array}[t]{c}
%
\synlem{LSYN-2PRED}\\
%% \pure_1'{=}\project{\pure_1}{r{::}\bar{w_1}} ~~
%% \pure_2'{=}\project{\pure_2}{r{::}\bar{w_2}} \quad
%% \code{lookup}(\G_i, \rlem,  \seppred{\code{P}}{r{,}\bar{w_1}}{\wedge}\pure_1',
%% \seppred{\code{Q}}{r{,}\bar{w_2}} {\wedge}\pure_2')
%%  {=} \code{\lemerr} \\
{t} = \code{pure}(\bar{w_1} \cup  \bar{w_2}) \quad \fresh ~\code{U} \quad
 \lem {=} {\seppred{\code{P}}{r{,}\bar{w_1}}}{\wedge}{\pure_1'}{\wedge}
 \seppred{\code{U}}{t} \rlem {\seppred{\code{Q}}{r{,}\bar{w_2}}}
{\wedge} {\pure_2'} \\
\bigvee^n_{j=1} \D^u_{j} {=} \unfold(\seppredF{\code{P}}{\setvars{w_1}}{\wedge}\pure_1',\code{P}, \setvars{w_1})
 \qquad
 \entailLEM{(\G_i \cup \{\lem \})}
{\D^u_{j}}{\heap}{V}{\D_2}{((\constr^R_{j},\flow_j),\G^o_{j})}\\
\hline
\synlemma{\G_i}{\seppred{\code{P}}{r{,}\bar{w_1}}}{\pure_1}
  {\seppred{\code{Q}}{r{,}\bar{w_2}}{\wedge}\pure_2}{\rlem} \yields \lem
\end{array}
\]
\hide{\[
\renewcommand{\arraystretch}{1.2}
\begin{array}[t]{c}
%
\synlem{LSYN-2PRED}\\
%% \pure_1'{=}\project{\pure_1}{r{::}\bar{w_1}} ~~
%% \pure_2'{=}\project{\pure_2}{r{::}\bar{w_2}} \quad
\code{lookup}(\G_i, \rlem,  \seppred{\code{P}}{r{,}\bar{w_1}}{\wedge}\pure_1',
\seppred{\code{Q}}{r{,}\bar{w_2}} {\wedge}\pure_2')
 {=} \code{\lemerr} \\
{t} = \code{pure}(\bar{w_1} \cup  \bar{w_2}) \quad \fresh ~\code{U} \quad
 \lem {=} {\seppred{\code{P}}{r{,}\bar{w_1}}}{\wedge}{\pure_1'}{\wedge}
 \seppred{\code{U}}{t} \rlem {\seppred{\code{Q}}{r{,}\bar{w_2}}}
{\wedge} {\pure_2'} \\
\bigvee^n_{j=1} \D^u_{j} {=} \unfold(\seppredF{\code{P}}{\setvars{w_1}}{\wedge}\pure_1',\code{P}, \setvars{w_1})
 \qquad
 \entailLEM{(\G_i \cup \{\lem \})}
{\D^u_{j}}{\heap}{V}{\D_2}{((\constr^R_{j},\flow_j),\G^o_{j})}\\
\hline
\synlemma{\G_i}{\seppred{\code{P}}{r{,}\bar{w_1}}}{\pure_1}
  {\seppred{\code{Q}}{r{,}\bar{w_2}}} {\pure_2}{\rlem} \yields \lem
\end{array}
\]}
\[
\renewcommand{\arraystretch}{1.2}
\begin{array}[t]{c}
%
\synlem{LSYN-FOLD}\\
%% \code{P} {\not=} \code{Q}
 \qquad r {\in} \bar{w_2} \qquad
  \lem {=} \synlemma{\G_i}{\sepnodeF{r}{c}{p{,}\setvars{w_1}} {\sep} \seppred{\code{P}}{p{,}\bar{w_3}}}
   {\pure_1}{\seppred{\code{Q}}{r{,}\bar{w_2}}}{\pure_2}{\rlem} \qquad \lem ~{\not=}~ \bot \\
\bigvee^n_{j=1} \D^f_{j} {=} \unfold(\seppred{\code{Q}}{\bar{w_2}} {\sep} \heap_2 {\wedge}\pure_2,\code{Q}, \setvars{w_2})
 \\
\entailLEM{(\G_i \cup \{\lem \})}{\sepnodeF{r}{c}{p{,}\setvars{w_1}} {\sep} \seppred{\code{P}}{p{,}\bar{w_3}}{\sep} \heap_1 {\wedge} \pure_1}{\heap}{V} {\D^f_{j}} {((\constr^R_j,\flow),\G^o_j)}\\
\hline
\entailLEM{\G_i}{\sepnodeF{r}{c}{p{,}\setvars{w_1}} {\sep} \seppred{\code{P}}{p{,}\bar{w_3}} {\sep}
                 \heap_1 {\wedge} \pure_1}{\heap}{V}{
\seppred{\code{Q}}{\bar{w_2}} {\sep} \heap_2 {\wedge} \pure_2}{(\efold \{(\D^R_{j}, \flow_j) \mid j{\in}1...n\},\G_i)}
\end{array}
\]
\[
\renewcommand{\arraystretch}{1.2}
\begin{array}[t]{c}
%
\synlem{LSYN-UNFOLD}\\
%% \code{P} {\not=} \code{Q} \qquad
 r {\in} \bar{w_1} \qquad
   \lem {=} \synlemma{\G_i}{ \seppred{\code{P}}{\bar{w_1}}} {\pure_1}
{\seppred{\sepnodeF{r}{c}{p{,}\setvars{w_3}} {\sep} \code{Q}}{p{,}\bar{w_2}}} {\pure_2}{\llem} \qquad \lem ~{\not=}~ \bot\\
\bigvee^n_{j=1} \D^u_{j} {=} \unfold(\seppredF{\code{P}}{\setvars{w_1}}{\sep}\heap_1{\wedge}\pure_1,\code{P}, \setvars{w_1})
 \\
\entailLEM{(\G_i \cup \{\lem \})}{\D^u_{j}}{\heap}{V}
{\seppred{\sepnodeF{r}{c}{p{,}\setvars{w_3}} {\sep} \code{Q}}{p{,}\bar{w_2}}{\sep}
\heap_2 {\wedge} \pure_2}{((\constr^R_j,\flow_j),\G^o_j)}\\
\hline
\entailLEM{\G_i}{ \seppred{\code{P}}{\bar{w_1}} {\sep} \heap_1 {\wedge} \pure_1}
{\heap}{V}
{\seppred{\sepnodeF{r}{c}{p{,}\setvars{w_3}} {\sep} \code{Q}}{p{,}\bar{w_2}} {\sep} \heap_2 {\wedge} \pure_2}
{(\eunfold \{(\D^R_{j}, \flow_j) \mid j{\in}1...n\},\G_i)}
\end{array}
\]
\caption{Inference Rules for Inductive Reasoning}\label{fig.entail.cycle}
 \vspace{-15pt}
\end{frameit}
 %\vspace{-10pt}
\end{minipage}
\end{center}
\end{figure*}

\hide{
\begin{figure}[hbt]
\begin{center}
\begin{minipage}{0.98\textwidth}
\begin{frameit}
%\begin{small}
 \vspace{-2pt}
\[
\renewcommand{\arraystretch}{1.2}
\begin{array}[t]{c}
%
\synlem{LSYN-2PRED}\\
%% \pure_1'{=}\project{\pure_1}{r{::}\bar{w_1}} ~~
%% \pure_2'{=}\project{\pure_2}{r{::}\bar{w_2}} \quad
%% \code{lookup}(\G_i, \rlem,  \seppred{\code{P}}{r{,}\bar{w_1}}{\wedge}\pure_1',
%% \seppred{\code{Q}}{r{,}\bar{w_2}} {\wedge}\pure_2')
%%  {=} \code{\lemerr} \\
{t} = \code{pure}(\bar{w_1} \cup  \bar{w_2}) \quad \fresh ~\code{U} \quad
 \lem {=} {\seppred{\code{P}}{r{,}\bar{w_1}}}{\wedge}{\pure_1'}{\wedge}
 \seppred{\code{U}}{t} \rlem {\seppred{\code{Q}}{r{,}\bar{w_2}}}
{\wedge} {\pure_2'} \\
\bigvee^n_{j=1} \D^u_{j} {=} \unfold(\seppredF{\code{P}}{\setvars{w_1}}{\wedge}\pure_1',\code{P}, \setvars{w_1})
 \qquad
 \entailLEM{(\G_i \cup \{\lem \})}
{\D^u_{j}}{\heap}{V}{\D_2}{((\constr^R_{j},\flow_j),\G^o_{j})}\\
\hline
\synlemma{\G_i}{\seppred{\code{P}}{r{,}\bar{w_1}}}{\pure_1}
  {\seppred{\code{Q}}{r{,}\bar{w_2}}} {\pure_2}{\rlem} \yields \lem
\end{array}
\]
\caption{Inference Rules for Inductive Reasoning}\label{fig.entail.cycle}
 \vspace{-15pt}
\end{frameit}
 %\vspace{-10pt}
\end{minipage}
\end{center}
\end{figure}
}


==> entail-old.tex <==
We begin this section with basic inference rules (in Fig. \ref{fig.entail}) for a entailment
procedure on separation logic. After that, we discuss
%% two sets
 set of
inference rules to enhance the completeness of the procedure in section
 \ref{entail.extra}. %% and section \ref{entail.cycle}.
Finally, we discuss a preliminary mechanism on lemma to support induction proving in section \ref{entail.lemma}.
\subsection{Essence of Entailment Procedure}
Entailment procedure between \form{\D_{ante}} and \form{\D_{conseq}} is formalized as follows:
\[
\entailVVE{\D_{ante}}{\D_{conseq}}{(\constr_R,\tau)}
\]

\noindent where \form{\heap} (V) is accumulated footprints (existential quantifiers of consequent, respectively).
The entailment outputs: \form{\constr_R} is residual frame and \form{\tau} is result: valid, invalid,
or unknown.

\hide{We start with a set of inference rules
for an essential entailment procedure in separation logic.
Those rules are presented in Fig. \ref{fig.entail}, and Fig. \ref{fig.entail.extra}.
After that 
 from the entailment procedure presented. This procedure is sound to prove validity, but invalidity due to
over-approximation. For invalid proving and more complete results,

We enhance entailment procedure in \cite{Nguyen:VMCAI07} to exact predicate invariant, segment fold rules,
and fold/unfold rules. We will present the extension in Fig. \ref{fig.entail}, and Fig. \ref{fig.entail.extra};
% , and Fig. \ref{fig.entail.cycle};
 other rules can be found in Appendix \ref{app.entail}.}

\input{entail-fig}

For entailment checking, we prove that (i) all matching models of the antecedent would be subsumed by
models of the consequent; (ii) irrelevant part of the antecedent will be inferred as residual frame.
Firstly, the matching of heap part is performed until
heap in the consequent is empty ($\entrulen{*-UNIFY}$,  $\entrulen{UNFOLD-L}$,
  $\entrulen{UNFOLD-R}$,
 $\entrulen{SEG-UNFOLD*}$ inference rules).
 After that, the implication of the pure part is checked semantically through
external SMT solvers and theorem provers ($\entrulen{XPURE}$ inference rule).
Typically, an entailment is performed as follows.
\begin{itemize}
\item {\bf Detecting dead proof. } Employ $\xpure$ reduction to check satisfiabilty of the antecedent through $\entrulen{DP}$ rule.
\item {\bf Matching.} Match up identified %% points-to
 heap chains.
       Starting from identified root pointers, the procedure keeps matching all their reachable heaps
with $\entrulen{PTO-UNIFY}$ and $\entrulen{SUMMARY-UNIFY}$ rules.
 The former (latter) rule matches two points-to (summary, resp.) predicates in antecedent
and consequent if they have identified root and stores matched points-to predicates in the footprint list
 \code{\heap}.
After that, it unifies corresponding fields of matched roots
 by using auxiliary function $\text{freeEQ}(\rho, V)$:
\form{\text{freeEQ}([u_i/v_i]^n_{i=1}, V) = \bigwedge^n_{i=1} \{ u_i = v_i ~|~ v_i \notin V\}}.
\item {\bf Unfolding.} Derive alternative %{\em points-to}
 heap chains.
 When the procedure is unable to make a progress on matching,
it will look up alternative chains for matching through unfolding heap predicates.
Different to unfolding in \cite{Nguyen:VMCAI07}, we do not restrict user-defined
predicates in a well-found form for generality. Thus, our procedure may not terminate with
unfolding. In implementation, we limit unfolding operations on
a heap predicate formula to a bounded number.
For unfolding in the antecedent ($\entrulen{UNFOLD-L}$ rule),
the unfolding does cases split in the proof
and combination of results is determined by the operator $\eunfold$.
For unfolding in the consequent ($\entrulen{UNFOLD-R}$ rule),
the unfolding does proof search over cases
and combination of results is determined by the operator \form{\efold}.
 Two operators \form{\eunfold} and \form{\efold}
 will be discussed in the next paragraph.
\item {\bf  $\xpure$ Reducing.} Reduce entailment checking on separation logic to implication checking
       on the first order-logic with $\entrulen{XPURE2}$ rule. When the consequent remains empty heap, e.g. $\emp \wedge \pure_{c}$,
the procedure employs $\entrulen{\xpure}$ inference rule
to decide the entailment result. Firstly, this rules make use of the $\xpure$ reduction to transform the combination of
 remain heaps in the antecedent
and footprints into the first order-logic formula on the combination of pure domains, e.g. $\pure_{a}$.
 Then it checks the implication \form{\pure_{a} \implies \pure_{c}}.
%% Technically, this implication is implemented through
%% SMT solvers and theorem provers like
%% Z3 \cite{TACAS08:Moura}, Omega \cite{Pugh:CACM} for arimethic domain, Mona \cite{klarlund-mona} for bag/set domain.
%%More concretely, 
Technically, to perform such implication checking,
 the following satisfiability check is performed:
\form{\satp{\pure_{a} ~{\wedge}~ \neg (\pure_{c})}}. If it returns \code{unsat}, the result of the implication is valid;
 it returns \code{sat}, the result of the implication is invalid; otherwise, the result of the implication is unknown.

\end{itemize}
During the heap chains matching,
aliasing relation on pointers are considered to introduce alternative proofs via
\form{\entrulen{ALIAS}} rule.

In the following, we present \form{\eunfold} and \form{\efold} operators for
combining unfolding/folding results. Without loss of generality,
we discuss those operators
 on the sets of two members. The extension of those operators on the sets of more than two members is
straightforward.
For the unfolding on the antecedent, case split returns valid if outputs of
all cases are valid (the first line below). Otherwise, the unfolding fails.
\[
 \begin{array}{l}
 {\eunfold} \{(\D_1,\flow_1),(\D_2,\flow_2) \} {=}\\
 \quad \left\{
  \begin{array}{l l}
    (\D_1 \vee \D_2, \text{valid}) & ~  \text {if } (\flow_1=\text{valid) and } (\flow_2=\text{valid)}\\
    (\D_1, \text{invalid}) & ~ \text{ otherwise}
  \end{array} \right.
 \end{array}
\]

For the folding, unfolding on the consequent, proof search returns valid
 if any outputs of
 searches are valid (the two first line below). Otherwise, the folding fails.
We would like to emphasize that for the sage of the failed proof search,
 our procedure gives higher priority on unknown (third and fourth lines)
 to invalid results (the two last lines).
\[
\begin{array}{l}
 \form{\efold} \{(\D_1,\flow_1),(\D_2,\flow_2) \} {=} \\
 \qquad \left\{
  \begin{array}{l l}
    (\D_1, \text{valid}) & \quad  \text {if } (\flow_1=\text{valid) }\\
    (\D_2, \text{valid}) & \quad  \text {if } (\flow_2=\text{valid) }\\
    (\D_1, \text{unknown}) & \quad  \text {if } (\flow_1=\text{unknown) }\\
    (\D_2, \text{unknown}) & \quad  \text {if } (\flow_2=\text{unknown) }\\
    (\D_1, \text{invalid}) & \quad \text{ otherwise}
  \end{array} \right.
 \end{array}
\]

\noindent{\bf Satisfiability with ${\xpure}$ Reduction} \locsay{} \cite{s2sat}

For fastening the proof searching,
 we discuss two heuristics to pick a predicate for unfolding as follows.
 With $\entrulen{UNFOLD-L}$ rule,
if \form{x} is a root and exists a points-to predicate in the consequent whose root
is \form{x},
among predicate formulas of the antecedent \form{\seppredF{\code{P}}{x,\setvars{w}}} should be given higher priority to be unfolded. (The entailment has the form of
\form{\seppredF{\code{P}}{x,\setvars{w}}{\sep}\D_1 \ent \sepnodeF{x}{c}{\setvars{v}} {\sep} \D_2}.)
Similarly, with $\entrulen{UNFOLD-R}$ rule,
if \form{x} is a root and exists a points-to predicate in the antecedent whose root
is \form{x},
among predicate formulas of the consequent
\form{\seppredF{\code{P}}{x,\setvars{w}}}
 should be given higher priority to be unfolded. (The entailment has the form of
\form{\sepnodeF{x}{c}{\setvars{v}} {\sep} \D_1 \ent \seppredF{\code{P}}{x,\setvars{w}} \sep \D_2}.)

We illustrate the entailment procedure though the following example.
%% \begin{footnotesize}
%% \[
%% \begin{array}{|l|}
%% \hline
%% \begin{array}{lr}
%% \begin{array}{l}
%% \begin{array}{|l|}
%% \hline
%% {\scriptsize 3.2.3}~ \seppredF{\code{lsegn}}{{q_2},\nil,n_2}  {\wedge} n{>}0 {\wedge} p{=}q {\wedge} n_2{=}n {-}1  ~\ent^{\heap_2}_\emptyset~ \emp  \yields (\D_2, \text{valid}) ~~ {\bf \scriptstyle XPURE}\\
%% {\scriptsize3.2.2}~ \seppredF{\code{lsegn}}{{q_2},\nil,n_2}  \wedge n{>}0 \wedge p{=}q \wedge n_2{=}n -1  ~\ent^{\heap_2}_\emptyset~ \emp  \qquad \quad \quad {\bf \scriptstyle MATCH}\\
%% {\scriptsize 3.2.1}~ \sepnodeF{q}{c_1}{q_2} {\sep}\seppredF{\code{lsegn}}{{q_2},\nil,n_2}  \wedge n{>}0 \wedge p{=}q \wedge n_2{=}n -1 \\
%%  \qquad \quad ~\ent^{\heap_1}_\emptyset~
%%   \sepnodeF{q}{c_1}{\nil}  \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad {\bf \scriptstyle EXs}\\
%% {\scriptsize 3.2}~ \exists q_1,n_1 \cdot \sepnodeF{q}{c_1}{q_1} {\sep}\seppredF{\code{lsegn}}{{q_1},\nil,n_1}  \wedge n{>}0 \wedge p{=}q \wedge n_1{=}n -1 \\
%%  \qquad \quad ~\ent^{\heap_1}_\emptyset~
%%  \exists q \cdot (\sepnodeF{q}{c_1}{\nil})  \\
%% \hline
%% \end{array}
%%  \\
%% \begin{array}{|l|}
%% \hline
%% {\scriptsize 3.1.1.}~q{=}\nil {\wedge} n{>}0 {\wedge} p{=}q {\wedge} n{=}0
%% ~\ent^{\heap_1}_\emptyset~ \exists q {\cdot} (\sepnodeF{q}{c_1}{\nil})
%% \yields (\D_1, \text{valid})
%% ~
%% {\bf \tiny  \scriptstyle DP} \\
%% {\scriptsize 3.1}~q=\nil \wedge n{>}0 \wedge p{=}q \wedge n{=}0
%% ~\ent^{\heap_1}_\emptyset~ \exists q \cdot (\sepnodeF{q}{c_1}{\nil}) \\
%% \hline
%% \end{array}
%% \end{array}
%%  &
%%  \\
%% {\scriptsize 2}~\seppredF{\code{lsegn}}{\textcolor{blue}{q},\nil,n} {\wedge} n{>}0 {\wedge} p{=}q
%% ~\ent^{\heap_1}_\emptyset~ \exists q {\cdot} (\sepnodeF{q}{c_1}{\nil})
%%  &
%% {\bf \tiny \scriptstyle ALIAS} \\
%% {\scriptsize 1}~ \seppredF{\code{lsegn}}{p,\nil,n} {\wedge} n{>}0 {\wedge} p{=}q
%% ~\ent^{\textcolor{blue}{\heap_1}}_\emptyset~ \exists q \cdot (\sepnodeF{q}{c_1}{\nil})
%%  &
%% {\bf \tiny \scriptstyle MATCH} \\
%% \hline
%% \end{array}\\
%% \begin{array}{c}
%% {\scriptsize 0}~\sepnodeF{x}{c_1}{p} {\sep} \seppredF{\code{lsegn}}{p,\nil,n} {\wedge} n{>}0 
%%  ~\ent^\emp_\emptyset ~ \exists q {\cdot} (\sepnodeF{x}{c_1}{q} {\sep} \sepnodeF{q}{c_1}{\nil})\\
%% \end{array}\\
%% \qquad  \yields (\D_1 \vee \D_2,\text{valid}) \\
%% \hline
%% \end{array}
%% \]
%% \end{footnotesize}
\begin{figure*}[tb]
 \begin{center}
 \begin{minipage}{0.8\textwidth}
 \begin{frameit} \savespace \savespace
%\begin{footnotesize}
\[
\begin{array}{|l|}
\hline
\begin{array}{l}
\begin{array}{l}
\begin{array}{|l|}
\hline
{\scriptsize 2.2.4}~ \seppredF{\code{lsegn}}{{q_1},\nil,n_2}  {\wedge} n{>}0 {\wedge} p{=}q {\wedge} n_2{=}n {-}1  ~\ent^{\heap_2}_\emptyset~ \emp  \yields (\D_2, \text{valid}) ~~ {\bf \scriptstyle XPURE}\\
{\scriptsize3.2.2}~ \seppredF{\code{lsegn}}{{q_2},\nil,n_2}  \wedge n{>}0 \wedge p{=}q \wedge n_2{=}n -1  ~\ent^{\heap_2}_\emptyset~ \emp  \qquad \quad \quad {\bf \scriptstyle UNIFY}\\
{\scriptsize 2.2.2}~ \sepnodeF{q_1}{c_1}{q_1} {\sep}\seppredF{\code{lsegn}}{{q_2},\nil,n_2}  \wedge n{>}0 \wedge p{=}q \wedge n_2{=}n -1 \\
 \qquad \quad ~\ent^{\heap_1}_\emptyset~
  \sepnodeF{q_2}{c_1}{\nil}  \qquad \qquad \qquad  \qquad \qquad \qquad \qquad \quad \qquad \qquad {\bf \scriptstyle RHS-EX}\\
{\scriptsize 2.2.1}~\exists q_1,n_1 \cdot \sepnodeF{\textcolor{blue}{q}}{c_1}{q_1} {\sep}\seppredF{\code{lsegn}}{{q_1},\nil,n_1}  \wedge n{>}0 \wedge p{=}q \wedge n_1{=}n -1 \\
\qquad \qquad ~\ent^{\heap_1}_\emptyset~ \exists q {\cdot} (\sepnodeF{q}{c_1}{\nil})
\qquad \qquad \qquad  \qquad \qquad  \qquad \qquad \qquad ~~
{\bf \tiny \scriptstyle ALIAS} \\
{\scriptsize 2.2}~ \exists q_1,n_1 \cdot \sepnodeF{p}{c_1}{q_1} {\sep}\seppredF{\code{lsegn}}{{q_1},\nil,n_1}  \wedge n{>}0 \wedge p{=}q \wedge n_1{=}n -1 \\
 \qquad \qquad ~\ent^{\heap_1}_\emptyset~
 \exists q \cdot (\sepnodeF{q}{c_1}{\nil}) \qquad \qquad \qquad ~~ \quad \qquad  \qquad  \qquad {\bf \tiny \scriptstyle UNFOLD(Ind)} \\
\hline
\end{array}
 \\
\begin{array}{|l|}
\hline
{\scriptsize 2.1.1.}~p{=}\nil {\wedge} n{>}0 {\wedge} p{=}q {\wedge} n{=}0
~\ent^{\heap_1}_\emptyset~ \exists q {\cdot} (\sepnodeF{q}{c_1}{\nil})
\yields (\D_1, \text{valid})
~
{\bf \tiny  \scriptstyle XPURE} \\
{\scriptsize 2.1}~p=\nil \wedge n{>}0 \wedge p{=}q \wedge n{=}0
~\ent^{\heap_1}_\emptyset~ \exists q \cdot (\sepnodeF{q}{c_1}{\nil}) \qquad \quad  {\bf \tiny \scriptstyle UNFOLD(Base)}\\
\hline
\end{array}
\end{array}
 
 \\
{\scriptsize 1}~ \seppredF{\code{lsegn}}{p,\nil,n} {\wedge} n{>}0 {\wedge} p{=}q
~\ent^{\textcolor{blue}{\heap_1}}_\emptyset~ \exists q \cdot (\sepnodeF{q}{c_1}{\nil})
  \qquad \qquad \qquad ~~ \quad \qquad  \qquad 
{\bf \tiny \scriptstyle UNIFY} \\
\hline
\end{array}\\
\begin{array}{c}
{\scriptsize 0}~\sepnodeF{x}{c_1}{p} {\sep} \seppredF{\code{lsegn}}{p,\nil,n} {\wedge} n{>}0 
 ~\ent^\emp_\emptyset ~ \exists q {\cdot} (\sepnodeF{x}{c_1}{q} {\sep} \sepnodeF{q}{c_1}{\nil})\\
\end{array}\\
\qquad  \yields (\D_1 \vee \D_2,\text{valid}) \\
\hline
\end{array}
\]
%\end{footnotesize}
\end{frameit}
\end{minipage}
\caption{Entailment Example}\label{ent.example.fig}
\end{center}
\end{figure*}
\noindent where
the steps from 3.2 to 3.2.3 (in the box) corresponds to  ${\bf \scriptstyle UNFOLD-L}$ (short for $\entrulen{UNFOLD-L}$ rule);
 the footprints \form{\heap_1{=}\sepnodeF{x}{c_1}{p}}, and
\form{\heap_2{=} \heap_1 \sep \sepnodeF{q}{c_1}{q_2}}.
The residual heap in two cases of the unfolding is:
\form{\D_1{=}q{=}\nil {\wedge} n{>}0 {\wedge} p{=}q {\wedge} n{=}0} and

\noindent\form{\D_2{=} \seppredF{\code{lsegn}}{{q_2},\nil,n_2}  {\wedge} n{>}0 {\wedge} p{=}q {\wedge} n_2{=}n {-}1}.

In the above proof tree,
the LHS of the entailment is performed bottom-up while the result in RHS
is computed top-down. For simplicity, we discard some intermediate RHS.

Compared to the entailment procedure in \cite{Nguyen:VMCAI07}, the main advantage of our entailment procedure is
the use of  exact predicate invariant, instead of over-approximate (like in \cite{Nguyen:VMCAI07}).
This enhances the completeness of
 our decision procedure, i.e. we  can confirm invalid entailments beside the valid ones.


\subsection{On Complete Entailment Procedure}\label{entail.extra}

\input{entail-extra}


\subsection{Lemma Mechanism for Induction Proving}\label{entail.lemma}
\input{entail-lemma}

\subsection{On Induction Proving}
\label{entail.cycle}
\input{entail-cycle}





==> entail-old2.tex <==
We begin this section with basic inference rules (in Fig. \ref{fig.entail}) for a entailment
procedure on separation logic. After that, we discuss
%% two sets
 set of
inference rules to enhance the completeness of the procedure in section
 \ref{entail.extra}. %% and section \ref{entail.cycle}.
Finally, we discuss a preliminary mechanism on lemma to support induction proving in section \ref{entail.lemma}.

\subsection{Essence of Entailment Procedure}
Entailment procedure between \form{\D_{a}} and \form{\D_{c}} is formalized as follows:
\[
\entailSS{\lemstore_i}{\D_{a}}{\D_{c}}{\ustack}{\constr_R}{\lemstore_o}{\tau}
\]

\noindent where \form{\heap} (V) is accumulated footprints (existential quantifiers of consequent, respectively).
The entailment outputs: \form{\constr_R} is residual frame and \form{\tau} is result: valid, invalid,
or unknown.

\hide{We start with a set of inference rules
for an essential entailment procedure in separation logic.
Those rules are presented in Fig. \ref{fig.entail}, and Fig. \ref{fig.entail.extra}.
After that 
 from the entailment procedure presented. This procedure is sound to prove validity, but invalidity due to
over-approximation. For invalid proving and more complete results,

We enhance entailment procedure in \cite{Chin:SCP:12} to exact predicate invariant, segment fold rules,
and fold/unfold rules. We will present the extension in Fig. \ref{fig.entail}, and Fig. \ref{fig.entail.extra};
% , and Fig. \ref{fig.entail.cycle};
 other rules can be found in Appendix \ref{app.entail}.}

\input{entail-fig}

For entailment checking, we prove that (i) all matching models of the antecedent would be subsumed by
models of the consequent; (ii) irrelevant part of the antecedent will be inferred as residual frame.
Firstly, the matching of heap part is performed until
heap in the consequent is empty ($\entrulen{*-UNIFY}$,  $\entrulen{UNFOLD-L}$,
  $\entrulen{UNFOLD-R}$,
 $\entrulen{SEG-UNFOLD*}$ inference rules).
 After that, the implication of the pure part is checked semantically through
external SMT solvers and theorem provers ($\entrulen{XPURE}$ inference rule).
Typically, an entailment is performed as follows.
\begin{itemize}
\item {\bf Detecting dead proof. } Employ $\xpure$ reduction to check satisfiabilty of the antecedent through $\entrulen{DP}$ rule.
\item {\bf Matching.} Match up identified %% points-to
 heap chains.
       Starting from identified root pointers, the procedure keeps matching all their reachable heaps
with $\entrulen{PTO-UNIFY}$ and $\entrulen{SUMMARY-UNIFY}$ rules.
 The former (latter) rule matches two points-to (summary, resp.) predicates in antecedent
and consequent if they have identified root and stores matched points-to predicates in the footprint list
 \code{\heap}.
After that, it unifies corresponding fields of matched roots
 by using auxiliary function $\text{freeEQ}(\rho, V)$:
\form{\text{freeEQ}([u_i/v_i]^n_{i=1}, V) = \bigwedge^n_{i=1} \{ u_i = v_i ~|~ v_i \notin V\}}.
\item {\bf Unfolding.} Derive alternative %{\em points-to}
 heap chains.
 When the procedure is unable to make a progress on matching,
it will look up alternative chains for matching through unfolding heap predicates.
Different to unfolding in \cite{Nguyen:VMCAI07}, we do not restrict user-defined
predicates in a well-found form for generality. Thus, our procedure may not terminate with
unfolding. In implementation, we limit unfolding operations on
a heap predicate formula to a bounded number.
For unfolding in the antecedent ($\entrulen{UNFOLD-L}$ rule),
the unfolding does cases split in the proof
and combination of results is determined by the operator $\eunfold$.
For unfolding in the consequent ($\entrulen{UNFOLD-R}$ rule),
the unfolding does proof search over cases
and combination of results is determined by the operator \form{\efold}.
 Two operators \form{\eunfold} and \form{\efold}
 will be discussed in the next paragraph.
\item {\bf  $\xpure$ Reducing.} Reduce entailment checking on separation logic to implication checking
       on the first order-logic with $\entrulen{XPURE2}$ rule. When the consequent remains empty heap, e.g. $\emp \wedge \pure_{c}$,
the procedure employs $\entrulen{\xpure}$ inference rule
to decide the entailment result. Firstly, this rules make use of the $\xpure$ reduction to transform the combination of
 remain heaps in the antecedent
and footprints into the first order-logic formula on the combination of pure domains, e.g. $\pure_{a}$.
 Then it checks the implication \form{\pure_{a} \implies \pure_{c}}.
%% Technically, this implication is implemented through
%% SMT solvers and theorem provers like
%% Z3 \cite{TACAS08:Moura}, Omega \cite{Pugh:CACM} for arimethic domain, Mona \cite{klarlund-mona} for bag/set domain.
%%More concretely, 
Technically, to perform such implication checking,
 the following satisfiability check is performed:
\form{\satp{\pure_{a} ~{\wedge}~ \neg (\pure_{c})}}. If it returns \code{unsat}, the result of the implication is valid;
 it returns \code{sat}, the result of the implication is invalid; otherwise, the result of the implication is unknown.

\end{itemize}
During the heap chains matching,
aliasing relation on pointers are considered to introduce alternative proofs via
\form{\entrulen{ALIAS}} rule.

In the following, we present \form{\eunfold} and \form{\efold} operators for
combining unfolding/folding results. Without loss of generality,
we discuss those operators
 on the sets of two members. The extension of those operators on the sets of more than two members is
straightforward.
For the unfolding on the antecedent, case split returns valid if outputs of
all cases are valid (the first line below). Otherwise, the unfolding fails.
\[
 \begin{array}{l}
 {\eunfold} \{(\D_1,\flow_1),(\D_2,\flow_2) \} {=}\\
 \quad \left\{
  \begin{array}{l l}
    (\D_1 \vee \D_2, \text{valid}) & ~  \text {if } (\flow_1=\text{valid) and } (\flow_2=\text{valid)}\\
    (\D_1, \text{invalid}) & ~ \text{ otherwise}
  \end{array} \right.
 \end{array}
\]

For the folding, unfolding on the consequent, proof search returns valid
 if any outputs of
 searches are valid (the two first line below). Otherwise, the folding fails.
We would like to emphasize that for the sage of the failed proof search,
 our procedure gives higher priority on unknown (third and fourth lines)
 to invalid results (the two last lines).
\[
\begin{array}{l}
 \form{\efold} \{(\D_1,\flow_1),(\D_2,\flow_2) \} {=} \\
 \qquad \left\{
  \begin{array}{l l}
    (\D_1, \text{valid}) & \quad  \text {if } (\flow_1=\text{valid) }\\
    (\D_2, \text{valid}) & \quad  \text {if } (\flow_2=\text{valid) }\\
    (\D_1, \text{unknown}) & \quad  \text {if } (\flow_1=\text{unknown) }\\
    (\D_2, \text{unknown}) & \quad  \text {if } (\flow_2=\text{unknown) }\\
    (\D_1, \text{invalid}) & \quad \text{ otherwise}
  \end{array} \right.
 \end{array}
\]

\noindent{\bf Satisfiability with ${\xpure}$ Reduction} \locsay{} \cite{s2sat}

For fastening the proof searching,
 we discuss two heuristics to pick a predicate for unfolding as follows.
 With $\entrulen{UNFOLD-L}$ rule,
if \form{x} is a root and exists a points-to predicate in the consequent whose root
is \form{x},
among predicate formulas of the antecedent \form{\seppredF{\code{P}}{x,\setvars{w}}} should be given higher priority to be unfolded. (The entailment has the form of
\form{\seppredF{\code{P}}{x,\setvars{w}}{\sep}\D_1 \ent \sepnodeF{x}{c}{\setvars{v}} {\sep} \D_2}.)
Similarly, with $\entrulen{UNFOLD-R}$ rule,
if \form{x} is a root and exists a points-to predicate in the antecedent whose root
is \form{x},
among predicate formulas of the consequent
\form{\seppredF{\code{P}}{x,\setvars{w}}}
 should be given higher priority to be unfolded. (The entailment has the form of
\form{\sepnodeF{x}{c}{\setvars{v}} {\sep} \D_1 \ent \seppredF{\code{P}}{x,\setvars{w}} \sep \D_2}.)

We illustrate the entailment procedure though the following example.
\begin{figure*}[tb]
 \begin{center}
 \begin{minipage}{0.8\textwidth}
 \begin{frameit} \savespace \savespace
%\begin{footnotesize}
\[
\begin{array}{|l|}
\hline
\begin{array}{l}
\begin{array}{l}
\begin{array}{|l|}
\hline
{\scriptsize 2.2.4}~ \seppredF{\code{lsegn}}{{q_1},\nil,n_2}  {\wedge} n{>}0 {\wedge} p{=}q {\wedge} n_2{=}n {-}1  ~\ent^{\heap_2}_\emptyset~ \emp  \yields (\D_2, \text{valid}) ~~ {\bf \scriptstyle XPURE}\\
{\scriptsize3.2.2}~ \seppredF{\code{lsegn}}{{q_2},\nil,n_2}  \wedge n{>}0 \wedge p{=}q \wedge n_2{=}n -1  ~\ent^{\heap_2}_\emptyset~ \emp  \qquad \quad \quad {\bf \scriptstyle UNIFY}\\
{\scriptsize 2.2.2}~ \sepnodeF{q_1}{c_1}{q_1} {\sep}\seppredF{\code{lsegn}}{{q_2},\nil,n_2}  \wedge n{>}0 \wedge p{=}q \wedge n_2{=}n -1 \\
 \qquad \quad ~\ent^{\heap_1}_\emptyset~
  \sepnodeF{q_2}{c_1}{\nil}  \qquad \qquad \qquad  \qquad \qquad \qquad \qquad \quad \qquad \qquad {\bf \scriptstyle RHS-EX}\\
{\scriptsize 2.2.1}~\exists q_1,n_1 \cdot \sepnodeF{\textcolor{blue}{q}}{c_1}{q_1} {\sep}\seppredF{\code{lsegn}}{{q_1},\nil,n_1}  \wedge n{>}0 \wedge p{=}q \wedge n_1{=}n -1 \\
\qquad \qquad ~\ent^{\heap_1}_\emptyset~ \exists q {\cdot} (\sepnodeF{q}{c_1}{\nil})
\qquad \qquad \qquad  \qquad \qquad  \qquad \qquad \qquad ~~
{\bf \tiny \scriptstyle ALIAS} \\
{\scriptsize 2.2}~ \exists q_1,n_1 \cdot \sepnodeF{p}{c_1}{q_1} {\sep}\seppredF{\code{lsegn}}{{q_1},\nil,n_1}  \wedge n{>}0 \wedge p{=}q \wedge n_1{=}n -1 \\
 \qquad \qquad ~\ent^{\heap_1}_\emptyset~
 \exists q \cdot (\sepnodeF{q}{c_1}{\nil}) \qquad \qquad \qquad ~~ \quad \qquad  \qquad  \qquad {\bf \tiny \scriptstyle UNFOLD(Ind)} \\
\hline
\end{array}
 \\
\begin{array}{|l|}
\hline
{\scriptsize 2.1.1.}~p{=}\nil {\wedge} n{>}0 {\wedge} p{=}q {\wedge} n{=}0
~\ent^{\heap_1}_\emptyset~ \exists q {\cdot} (\sepnodeF{q}{c_1}{\nil})
\yields (\D_1, \text{valid})
~
{\bf \tiny  \scriptstyle XPURE} \\
{\scriptsize 2.1}~p=\nil \wedge n{>}0 \wedge p{=}q \wedge n{=}0
~\ent^{\heap_1}_\emptyset~ \exists q \cdot (\sepnodeF{q}{c_1}{\nil}) \qquad \quad  {\bf \tiny \scriptstyle UNFOLD(Base)}\\
\hline
\end{array}
\end{array}
 
 \\
{\scriptsize 1}~ \seppredF{\code{lsegn}}{p,\nil,n} {\wedge} n{>}0 {\wedge} p{=}q
~\ent^{\textcolor{blue}{\heap_1}}_\emptyset~ \exists q \cdot (\sepnodeF{q}{c_1}{\nil})
  \qquad \qquad \qquad ~~ \quad \qquad  \qquad 
{\bf \tiny \scriptstyle UNIFY} \\
\hline
\end{array}\\
\begin{array}{c}
{\scriptsize 0}~\sepnodeF{x}{c_1}{p} {\sep} \seppredF{\code{lsegn}}{p,\nil,n} {\wedge} n{>}0 
 ~\ent^\emp_\emptyset ~ \exists q {\cdot} (\sepnodeF{x}{c_1}{q} {\sep} \sepnodeF{q}{c_1}{\nil})\\
\end{array}\\
\qquad  \yields (\D_1 \vee \D_2,\text{valid}) \\
\hline
\end{array}
\]
%\end{footnotesize}
\end{frameit}
\end{minipage}
\caption{Entailment Example}\label{ent.example.fig}
\end{center}
\end{figure*}
\noindent where
the steps from 3.2 to 3.2.3 (in the box) corresponds to  ${\bf \scriptstyle UNFOLD-L}$ (short for $\entrulen{UNFOLD-L}$ rule);
 the footprints \form{\heap_1{=}\sepnodeF{x}{c_1}{p}}, and
\form{\heap_2{=} \heap_1 \sep \sepnodeF{q}{c_1}{q_2}}.
The residual heap in two cases of the unfolding is:
\form{\D_1{=}q{=}\nil {\wedge} n{>}0 {\wedge} p{=}q {\wedge} n{=}0} and

\noindent\form{\D_2{=} \seppredF{\code{lsegn}}{{q_2},\nil,n_2}  {\wedge} n{>}0 {\wedge} p{=}q {\wedge} n_2{=}n {-}1}.

In the above proof tree,
the LHS of the entailment is performed bottom-up while the result in RHS
is computed top-down. For simplicity, we discard some intermediate RHS.

Compared to the entailment procedure in \cite{Nguyen:VMCAI07}, the main advantage of our entailment procedure is
the use of  exact predicate invariant, instead of over-approximate (like in \cite{Nguyen:VMCAI07}).
This enhances the completeness of
 our decision procedure, i.e. we  can confirm invalid entailments beside the valid ones.

\hide{
\subsection{On Complete Entailment Procedure}\label{entail.extra}

\input{entail-extra}


\subsection{Lemma Mechanism for Induction Proving}\label{entail.lemma}
\input{entail-lemma}

\subsection{On Induction Proving}
\label{entail.cycle}
\input{entail-cycle}
}




==> entail-proof.tex <==
 We will show that for all
 $\D_{{a}}$ and $\D_{c}$ such that \form{\entailSA{\setvars{P}}{\D_{{a}}}
 {\D_{c}} {\RA}{\D_{\code{frame}}}}

\noindent and
$\Gamma{=}\{\form{\code{\UNK_1}(\setvars{v}_1){\implyeq}\D_1},..\form{\code{\UNK_n}(\setvars{v}_n){\implyeq}\D_n}\}$,
a set of definitions for unknown predicates
such that $\assumpset(\Gamma)$ then the entailment $
\sols \D_{a}\vdash \D_{c}{\sep}\D_{\code{frame}}$
holds.
We will show  by structural induction on \hide{$\D_a$ and} $\D_c$.

Due to the construction of the $\entailSA{\setvars{P}}{\D_{a}}
 {\D_{c}} {\RA}{\D_{\code{frame}}}$ procedure as an extension of  an
 existing entailment procedure with frame inference, for all  $\D_{a}$
 and $\D_{c}$ not involving unknown predicates
 $\RA=\true\hide{\emptyset}$ and $ \sols \D_{a}\vdash
\D_{c}{\sep}\D_{\code{frame}}$. 

Bellow we consider the cases that actually involve unknown predicates. These
cases fall under two categories:

 \begin{enumerate}
   \item
 $\D_a=
  \seppredF{\code{\UNK}}{\form{r,\setvars{w},\setvars{z}\NI}}{\sep}\heap_1{\wedge}\pure_1$
  and $\D_c=\head(r{,}\setvars{t}){\sep}\heap_2{\wedge}\pure_2$ where 
  $\form{\head(r{,}\setvars{t}) \equiv \sepnodeF{r}{c}{\setvars{t}}}$ or
  $\form{\head(r{,}\setvars{t}) \equiv\seppredF{P}{r,\setvars{t}}}$,
or $\form{\head(r{,}\setvars{t}) \equiv  \seppredF{\code{\UNK'}}{\form{r,\setvars{t}}}}$. By hypothesis
  $ \entailSA{\setvars{P}}{\D_{a}} {\D_{c}}
  {\RA}{\D_{\code{frame}}}$. Then, as described
  in Sec.\ref{sec.entail.sound} the \form{\entrulen{AU}} step must hold ensuring the
  following assertion holds:
\[
{\entailSA{}{\seppredF{\code{\UNK_f}}{\setvars{w},\setvars{t'},\setvars{z}\NI,r\NI}{\sep}\heap_1{\sep}{\wedge}\pure_1}
{\heap_2{\wedge}\pure_2}{\Horn'}{\D_{f}}}
\]
where $ \form{\Horn = \Horn' \wedge %\cup
\seppredF{\code{\UNK}}{r{,}\setvars{w},\setvars{z}\NI}
~{\imply}~
\head(r{,}\setvars{t}){\sep} \seppredF{\code{\UNK_f}}{\setvars{w},\setvars{t'},\setvars{z}\NI,r\NI} {\wedge}\FIL{\setvars{w}\cup\{r\}}{\pure_1}
}$.
 It follows from the structural induction hypothesis that:
 \begin{equation}\label{eq:l11}
 \sols {\seppredF{\code{\UNK_f}}{\setvars{w},\setvars{t'},\setvars{z}\NI,r\NI}{\sep}\heap_1{\sep}{\wedge}\pure_1
\vdash (\heap_2{\wedge}\pure_2)\sep \D_{f}}
\end{equation}
From $\assumpset(\Gamma)$ it follows that
 \begin{equation}\label{eq:l12}
 \sols \form{
\seppredF{\code{\UNK}}{r{,}\setvars{w},\setvars{z}\NI}
{\vdash}
\head(r{,}\setvars{t}){\sep} \seppredF{\code{\UNK_f}}{\setvars{w},\setvars{t'},\setvars{z}\NI,r\NI} {\wedge}\FIL{\setvars{w}\cup\{r\}}{\pure_1}
}
 \end{equation}
 From equations \ref{eq:l11} and \ref{eq:l12} it follows that 
  $\sols \D_{a} \vdash \D_{c} \sep \D_{\code{f}}$.

\item
%%\noindent {\bf \form{\entrulen{AF}}} rule.
 $\form{\D_a{=}\head(r{,}\setvars{t}){\sep}\heap_1 {\wedge}\pure_1}$
  and
  $\form{\D_c{=}\seppredF{\UNK_c}{\setvars{w}{,}\setvars{z}\NI}{\sep}\heap_2
  {\wedge}\pure_2}$.
  By hypothesis :$
  \entailSA{\setvars{P}}{\D_{a}} {\D_{c}}
  {\RA}{\D_{\code{f}}}$.\\
  Then, as described
  in Sec.\ref{sec.entail.sound} the \form{\entrulen{AF}}  step must hold ensuring the
  following assertions hold:
  \[
{\entailSA{}{\head(r{,}\setvars{t}){\sep}\heap_1 {\wedge}\pure_1}
{\seppredF{\UNK_c}{\setvars{w}{,}\setvars{z}\NI}{\sep}\heap_2
  {\wedge}\pure_2 }{\Horn'}{\D_{f}}}
\]
where $ \form{\Horn = \Horn' \wedge %\cup
\head(r{,}\setvars{t}){\sep} \seppredF{\code{\UNK_f}}{\setvars{w},\setvars{t'},\setvars{z}\NI,r\NI} {\wedge}\FIL{\setvars{w}\cup\{r\}}{\pure_1}~{\imply}~
\seppredF{\UNK}{r{,}\setvars{w},\setvars{z}\NI}
}$.
 It follows from the structural induction hypothesis that:
 \begin{equation}\label{eq:l13}
 \sols {
\heap_{1}~{\wedge}~\pure_1
\vdash
 (\seppredF{\code{\UNK_f}}{\setvars{w},\setvars{t'},\setvars{z}\NI,r\NI} {\sep}\heap_2 ~{\wedge}~\pure_2)
 {\sep} \D_{f}
}
\end{equation}
From $\assumpset(\Gamma)$ it follows that
 \begin{equation}\label{eq:l14}
 \sols \form{
\head(r{,}\setvars{t}){\sep} \seppredF{\code{\UNK_f}}{\setvars{w},\setvars{t'},\setvars{z}\NI,r\NI} {\wedge}\FIL{\setvars{w}\cup\{r\}}{\pure_1}
{\vdash}
\seppredF{\UNK}{r{,}\setvars{w},\setvars{z}\NI}
}
 \end{equation}
 From equations \ref{eq:l13} and \ref{eq:l14} it follows that 
  $\sols \D_{a} \vdash \D_{c} \sep \D_{\code{f}}$.



\item \form{\D_a{=}\heap_1 {\wedge} \seppredF{\code{\UNKP}}{\setvars{w}}{\wedge}\pure_1} and
\form{\D_c{=}\emp {\wedge}\pure_2}.
The proof of this case is similar to the proof of the first case.

\item  \form{\D_a{=} \heap_1 {\wedge}\pure_1} and
\form{\D_c{=} \emp {\wedge} \seppredF{\code{\UNKP}}{\setvars{w}}
{\wedge}\pure_2}.
The proof of this case is similar to the proof of the second case.
 \end{enumerate}
 \qed


==> ex-syn-lem1.tex <==
For example,
\[
{\exists}q{\cdot}~
 \form{\seppred{\code{lsegn}}{\self{,}q{,}m}{\sep} \sepnode{\code{q}}{c_1}{\nil}
{\wedge} \code{P}(n,m)}
~{\rightarrow} ~
 \form{\seppred{\code{lln}}{\self{,}n} 
;}
\]

base case
\[
\form{{\exists}q{\cdot}  \sepnode{\code{q}}{c_1}{\nil} {\wedge} \self{=}q
{\wedge} \code{P}(n,m) {\wedge}m{=}0 {\wedge}n{=}1
~{\ent} ~
 \form{\sepnode{\code{\self}}{c_1}{\nil}  }
;}
\]

\[
\RA_0 {\equiv} m{=}0 {\wedge} \code{P}(n,m)  {\wedge}n{=}1 \imply \emp{\wedge}\true
\]

inductive case
\[
 \form{~\exists ~q,q_1 {\cdot}~ \sepnode{\code{\self}}{c_1}{q_1} {\sep}
\seppred{\code{lsegn}}{q_1{,}q{,}m_1}{\sep}\sepnode{\code{q}}{c_1}{\nil} {\wedge}m{=}m_1{+}1 {\wedge} \code{P}(n,m)}  ~{\ent} ~{\exists}q_2{\cdot}~
 \form{\sepnode{\code{\self}}{c_1}{q_2} {\sep}\seppred{\code{lln}}{q_2{,}n_1}{\wedge} n{=}n_1{+}1
;}
\]

match \form{\self}

\[
 \form{~\exists ~q {\cdot}~
\seppred{\code{lsegn}}{q_1{,}q{,}m_1}{\sep}\sepnode{\code{q}}{c_1}{\nil} {\wedge}m{=}m_1{+}1 {\wedge} \code{P}(n,m) {\wedge}q_1{=}q_2}{\wedge} n{=}n_1{+}1  ~{\ent} ~
 \form{\seppred{\code{lln}}{q_2{,}n_1}
;}
\]

apply lemma \code{l_1}, need to prove
\locsay{fresh free variable in LHS of lemma, subst into RHS}

\form{\rho{=} [\self/q_1, m/m_1]}

prove heap
\[
 \form{~\exists ~q {\cdot}~
\seppred{\code{lsegn}}{q_1{,}q{,}m_1}{\sep}\sepnode{\code{q}}{c_1}{\nil} {\wedge}m{=}m_1{+}1 {\wedge} \code{P}(n,m) {\wedge}q_1{=}q_2} {\wedge} n{=}n_1{+}1  ~{\ent} ~
 {\exists}q{\cdot}~
 \form{\seppred{\code{lsegn}}{q_1{,}q{,}m_1}{\sep} \sepnode{\code{q}}{c_1}{\nil}}
\]

match \form{q_1,q}
\[
 \form{m{=}m_1{+}1 {\wedge} \code{P}(n,m) {\wedge}q_1{=}q_2} {\wedge} n{=}n_1{+}1{\wedge}m_1{\geq}0  ~{\ent} ~
  \emp {\wedge} \true
\]

combine RHS of lemma l1

\[
 \form{\seppred{\code{lln}}{q_1{,}n_{fr}} {\wedge} {m{=}m_1{+}1 {\wedge} \code{P}(n,m) {\wedge}q_1{=}q_2} {\wedge} n{=}n_1{+}1 {\wedge}m_1{\geq}0 }  ~{\ent} ~
 \form{\seppred{\code{lln}}{q_2{,}n_1}
;}
\]

match
\[
 \form{{m{=}m_1{+}1 {\wedge} \code{P}(n,m) {\wedge}q_1{=}q_2} {\wedge} n{=}n_1{+}1  {\wedge} n_1{=}n_{fr}{\wedge}m_1{\geq}0 {\wedge}n_{fr}{\geq}0}   ~{\ent} ~
 \emp{\wedge}\true
\]

\[
\RA_2 {\equiv} \true
\]

prove guard
\[
 \form{m{=}m_1{+}1 {\wedge} \code{P}(n,m) {\wedge}q_1{=}q_2} {\wedge} n{=}n_1{+}1 {\wedge} n_1{=}n_{fr} {\wedge}m_1{\geq}0 {\wedge}n_{fr}{\geq}0
 ~{\ent} ~  \form{ \code{P}(n_{fr},m_1)}
\]


\[
\RA_3 {\equiv} m{=}m_1{+}1 {\wedge} \code{P}(n,m) {\wedge} {\wedge} n{=}n_1{+}1 {\wedge} n_1{=}n_{fr} {\wedge}m_1{\geq}0 {\wedge}n_{fr}{\geq}0
\imply \code{P}(n_{fr},m_1)
\]


==> ex-syn-lem2.tex <==
For example,
\[
 \form{\seppred{\code{lln}}{\self{,}n} {\wedge} \code{P}(n,i,j)}  ~{\rightarrow} ~{\exists}q{\cdot}~
 \form{\seppred{\code{lsegn}}{\self{,}q{,}i}{\sep} \seppred{\code{lln}}{q{,}j}
;}
\]

base case
\[
 \form{\self{=}\nil {\wedge}n{=}0 {\wedge} \code{P}(n,i,j)}  ~{\ent} ~{\exists}q{\cdot}~
 \form{\seppred{\code{lsegn}}{\self{,}q{,}i}{\sep} \seppred{\code{lln}}{q{,}j}
;}
\]

\[
 \form{\self{=}\nil {\wedge}n{=}0 {\wedge} \code{P}(n,i,j)}  ~{\ent} ~
 \form{x{=}\nil {\wedge}i{=}0 {\wedge}j{=}0}
\]

inductive case
\[
 \form{~\exists ~p {\cdot}~ \sepnode{\code{\self}}{c_1}{p} {\sep}
\seppred{\code{lln}}{p{,}n_1} {\wedge}n{=}n_1{+}1 {\wedge} \code{P}(n,i,j)}  ~{\ent} ~{\exists}q{\cdot}~
 \form{\seppred{\code{lsegn}}{\self{,}q{,}i}{\sep} \seppred{\code{lln}}{q{,}j}
;}
\]

ic1
\[
 \form{~\exists ~p {\cdot}~ \sepnode{\code{\self}}{c_1}{p} {\sep}
\seppred{\code{lln}}{p{,}n_1} {\wedge}n{=}n_1{+}1 {\wedge} \code{P}(n,i,j)}  ~{\ent} ~{\exists}q{\cdot}~
 \form{\self{=}q{\wedge}i{=}0{\sep} \seppred{\code{lln}}{q{,}j}
}
\]
\[
 \form{\self{\neq}\nil{\wedge} n{=}n_1{+}1 {\wedge} \code{P}(n,i,j)}  ~{\ent} 
 \form{i{=}0{\wedge}j{=}j_1{+}1 {\wedge} n_1{=}j_1
}
\]

ic2
\[
 \form{~\exists ~p_1 {\cdot}~ \sepnode{\code{\self}}{c_1}{p} {\sep}
\seppred{\code{lln}}{p{,}n_1} {\wedge}n{=}n_1{+}1 {\wedge} \code{P}(n,i,j)}  ~{\ent} ~{\exists}q,p_2{\cdot}~
 \form{\sepnode{\code{\self}}{c_1}{p_2} {\sep}
\seppred{\code{lsegn}}{p_2{,}i_1}{\sep} \seppred{\code{lln}}{q{,}j}
{\wedge}i{=}i_1{+}1 
}
\]


==> ex-syn-lem3.tex <==
For illustration,  %% we
  %% show how \code{lemprove} proves the following
consider the following conjecture with two unknown shape predicates \code{Q_1}, \code{Q_2}:
\form{\code{lemma~para~}\seppred{\code{zip}}{\self{,}r_2}
{\rightarrow}
 \seppred{\code{Q_1}}{\self} {\sep}  \seppred{\code{Q_2}}{r_2}};
whereas \code{zip} is defined by
\savespace
\[\savespace
\begin{array}{l}
\form{\defpred~ \seppred{\code{zip}}{r_1{,}r_2}} {\equiv}
\form{\emp} {\wedge} \form{r_1{=}\nil {\wedge} r_2{=}\nil}
 {\vee} \form{{\exists}q_1{,}q_2 {\cdot}~ \sepnode{r_1}{c_1}{q_1} {\sep}
 \sepnode{r_2}{c_1}{q_2} {\sep}
\seppred{\code{zip}}{q_1{,}q_2} } ;
\end{array}
\]
 By initially unfolding
predicate instance \form{\seppred{\code{zip}}{\self{,}r_2}} in the antecedent,
two subgoals are generated as
\savespace\[\savespace
\begin{array}{ll}
\code{E_4}. & \emp {\wedge} {\self{=}\nil {\wedge} r_2{=}\nil }~{\ent}_{\{\code{para}\}}~{\seppred{\code{Q_1}}{\self} {\sep}  \seppred{\code{Q_2}}{r_2}} \\
\code{E_5}. & {{\exists}q_1{,}q_2 {\cdot}~ \sepnode{\self}{c_1}{q_1} {\sep}
 \sepnode{r_2}{c_1}{q_2} {\sep}
\seppred{\code{zip}}{q_1{,}q_2} }~{\ent}_{\{\code{para}\}}~{\seppred{\code{Q_1}}{\self} {\sep}  \seppred{\code{Q_2}}{r_2} }
\end{array}
\]
Our system confirms the
validity of \code{E_4} and outputs a pair of residue and
 set of relational assumptions (\form{\D_{R_4}}, \form{\RA_4}) as:
\form{\RA_4{\equiv}(\emp {\wedge}\self{=}\nil{\imply}\seppred{\code{Q_1}}{\self})
 {\wedge}(\emp {\wedge}r_2{=}\nil{\imply}\seppred{\code{Q_2}}{r_2})},
 \form{\D_{R_4}{\equiv}\emp{\wedge}\self{=}\nil {\wedge} r_2{=}\nil}.
To search a proof for \code{E_5},
 our system first applies lemma \code{para}
over predicate instance \form{\seppred{\code{zip}}{q_1{,}q_2} }
and generates the following entailment
%\savespace
\[%\savespace
 {{\exists}q_1{,}q_2 {\cdot}~ \sepnode{\self}{c_1}{q_1} {\sep}
 \sepnode{r_2}{c_1}{q_2} {\sep}
 {\seppred{\code{Q_1}}{q_1} {\sep}  \seppred{\code{Q_2}}{q_2} }
}~{\ent}_{\{\code{para}\}}~{\seppred{\code{Q_1}}{\self} {\sep}  \seppred{\code{Q_2}}{r_2} }
\]
After that, our system successfully proves the above
 entailment and outputs a pair
(\form{\D_{R_5}}, \form{\RA_5}) as:
 \form{\D_{R_5}{\equiv}\emp{\wedge}\self{\neq}\nil {\wedge} r_2{\neq}\nil},
 \form{\RA_5{\equiv}
({\exists}q_1{\cdot}\sepnode{\self}{c_1}{q_1} {\sep} \seppred{\code{Q_1}}{q_1} {\imply}\seppred{\code{Q_1}}{\self})
 {\wedge}}
\form{({\exists}q_2{\cdot}\sepnode{r_2}{c_1}{q_2} {\sep} \seppred{\code{Q_2}}{q_2} {\imply}\seppred{\code{Q_2}}{r_2})}.
Using the algorithm in \cite{Loc:CAV:2014} to solve the set \form{\RA_4{\wedge}\RA_5},
we obtain definitions of \code{Q_1} and \code{Q_2} as:
\begin{small}\form{\seppred{\code{Q_1}}{\root}{\equiv}\emp {\wedge}\root{=}\nil\vee{\exists}q_1{\cdot}\sepnode{\self}{c_1}{q_1} {\sep} \seppred{\code{Q_1}}{q_1}}\end{small};
\begin{small}\form{\seppred{\code{Q_2}}{r_2}{\equiv}\emp {\wedge}r_2{=}\nil\vee{\exists}q_2{\cdot}\sepnode{r_2}{c_1}{q_2} {\sep} \seppred{\code{Q_2}}{q_2}}\end{small}.


==> ex-syn-lem4-bk.tex <==
We consider \form{a} as  and unfolding predicate
\form{\seppred{\code{ls1}}{a{,}p_1}}


\begin{center}
\begin{small}
\def\defaultHypSeparation{\hskip 5pt}
\def\labelSpacing{1pt}
\AxiomC{$\begin{array}{l}
\form{\seppred{\code{ls2}}{a{,}p_2}{\sep}
 \sepnode{p_2}{\code{c_2}}{3,\nil}~{\ent_{\{l_3\}}}}\\
\form{\seppred{\code{ls1}}{a{,}p_3}{\sep}\sepnode{p_3}{\code{c_2}}{v_1{,}p_4}{\sep}U(\setvars{v_1}){\wedge}v_1{\neq}1}
\end{array}$}
\AxiomC{$\begin{array}{l}
\form{\sepnode{a}{\code{c_2}}{1,a'}{\sep}\seppred{\code{ls1}}{a'{,}p_1} {\sep}\seppred{\code{ls2}}{p_1{,}p_2}{\sep}
 \sepnode{p_2}{\code{c_2}}{3,\nil}} \\
~\form{{\ent_{\{l_3\}}}\seppred{\code{ls1}}{a{,}p_3}{\sep}\sepnode{p_3}{\code{c_2}}{v_1{,}p_4}{\sep}U(\setvars{v}){\wedge}v_1{\neq}1}
\end{array}$}
\LeftLabel{\scriptsize LU}
\BinaryInfC{$\begin{array}{l}
\form{\seppred{\code{ls1}}{a{,}p_1} {\sep}\seppred{\code{ls2}}{p_1{,}p_2}{\sep}
 \sepnode{p_2}{\code{c_2}}{3,\nil}}
\form{{\ent_{\emptyset}}\seppred{\code{ls1}}{a{,}p_3}{\sep}\sepnode{p_3}{\code{c_2}}{v_1{,}p_4}{\sep}U(\setvars{v}){\wedge}v_1{\neq}1}
\end{array}$}
\DisplayProof
\end{small}\end{center}

with \form{\setvars{v}{\equiv}\{a{,}p_1{,}p_2{,}p_3{,}p_4{,}v_1}\},
\form{\setvars{v_1}{\equiv}\{a{,}a{,}p_2{,}p_3{,}p_4{,}v_1}\}.

Base case

\begin{center}
\begin{small}
\def\defaultHypSeparation{\hskip .1in}
\def\labelSpacing{1pt}
\AxiomC{$\begin{array}{l}
\form{ a{=}p_1{\wedge}a{=}p_3{\wedge}p_1{=}p_2{\wedge}p_4{=}\nil{\wedge}v_1{=}3}\\
~\form{{\ent_{\{l_3\}}}U(\setvars{v}){\wedge}v_1{\neq}1
\yields (\RA_1,\emp{\wedge}..)}
\end{array}$}
\LeftLabel{\scriptsize M}
\UnaryInfC{$\begin{array}{l}
\form{ \sepnode{p_2}{\code{c_2}}{3,\nil}{\wedge}a{=}p_1{\wedge}a{=}p_3{\wedge}p_1{=}p_2}\\
~\form{{\ent_{\{l_3\}}}\sepnode{p_3}{\code{c_2}}{v_1{,}p_4}{\sep}U(\setvars{v}){\wedge}v_1{\neq}1}
\end{array}$}

\AxiomC{$\begin{array}{l}
\form{\seppred{\code{ls2}}{p_4{,}p_2}{\sep}
 \sepnode{p_2}{\code{c_2}}{3,\nil}{\wedge}a{=}p_1{\wedge}a{=}p_3{\wedge}}\\
~\form{v_1{=}2~{\ent_{\{l_3\}}}U(\setvars{v}){\wedge}v_1{\neq}1
\yields (\RA_2,\emp{\wedge}..)}
\end{array}$}
\LeftLabel{\scriptsize M}
\UnaryInfC{$\begin{array}{l}
\form{\sepnode{p_1}{\code{c_2}}{2{,}p_1'}{\sep}\seppred{\code{ls2}}{p_1'{,}p_2}{\sep}
 \sepnode{p_2}{\code{c_2}}{3,\nil}{\wedge}}\\
~\form{a{=}p_1{\wedge}a{=}p_3{\ent_{\{l_3\}}}\sepnode{p_3}{\code{c_2}}{v_1{,}p_4}{\sep}U(\setvars{v}){\wedge}v_1{\neq}1}
\end{array}$}
\LeftLabel{\scriptsize LU}
\BinaryInfC{$\begin{array}{l}
\form{\seppred{\code{ls2}}{p_1{,}p_2}{\sep}
 \sepnode{p_2}{\code{c_2}}{3,\nil}{\wedge}a{=}p_1{\wedge}a{=}p_3}
\form{{\ent_{\{l_3\}}}\sepnode{p_3}{\code{c_2}}{v_1{,}p_4}{\sep}U(\setvars{v}){\wedge}v_1{\neq}1}
\end{array}$}
\LeftLabel{\scriptsize RU}
\UnaryInfC{$\begin{array}{l}
\form{\seppred{\code{ls2}}{p_1{,}p_2}{\sep}
 \sepnode{p_2}{\code{c_2}}{3,\nil}{\wedge}a{=}p_1}
\form{{\ent_{\{l_3\}}}\seppred{\code{ls1}}{a{,}p_3}{\sep}\sepnode{p_3}{\code{c_2}}{v_1{,}p_4}{\sep}U(\setvars{v}){\wedge}v_1{\neq}1}
\end{array}$}
\DisplayProof
\end{small}\end{center}

\[
\begin{array}{l}
\form{\RA_1{:}}~ \form{p_4{=}\nil {\wedge} {a{=}p_1} {\wedge}p_1{=}p_2 {\wedge}{a{=}p_3}{\wedge}v_1{=}3}~
 \form{~{\imply}~{U(a{,}p_1{,}p_2{,}p_3{,}p_4{,}v_1)}}\\
\form{\RA_2{:}}~ \form{\seppred{\code{ls2}}{p_4{,}p_2}{\sep}\sepnode{p_2}{\code{c_2}}{3,\nil}{\wedge}
 {a{=}p_1} {\wedge}{a{=}p_3}{\wedge}v_1{=}2}~
 \form{~{\imply}~{U(a{,}p_1{,}p_2{,}p_3{,}p_4{,}v_1)}}
\end{array}
\]

Inductive case
\begin{center}
\begin{small}
\def\defaultHypSeparation{\hskip .1in}
\def\labelSpacing{1pt}
\AxiomC{$\begin{array}{l}
\form{U(\setvars{v'}){\wedge}v_1'{\neq}1{\wedge}p_3'{=}p_3{\wedge}v_1'{=}v_1{\wedge}p_4'{=}p_4}
~\form{{\ent_{\{l_3\}}}~U(\setvars{v}){\wedge}v_1{\neq}1\yields (\RA_3,\emp{\wedge}..)}
\end{array}$}
\LeftLabel{\scriptsize M}
\UnaryInfC{$\begin{array}{l}
\form{\seppred{\code{ls1}}{a'{,}p_3'}{\sep}\sepnode{p_3'}{\code{c_2}}{v_1'{,}p_4'}{\sep}U(\setvars{v'}){\wedge}v_1'{\neq}1} 
~\form{{\ent_{\{l_3\}}}~\seppred{\code{ls1}}{a'{,}p_3}{\sep}\sepnode{p_3}{\code{c_2}}{v_1{,}p_4}{\sep}U(\setvars{v}){\wedge}v_1{\neq}1}
\end{array}$}
\LeftLabel{\scriptsize LAPP}
\UnaryInfC{$\begin{array}{l}
\form{\seppred{\code{ls1}}{a'{,}p_1} {\sep}\seppred{\code{ls2}}{p_1{,}p_2}{\sep}
 \sepnode{p_2}{\code{c_2}}{3,\nil}} 
~\form{{\ent_{\{l_3\}}}~\seppred{\code{ls1}}{a'{,}p_3}{\sep}\sepnode{p_3}{\code{c_2}}{v_1{,}p_4}{\sep}U(\setvars{v}){\wedge}v_1{\neq}1}
\end{array}$}
\LeftLabel{\scriptsize M}
\UnaryInfC{$\begin{array}{l}
\form{\sepnode{a}{\code{c_2}}{1,a'}{\sep}\seppred{\code{ls1}}{a'{,}p_1} {\sep}\seppred{\code{ls2}}{p_1{,}p_2}{\sep}
 \sepnode{p_2}{\code{c_2}}{3,\nil}} \\
~~\quad\form{{\ent_{\{l_3\}}}\sepnode{a}{\code{c_2}}{1,a'}{\sep}\seppred{\code{ls1}}{a'{,}p_3}{\sep}\sepnode{p_3}{\code{c_2}}{v_1{,}p_4}{\sep}U(\setvars{v}){\wedge}v_1{\neq}1}
\end{array}$}
\LeftLabel{\scriptsize RU}
\UnaryInfC{$\begin{array}{l}
\form{\sepnode{a}{\code{c_2}}{1,a'}{\sep}\seppred{\code{ls1}}{a'{,}p_1} {\sep}\seppred{\code{ls2}}{p_1{,}p_2}{\sep}
 \sepnode{p_2}{\code{c_2}}{3,\nil}} \\
~~\quad\form{{\ent_{\{l_3\}}}\seppred{\code{ls1}}{a{,}p_3}{\sep}\sepnode{p_3}{\code{c_2}}{v_1{,}p_4}{\sep}U(\setvars{v}){\wedge}v_1{\neq}1}
\end{array}$}
\DisplayProof
\end{small}\end{center}

with \form{\setvars{v'}{\equiv}a{,}p_1{,}p_2{,}p_3'{,}p_4'{,}v_1'}.
\[
\begin{array}{l}
\form{\RA_3{:}}~ \form{U(a'{,}p_1{,}p_2{,}p_3{,}p_4{,}v_1){\wedge}v_1{\neq}1}~
 \form{~{\imply}~{U(a{,}p_1{,}p_2{,}p_3{,}p_4{,}v_1)}}\\
\end{array}
\]


==> impl-ent-old.tex <==
\input{impl-table-ent}
We evaluated {\toolname} on the set of entailment checks of
the SMT-COMP 2014 competition in separation logic
\cite{smtcomp:sl:14}.
To stress on the entailment check, we only focused on those benchmarks of UDB\_ent division.
The results are described in Table \ref{tbl:expr:ent}.
Here we
used sll,dll,cll for singly-, doubly-, cyclic-singly-
linked lists; tll for binary tree with parent pointers and
all leaves are linked as a list \cite{Radu:ATVA:2014}; and
nll for nested singly-linked lists.
Those benchmarks were contributed by participants of the competition (Source column).
The benchmarks tested both valid (\#Valid column) and invalid (\#Invalid column) entailment checks.
Unknown results (\#Unknown column) were returned if {\toolname} can not prove
either valid or invalid, or {\toolname} was timeout \footnote{In all those experiments, timeout is 600 seconds.}.
Time (in second) of successful checks are captured in Time(s) column.
The benchmarks evaluated {\toolname} capability on checking entailment and satisfiability (lseg-spaguetti row)
\footnote{Satisfiability check for formula \form{\D} was encoded as \form{\D ~{\ent}~ \false}.},
segment unfolding (lseg-bolognesa, segment dll, segment nll, and segment skip-lists rows),
and
induction proving (cyclist row).
The last row shows that {\toolname} can prove 96.74\% (534/552) of entailment checks.
The unknown results due to (1) limitation of {\toolname} when unfolding segment predicates that
have more than one segment parameters (segment dll);
(2) infinitely unfolding (e.g. cyclist-11 and cyclist-17).
According to the result of the competition on the UDB\_ent division \cite{smtcompres:sl:14},
{\toolname} is promising; compared with all the participated solvers,
{\toolname} can solve more entailment problems with shorter in running time.

\hide{induction proving timeout (11, 17), unknown (08)

dll: timeout (05, 06, 12). unknown (07,08, 10, 11, 13)

nll time out (04)

can prove 96.74\% of entailment checks.}


==> impl-lemsyn.tex <==
\begin{table*}[tb]
 \vspace{-5pt} %%\savespace
%\begin{small}
%\scriptsize
\begin{center}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
\begin{tabular}[t]{|c | c | c| c |}
\hline
No. & Lemma  & {\toolname} & {\cyctool}  \\
%% \multicolumn{3}{|c|}{Singly-linked List}\\
\hline
1 &  & & \\
2      &    &  & \\
3      & &  & \\
4     &  & & \\
5  &  & & \\
6      &  & & \\
\hline
\end{tabular}

\end{center}
\caption{Experimental Results}
\label{tbl:expr}
%\end{small}
\end{table*}


==> impl-old.tex <==
%\subsection{Implementation}
We have implemented the proposed decision procedures
into {\toolname} which based on SLEEK \cite{Nguyen:VMCAI07,Loc:CAV:2014}.
%% To handle induction proving, we have implemented
%% cyclic technique \cite{Brotherston:CADE:11} into S2.
{\toolname} invoke Z3 \cite{TACAS08:Moura} to discharge satisfiability on pure formulas.

%\subsection{Experimental Results}
In the rest of this section,
we evaluate {\toolname} on three sets of benchmarks:
benchmarks on entailment problem of SMT-COMP competition for separation logic;
benchmarks on program verification of heap programs,
and benchmarks on entailment checks focusing on segment unfolding \cite{pldi:PerezR11}.
The experiments were performed on a machine with the Intel i7-960 (3.2GHz)
processor and 16 GB of RAM. Unfolding and lemma application on summary predicate is bounded by 2.

\subsection{Benchmarks on Entailment Checks}\label{impl-table-ent}\input{impl-table-ent}
We evaluated {\toolname} on the set of entailment checks of
the SMT-COMP 2014 competition in separation logic
\cite{smtcomp:sl:14}.
To stress on the entailment check, we only focused on those benchmarks of UDB\_ent division.
The results are described in Table \ref{tbl:expr:ent}.
Here we
used sll,dll,cll for singly-, doubly-, cyclic-singly-
linked lists; tll for binary tree with parent pointers and
all leaves are linked as a list \cite{Radu:ATVA:2014}; and
nll for nested singly-linked lists.
Those benchmarks were contributed by participants of the competition (Source column).
The benchmarks tested both valid (\#Valid column) and invalid (\#Invalid column) entailment checks.
Unknown results (\#Unknown column) were returned if {\toolname} can not prove
either valid or invalid, or {\toolname} was timeout \footnote{In all those experiments, timeout is 600 seconds.}.
Time (in second) of successful checks are captured in Time(s) column.
The benchmarks evaluated {\toolname} capability on checking entailment and satisfiability (lseg-spaguetti row)
\footnote{Satisfiability check for formula \form{\D} was encoded as \form{\D ~{\ent}~ \false}.},
segment unfolding (lseg-bolognesa, segment dll, segment nll, and segment skip-lists rows),
and
induction proving (cyclist row).
The last row shows that {\toolname} can prove 96.74\% (534/552) of entailment checks.
The unknown results due to (1) limitation of {\toolname} when unfolding segment predicates that
have more than one segment parameters (segment dll);
(2) infinitely unfolding (e.g. cyclist-11 and cyclist-17).
According to the result of the competition on the UDB\_ent division \cite{smtcompres:sl:14},
{\toolname} is promising; compared with all the participated solvers,
{\toolname} can solve more entailment problems with shorter in running time.

\hide{induction proving timeout (11, 17), unknown (08)

dll: timeout (05, 06, 12). unknown (07,08, 10, 11, 13)

nll time out (04)

can prove 96.74\% of entailment checks.}

\subsection{Benchmarks on Program Verification} % todo: glib programs % todo: automatically synthesize the lemma to relate sorted list and list.
\input{impl-table-prog}
\noindent{\bf List. } We tested {\toolname} on verifying functional correctness
of  singly-linked list (singly ll),
cyclic-linked list (cyclic ll) and doubly-linked list (dll).
Each program implements basic operations (\#Proc in Table \ref{tbl:expr}) on the data structures, e.g.
create, delete, append, insert, count, and so on.
This set of benchmarks tested how {\toolname} supports verification on data structures combining
of shape and pure properties (e.g. size property on the programs).
The results presented in Table \ref{tbl:expr} show that {\toolname} can support well the verification;
all functional specification was verified successfully within less than 1 second.

\input{impl-table-prog-sort}
\noindent{\bf Sortedness. }  In Table \ref{tbl:expr:sort}, we evaluated our entailment procedure
on the verification of some textbook sort algorithms, e.g. bubble sort (bubble),
insertion sort (insertion), merge sort (merge), quick sort (quick), selection sort (selection).
Those sortedness programs make use of two following shape predicates:
\[
 \begin{array}{l}
\code{data}~ \code{c_{1a}~\{{int ~val;~c_1 ~ next};\}} \text{\textcolor{blue}{\em // data structure declaration}} \\
\code{\seppred{blln}{\self{,}sm{,}bg{,}n}} {\equiv}
\code{\emp} {\wedge} \code{\self{=}\nil} {\wedge} \code{n{=}0 {\wedge} sm{\leq}bg} \\
\quad \vee \code{ \sepnode{\self}{c_{1a}}{d{,}q} {\sep}
\seppred{blln}{q{,}sm{,}bg{,}n{-}1} {\wedge}sm{\leq} d
 {\wedge}d{\leq} bg
}\\
~~ \invtext{:}~\{ ([~], \code { \self{=}\nil  {\wedge} sm{\leq}bg{\wedge} n{=}0 } ),
 ([\self], \code { sm{\leq}bg {\wedge} n{\geq}1 } ) \};
\end{array}
\]

\[ \begin{array}{l}
\code{\seppred{slln}{\self{,}sm{,}bg{,}n}} {\equiv}
\code{\sepnode{\self}{c_{1a}}{sm{,}q\nil}} {\wedge} \code{n{=}0 {\wedge} sm{=}bg} \\
\quad \vee \code{ \sepnode{\self}{c_{1a}}{sm{,}q} {\sep}
\seppred{slln}{q{,}qs{,}bg{,}n{-}1} {\wedge}sm{\leq} qs
 {\wedge}q{\neq} \nil
}\\
~~ \invtext{:}~\{ ([~], \code{ \self{=}\nil  {\wedge} sm{=}bg{\wedge} n{=}1 }),
 ([\self], \code{ sm{\leq}bg {\wedge} n{\geq}1 }) \};
\end{array}
\]

This set of benchmarks show the capability of {\toolname} on handling the combination of
shape, size and sortedness properties.
The results show that {\toolname} can manage well the data structures with
sortedness and size properties.

% todo: automatically synthesize the lemma to relate sorted list and list.

\input{impl-table-prog-tree}
\noindent{\bf Tree. } The last set of benchmark on this subsection
show how complex {\toolname} can handle the combination.
As shown in Table \ref{tbl:expr:tree},  {\toolname} can help to verify programs on
very complicated pure properties, e.g.
balanced trees (avl, avlb), complete tree, heaps, perfect tree, red black tree (rb),
and binary sort tree (bstree).
The shape predicates on trees use the following
data structures:
\[ \begin{array}{l|l}
\code{data}~ \code{c_{2a}~\{{int ~val;~c_{2a} ~ l;~c_{2a} ~ r};\}} &
\code{data}~ \code{c_{2b}~\{{int ~val;~int~color;~c_{2b} ~ l;~c_{2b} ~ r};\}} \\
\code{data}~ \code{c_{3}~\{{c_3 ~n_1;~c_3 ~ n_2;~c_3 ~ n_3};\}} &
\code{data}~ \code{c_{4}~\{{c_4 ~n_1;~c_4 ~ n_2;~c_4 ~ n_3;~c_4 ~ n_4};\}} \\
\end{array}
\]
\subsection{Benchmarks on Segment Predicates}\input{impl-table-seg}
% todo: clone files
As shown in subsection \ref{impl-table-ent}, {\toolname} can handle well
entailment problems with many segment shape predicates rather than only list segment.
In this subsection, we compared {\toolname} with the hard-fixed
solver \code{Asterix} \cite{pldi:PerezR11} in order to study the price of generality in {\toolname}.
\code{Asterix} solver only works with
 two kinds of shape predicates:
 \code{lseg} and \code{next},
syntactically.
We evaluated two solvers on the {\em bolognesa} set of
 synthetic entailment checks generated by authors of \code{Asterix} \cite{pldi:PerezR11}.
This benchmark focuses on unfolding inference in the entailment checks.
While inference rules of \code{Asterix} is hard-wired
for  \code{lseg}, the
$\entrulen{SEG-UNFOLD*}$ inference rules of {\toolname}
is able to work for arbitrary segment shape predicates,
e.g \code{lseg}, skip list segments, nested list segments, tree segments.

The results presented in Table and Chart \ref{tbl:expr:seg} show that
{\toolname} works well for the entailment with small number of variables
and worse than \code{Asterix} if the number of variables is great than 17.
This comes from the fact that  \code{Asterix} makes use of superposition to discharge
(dis)equality constraints and does not support pure domains, thus its performance is
quite consistent.
 {\toolname} supports pure domains and always invoke solvers pure domains to
when the RHS of entailment check is empty. The larger size of variable (and formula) is,
the larger size of pure formula and large number of the invocation are, and longer
the entailment check is.
Overall, the trade-off on performance of {\toolname} is acceptable.

\hide{
\subsection {Exact Invariant vs. Necessary Invariant}

{\bf SAT problem}
S2-exact, S2-o



{\bf Inference}

S2-exact, S2-o and SL-SAT

{\bf program verification}
S2-exact, S2-o

\input{table-impl-3}

\subsection {Fixed Defined Predicates Benchmark}

sat
\cite{pldi:PerezR11}

entailment

\subsection {User-Defined Predicates Benchmark}

sat

UDB\_sat


ent

UDB 

\subsection {Enhancing Program Verification with Lemma Synthesis}

\input{impl-lemsyn}
\input{impl-table-lem}}


==> impl-old2.tex <==
\subsection{Benchmarks on Segment Predicates}\input{impl-table-seg}
% todo: clone files
As shown in subsection \ref{impl-table-ent}, {\toolname} can handle well
entailment problems with many segment shape predicates rather than only list segment.
In this subsection, we compared {\toolname} with the hard-fixed
solver \code{Asterix} \cite{pldi:PerezR11} in order to study the price of generality in {\toolname}.
\code{Asterix} solver only works with
 two kinds of shape predicates:
 \code{lseg} and \code{next},
syntactically.
We evaluated two solvers on the {\em bolognesa} set of
 synthetic entailment checks generated by authors of \code{Asterix} \cite{pldi:PerezR11}.
This benchmark focuses on unfolding inference in the entailment checks.
While inference rules of \code{Asterix} is hard-wired
for  \code{lseg}, the
$\entrulen{SEG-UNFOLD*}$ inference rules of {\toolname}
is able to work for arbitrary segment shape predicates,
e.g \code{lseg}, skip list segments, nested list segments, tree segments.

The results presented in Table and Chart \ref{tbl:expr:seg} show that
{\toolname} works well for the entailment with small number of variables
and worse than \code{Asterix} if the number of variables is great than 17.
This comes from the fact that  \code{Asterix} makes use of superposition to discharge
(dis)equality constraints and does not support pure domains, thus its performance is
quite consistent.
 {\toolname} supports pure domains and always invoke solvers pure domains to
when the RHS of entailment check is empty. The larger size of variable (and formula) is,
the larger size of pure formula and large number of the invocation are, and longer
the entailment check is.
Overall, the trade-off on performance of {\toolname} is acceptable.

\hide{
\subsection {Exact Invariant vs. Necessary Invariant}

{\bf SAT problem}
S2-exact, S2-o



{\bf Inference}

S2-exact, S2-o and SL-SAT

{\bf program verification}
S2-exact, S2-o

\input{table-impl-3}

\subsection {Fixed Defined Predicates Benchmark}

sat
\cite{pldi:PerezR11}

entailment

\subsection {User-Defined Predicates Benchmark}

sat

UDB\_sat


ent

UDB 

\subsection {Enhancing Program Verification with Lemma Synthesis}

\input{impl-lemsyn}
\input{impl-table-lem}}


==> impl-table-ent.tex <==

\begin{table*}[tb]
% \vspace{-5pt} %%\savespace
%\begin{small}
%\scriptsize
\begin{center}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
\begin{tabular}[t]{|c |c | c | c | c|c|}
\hline
 Group & \#Valid & \# Invalid & \# Unknown  & Time(s) & Source \\
\hline
 lseg-bolognesa & 57 & 53  &   0  & 3.96  & \cite{pldi:PerezR11}  \\
 lseg-clones    & 60 & 40  &   0  &  3.67 & \cite{pldi:PerezR11}  \\
 lseg-spaguetti & 55  & 55  &   0  &  3.44 & \cite{pldi:PerezR11}  \\
lseg-smallfoot  &  55 & 27  &   9  &  2.91 & \cite{pldi:PerezR11}  \\
 cyclist & 19 & 0  &   3  &   4.34 & \cite{Brotherston:CADE:11} \\
  append (sll,cll,dll) & 44 &  2 &   0  & 2.99   & \cite{Nguyen:VMCAI07} \\
  tll & 13 & 0  &   0  & 0.95   & \cite{Loc:CAV:2014} \\
lseg (even, odd) & 16 & 6  &   0  &  1.26  & \cite{Nguyen:VMCAI07} \\
segment dll  & 4  & 1  &   8  & 4.63   & \cite{Ce:TR:2014} \\
segment nll & 14 & 5  &   1  &  5.53  & \cite{Ce:TR:2014} \\
segment skip-lists (skip2, skip3) & 7 & 1  &   6  &  15.73  & \cite{Ce:TR:2014} \\
%induction proving (dll,tll, bst) &  33 & 3  &   0  &    & \cite{Radu:ATVA:2014} \\
\hline
Total &  344 & 190  &   18  & 49.41   & \cite{smtcomp:sl:14} \\
\hline
\end{tabular}
\end{center}
\caption{Experimental Results on Entailment Checks}
\label{tbl:expr:ent}
%\end{small}
\end{table*}


==> impl-table-lem.tex <==
\begin{table}[tb]
 \vspace{-5pt} %%\savespace
%\begin{small}
%\scriptsize
\begin{center}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
\begin{tabular}[t]{|c | c | c|}
\hline
 Example & Synthesized Lemmas  & Time  \\
%% \multicolumn{3}{|c|}{Singly-linked List}\\
\hline
 dll-append-tail &  & \\
sll-sum          &  & \\
sll-get-kth      &  & \\
sll-get-last     &  & \\
sll-insert-last  &  & \\
bubble-sort      &  & \\
\hline
\end{tabular}

\end{center}
\caption{Experimental Results}
\label{tbl:expr}
%\end{small}
\end{table}


==> impl-table-prog-sort.tex <==
\begin{table*}[htb]
 %\vspace{-1pt} %%\savespace
%\begin{small}
%\scriptsize
\begin{center}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
\begin{tabular}[t]{|c |l | c  | c|}
\hline
 Example & Data Structures   & Procedures & Time(s)  \\
%% \multicolumn{3}{|c|}{Singly-linked List}\\
\hline
bll      & \code{blln}

 &   \code{insert},  \code{delete}    & 0.13 \\
\hline
bubble      &  \code{blln},  \code{slln},  \code{lln}
 & \code{bsort}, \code{insert} &   0.35    \\
\hline
insertion      & \code{blln},  \code{slln}
 &  \code{isort}, \code{insert} &   0.36    \\
\hline
merge      & \code{blln},  \code{slln} &  \code{count}, \code{split}, \code{msort}, \code{merge},\code{insert}  & 0.60       \\
\hline
quick      & \code{blln},  \code{slln} & \code{partition}, \code{append\_bll}, \code{qsort}  &  0.86     \\
\hline
selection      & \code{blln},  \code{slln} & \code{find\_min}, \code{delete\_min}, \code{ssort} &  0.43     \\
\hline
sorted-ll      &  \code{slln},  \code{lln} &  \code{insert},\code{insert2},\code{delete},\code{get\_tail}, \code{isort} &   0.79    \\
\hline
\end{tabular}

\end{center}
\caption{Experimental Results on Program Verification (sortedness)}
\label{tbl:expr:sort}
%\end{small}
\end{table*}



==> impl-table-prog-tree.tex <==


\begin{table*}[htb]
 %\vspace{-5pt} %%\savespace
%\begin{small}
\scriptsize 
\begin{center}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
\begin{tabular}[t]{|c |l | c  | c|}
\hline
 Example & Data Structures   & \#Proc & Time  \\
%% \multicolumn{3}{|c|}{Singly-linked List}\\
\hline
avl  &
$ \begin{array}{l}
\code{\seppred{avl}{\self{,}n{,}h}} {\equiv}
\code{\emp} {\wedge} \code{\self{=}\nil} {\wedge} \code{n{=}0 {\wedge} h{=}0} \\
\quad \vee~ \code{ \sepnode{\self}{c_{3}}{h{,}l{,}r} {\sep}
\seppred{avln}{l{,}n_l{,}h_l} {\sep}
\seppred{avln}{r{,}n_r{,}h_r} {\wedge}}\\
 \qquad \code{ n{=}1{+}n_l{+}n_r  {\wedge} h_r{\leq} h_l{+}1  {\wedge} h_l{\leq} h_r{+}1 {\wedge} h{=}\code{max}(h_l{,}h_r){+}1
}\\
~~ \invtext{:}~\{ ([], \code{ \self{=}\nil  {\wedge} n{=}0{\wedge} h{=}0 }),
 ( \code{[\self], n{\geq}1 {\wedge} h{\geq}1 } ) \};
\end{array}
$ 
 &  13 &     11.07  \\
\hline
avl-bal %-orig3
     &
$ \begin{array}{l}
\code{\seppred{avlb}{\self{,}n{,}h {,}b}} {\equiv}
\code{\emp} {\wedge} \code{\self{=}\nil} {\wedge} \code{n{=}0 {\wedge} h{=}0 {\wedge} b{=}1 }\\
\quad \vee~ \code{ \sepnode{\self}{c_{3}}{h{,}l{,}r} {\sep}
\seppred{avlb}{l{,}n_l{,}h_l{,}\anon} {\sep} 
\seppred{avlb}{r{,}n_r{,}h_r{,}\anon} {\wedge}} \\
\qquad  \code{ n{=}1{+}n_l{+}n_r  {\wedge} h_r{+}b{=}h_1{+}1 {\wedge}} \\
\qquad  \code{ h_r{\leq} h_l{+}1  {\wedge} h_l{\leq} h_r{+}1 {\wedge} h{=}\code{max}(h_l{,}h_r){+}1
}\\
~~ \invtext{:}~\{ ([~], \code{\self{=}\nil  {\wedge} n{=}0{\wedge} h{=}0 {\wedge} b{=}1}),\\
\qquad \quad ([\self], \code{ n{\geq}1 {\wedge} h{\geq}1 {\wedge} 0{\leq}b{\leq}2 } ) \};
\end{array}
$ 
 & 7 &      9.42   \\
\hline
complete      &
$ \begin{array}{l}
\code{\seppred{ctree}{\self{,}n{,}nm }} {\equiv}
\code{\emp} {\wedge} \code{\self{=}\nil} {\wedge} \code{n{=}0 {\wedge} nm{=}0} \\
\quad \vee~ \code{ \sepnode{\self}{c_{2}}{l{,}r} {\sep}
\seppred{ctree}{l{,}n{-}1{,}nm_l} {\sep}
\seppred{ctree}{r{,}n{-}2{,}nm_r} } \\
\qquad \code{{\wedge}  nm{=}\code{min}(nm_l{,}nm_r){+}1}\\
\quad \vee~ \code{ \sepnode{\self}{c_{2}}{l{,}r} {\sep}
\seppred{ctree}{l{,}n{-}1{,}nm_l} {\sep}
\seppred{ctree}{r{,}n{-}1{,}nm_r}} \\
\qquad \code{ {\wedge} nm{=}\code{min}(nm_l{,}nm_r){+}1}\\
~~ {\scriptsize \invtext{:}~\{ ([~], \code{\self{=}\nil  {\wedge} n{=}0{\wedge} nm{=}0} ),
 ([\self], \code{nm{\geq}1 {\wedge} n{\geq}nm }) \}};
\end{array}
$ 
 &  5 & 1.83      \\
\hline
heaps      &
$ \begin{array}{l}
\code{\seppred{pg}{\self{,}n{,}mx }} {\equiv}
\code{\emp} {\wedge} \code{\self{=}\nil} {\wedge} \code{n{=}0 {\wedge} mx{=}0} \\
\quad \vee \code{ \sepnode{\self}{c_{4a}}{d{,}n_l{,}n_r{,}l{,}r} {\sep}
\seppred{pg}{l{,}n_l{,}mx_l} {\sep}
\seppred{pg}{r{,}n_r{,}mx_r} {\wedge}}
 \code{  d{\geq}0} \\
 \qquad \code{  {\wedge} d{\geq} mx_l {\wedge} d{\geq} mx_r  {\wedge} mx{\geq}d  ~{\wedge}~ n{=}1{+}n_l{+}n_r  {\wedge} 0{\leq}n_1{-}n_2{\leq}1
}\\
~~ \invtext{:}~\{ ([~], \code{\self{=}\nil  {\wedge} n{=}0{\wedge} mx{=}0 }), 
 ([\self], \code{ n{\geq}1 {\wedge} mx{\geq}1  } ) \};
\end{array}
$ 
 &  5  &  3.77     \\
\hline
perfect      &
$ \begin{array}{l}
\code{\seppred{ptree}{\self{,}n }} ~ {\equiv}~
\code{\emp} {\wedge} \code{\self{=}\nil} {\wedge} \code{n{=}0}  \\
\quad \vee \code{ \sepnode{\self}{c_{4}}{\anon{,}\anon{,}l{,}r} {\sep}
\seppred{ptree}{l{,}n{-1}} {\sep}
\seppred{ptree}{r{,}n{-}1}
}\\
~~ \invtext{:}~\{ ([~], \code{\self{=}\nil  {\wedge} n{=}0 }), 
 ([\self], \code{ n{\geq}1 } ) \};
\end{array}
$ 
 &  5 &  0.31     \\
\hline
rb      &
$ \begin{array}{l}
\code{\seppred{rb}{\self{,}n{,}cl{,}bh }} ~{\equiv}~
\code{\emp} {\wedge} \code{\self{=}\nil} {\wedge} \code{n{=}0 {\wedge} bh{=}1 {\wedge} cl{=}0}  \\
\quad \vee \code{ \sepnode{\self}{c_{2b}}{v{,}1{,}l{,}r} {\sep}
\seppred{rb}{l{,}n_l{,}0{,}bh_l} {\sep}
\seppred{rb}{r{,}n_r{,}0{,}bh_r} {\wedge}} \\
\qquad \code{ cl{=}1 {\wedge} n{=}1{+}n_l{+}n_r
{\wedge} bh_l{=}bh {\wedge} bh_r{=}bh }\\
\quad \vee \code{ \sepnode{\self}{c_{2b}}{v{,}0{,}l{,}r} {\sep}
\seppred{rb}{l{,}n_l{,}\anon{,}bh_l} {\sep}
\seppred{rb}{r{,}n_r{,}\anon{,}bh_r}}  {\wedge} \\
\qquad \code{ cl{=}0 {\wedge} n{=}1{+}n_l{+}n_r
{\wedge} bh_l{=}bh_r {\wedge} bh{=}bh_l{+}1
}\\
~~ \invtext{:}~\{ ([~], \code{\self{=}\nil  {\wedge} n{=}0 {\wedge} bh{=}1 {\wedge} cl{=}0}), \\
\quad \qquad ([\self], \code{ n{\geq}1 {\wedge} bh{\geq}1 {\wedge} 0{\leq} cl {\leq}1} ) \};
\end{array}
$ 
 & 19 &   10.83    \\
\hline
bstree      &
$ \begin{array}{l}
\code{\seppred{bst}{\self{,}n{,}d }} ~ {\equiv}~
\code{\emp} {\wedge} \code{\self{=}\nil} {\wedge} \code{n{=}0 {\wedge} d{=}0}  \\
\quad \vee~ \code{ \sepnode{\self}{c_{2a}}{\anon{,}l{,}r} {\sep}
\seppred{bst}{l{,}n_l{,}d_l} {\sep}
\seppred{rb}{r{,}n_r{,}d_r} {\wedge}} \\
\qquad \code{  n{=}1{+}n_l{+}n_r
{\wedge} d{=}1{+}max(d_l{,}d_r)
}\\
~~ \invtext{:}~\{ ([~], \code{\self{=}\nil  {\wedge} n{=}0 {\wedge} d{=}0 }),
 ([\self], \code{ n{\geq}1 {\wedge} d{\geq}1 } ) \};
\end{array}
$ 
 &  6 &  0.79     \\
\hline
\end{tabular}

\end{center}
\caption{Experimental Results on Program Verification (tree)}
\label{tbl:expr:tree}
%\end{small}
\end{table*}


==> impl-table-prog.tex <==
\begin{table*}[htb]
 \vspace{-2pt} %%\savespace
%\begin{small}
%\scriptsize
\begin{center}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
\begin{tabular}[t]{|c |l | c  | c|}
\hline
 Example & Data Structures   & \#Proc & Time(s)  \\
%% \multicolumn{3}{|c|}{Singly-linked List}\\
\hline
singly ll     &
 $ \begin{array}{l}
\code{\seppred{lln}{\self,n}} {\equiv}
\code{\emp} {\wedge} \code{\self{=}\nil} {\wedge} \code{n{=}0} \\
\quad \vee \code{~\exists ~q \cdot \sepnode{\self}{c_1}{q} {\sep}
\seppred{lln}{q{,}n{-}1}}\\
~~ \invtext{:}~\{ ([], \code{\self{=}\nil {\wedge} n{=}0 } ),
 ([\self], \code{ n{\geq}1 } ) \};
\end{array}
$ 
  &   27   & 0.82 \\
%
\hline
cyclic-ll      &
$ \begin{array}{l}
\code{\seppred{clln}{\self,h,n}} {\equiv}
\code{\emp} {\wedge} \code{\self{=}h} {\wedge} \code{n{=}0} \\
\quad \vee \code{~\exists ~q \cdot \sepnode{\self}{c_1}{q} {\sep}
\seppred{lln}{q{,}s{,}n{-}1} {\wedge}\self{\neq} h}\\
~~ \invtext{:}~\{ ([], \code{ \self{=}h {\wedge} n{=}0 } ),
 ([\self], \code{ \self{\neq}h {\wedge} n{\geq}1 }) \};
\end{array}
$ 
  &   6   & 0.52 \\
\hide{\hline
append          &
\hide{$ \begin{array}{l}
\code{\seppred{lln}{\self{,}n}} {\equiv}
\code{\emp} {\wedge} \code{\self{=}\nil} {\wedge} \code{n{=}0} \\
\quad \vee \code{~\exists ~q \cdot \sepnode{\self}{c_1}{q} {\sep}
\seppred{lln}{q{,}n{-}1}}\\
~~ \invtext{:}~\{ ([], \self{=}\nil {\wedge} n{=}0), \\
\qquad \quad ([\self], n{\geq}1) \};\\
\code{\seppred{lsegn}{\self{,}s{,}n}} {\equiv}
\code{\emp} {\wedge} \code{\self{=}s} {\wedge} \code{n{=}0} \\
\quad \vee \code{~\exists ~q \cdot \sepnode{\self}{c_1}{q} {\sep}
\seppred{lsegn}{q{,}s{,}n{-}1} {\wedge}\self{\neq}s}\\
~~ \invtext{:}~\{ ([], \code{ \self{=}s {\wedge} n{=}0 } ),
 ([\self], \code{ n{\geq}1 {\wedge}\self{\neq}s } ) \};\\
\end{array}
$}
$
\begin{array}{l}
\code{lln}, \code{lsegn}\\
\code{\seppred{clist}{\self{,}n}} {\equiv}
\code{~\exists ~q \cdot \sepnode{\self}{c_1}{q} {\sep}
\seppred{lsegn}{q{,}\self{,}n{-}1}} \\
~~ \invtext{:}~\{ ([\self], n{\geq}1 ) \};
\end{array}
$ 
 &        &   \\
}
\hide{
\hline
 append-tail &
$ \begin{array}{l}
\code{\seppred{lltail}{\self{,}tl{,}n}} {\equiv}
\code{\sepnode{\self}{c_1}{\nil} } {\wedge} tl{=}\self {\wedge} \code{n{=}0} \\
\quad \vee \code{ \sepnode{\self}{c_1}{q} {\sep}
\seppred{lltail}{q{,}tl{,}n{-}1} {\wedge}q{\leq} \nil
}\\
~~ \invtext{:}~\{ ([\self],  \code{ tl{=}\self{\wedge} n{=}1 } ),
  ([\self,tl],  \code{ n{>}1 } ) \};
\end{array}
$ 
  &        &   \\
}
\hline
dll      &
$ \begin{array}{l}
\code{\seppred{dll}{\self{,}p{,}n}} {\equiv}
\code{\emp} {\wedge} \self{=}\nil {\wedge} \code{n{=}0} \\
\quad \vee \code{ \sepnode{\self}{c_2}{p{,}q} {\sep}
\seppred{lltail}{q{,}\self{,}n{-}1}
}\\
~~ \invtext{:}~\{ ([], \code{ \self{=}\nil  {\wedge}  n{=}0 } ),
 ([\self],  \code{ n{\geq}1 }) \};
\end{array}
$ 
 & 11 &   0.76    \\
\hline
\end{tabular}

\end{center}
\caption{Experimental Results on Program Verification (lists)}
\label{tbl:expr}
%\end{small}
\end{table*}



==> impl-table-seg.tex <==
\hide{
\begin{tabular}[t]{|c |c | c | c | c|}
\hline
& & &  \multicolumn{2}{|c|}{Time (s)} \\
\hline
 Vars & \code{P_{next}} & \% Valid & \code{Asterix}  & {\toolname}  \\
\hline
 10 & 0.70 & 53 &    1.701  &  1.327  \\
 11 & 0.69 & 53 &    1.912  &  1.526 \\
12  & 0.69 & 53 &    2.081  &  1.743 \\
13  & 0.70 & 53 &    2.252  &  2.018 \\
14  & 0.69 & 53 &    2.505  &  2.293 \\
15  & 0.69 & 52 &    2.651  &   2.548 \\
16  & 0.69 & 49 &    2.885  &   2.844 \\
17  & 0.71 & 53 &    3.076  &  3.229  \\
18  & 0.70 & 49 &    3.340  &  3.606 \\
19  & 0.70 & 53 &    3.580  &  3.885 \\
20  & 0.70 & 49 &    3.911  &  4.341 \\
\hline
total & & & 29.894 & 29.36 \\
\hline
\end{tabular} 
}

\begin{table*}[tb]
% \vspace{-5pt} %%\savespace
%\begin{small}
%\scriptsize
\begin{center}
\caption{Experimental Results on Entailment Checks: Generality Price}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
\begin{tabular}[t]{cc}
\begin{tabular}[t]{|c |c | c | c | c|}
\hline
& & &  \multicolumn{2}{|c|}{Time (s)} \\
\hline
 Vars & \code{P_{next}} & \% Valid & \code{Asterix}  & {\toolname}  \\
\hline
 10 & 0.70 & 53 &    1.701  &  1.327  \\
 11 & 0.69 & 53 &    1.912  &  1.526 \\
12  & 0.69 & 53 &    2.081  &  1.743 \\
13  & 0.70 & 53 &    2.252  &  2.018 \\
14  & 0.69 & 53 &    2.505  &  2.293 \\
15  & 0.69 & 52 &    2.651  &   2.548 \\
\hline
\end{tabular} &
\begin{tabular}[t]{|c |c | c | c | c|}
\hline
& & &  \multicolumn{2}{|c|}{Time (s)} \\
\hline
 Vars & \code{P_{next}} & \% Valid & \code{Asterix}  & {\toolname}  \\
\hline
16  & 0.69 & 49 &    2.885  &   2.844 \\
17  & 0.71 & 53 &    3.076  &  3.229  \\
18  & 0.70 & 49 &    3.340  &  3.606 \\
19  & 0.70 & 53 &    3.580  &  3.885 \\
20  & 0.70 & 49 &    3.911  &  4.341 \\
\hline
total & & & 29.894 & 29.36 \\
\hline
\end{tabular} 
\end{tabular} 
   %% \includegraphics[width=95mm,height=40mm]{expr-seg}
\end{center}
\savespace
\label{tbl:expr:seg}
%\end{small}
\end{table*}


==> impl-veri-old.tex <==

% todo: glib programs % todo: automatically synthesize the lemma to relate sorted list and list.
\input{impl-table-prog}
\noindent{\bf List. } We tested {\toolname} on verifying functional correctness
of  singly-linked list (singly ll),
cyclic-linked list (cyclic ll) and doubly-linked list (dll).
Each program implements basic operations (\#Proc in Table \ref{tbl:expr}) on the data structures, e.g.
create, delete, append, insert, count, and so on.
This set of benchmarks tested how {\toolname} supports verification on data structures combining
of shape and pure properties (e.g. size property on the programs).
The results presented in Table \ref{tbl:expr} show that {\toolname} can support well the verification;
all functional specification was verified successfully within less than 1 second.

\input{impl-table-prog-sort}
\noindent{\bf Sortedness. }  In Table \ref{tbl:expr:sort}, we evaluated our entailment procedure
on the verification of some textbook sort algorithms, e.g. bubble sort (bubble),
insertion sort (insertion), merge sort (merge), quick sort (quick), selection sort (selection).
Those sortedness programs make use of two following shape predicates:
\[
 \begin{array}{l}
\code{data}~ \code{c_{1a}~\{{int ~val;~c_1 ~ next};\}} \text{\textcolor{blue}{\em // data structure declaration}} \\
\code{\seppred{blln}{\self{,}sm{,}bg{,}n}} {\equiv}
\code{\emp} {\wedge} \code{\self{=}\nil} {\wedge} \code{n{=}0 {\wedge} sm{\leq}bg} \\
\quad \vee \code{ \sepnode{\self}{c_{1a}}{d{,}q} {\sep}
\seppred{blln}{q{,}sm{,}bg{,}n{-}1} {\wedge}sm{\leq} d
 {\wedge}d{\leq} bg
}\\
~~ \invtext{:}~\{ ([~], \code { \self{=}\nil  {\wedge} sm{\leq}bg{\wedge} n{=}0 } ),
 ([\self], \code { sm{\leq}bg {\wedge} n{\geq}1 } ) \};
\end{array}
\]

\[ \begin{array}{l}
\code{\seppred{slln}{\self{,}sm{,}bg{,}n}} {\equiv}
\code{\sepnode{\self}{c_{1a}}{sm{,}q\nil}} {\wedge} \code{n{=}0 {\wedge} sm{=}bg} \\
\quad \vee \code{ \sepnode{\self}{c_{1a}}{sm{,}q} {\sep}
\seppred{slln}{q{,}qs{,}bg{,}n{-}1} {\wedge}sm{\leq} qs
 {\wedge}q{\neq} \nil
}\\
~~ \invtext{:}~\{ ([~], \code{ \self{=}\nil  {\wedge} sm{=}bg{\wedge} n{=}1 }),
 ([\self], \code{ sm{\leq}bg {\wedge} n{\geq}1 }) \};
\end{array}
\]

This set of benchmarks show the capability of {\toolname} on handling the combination of
shape, size and sortedness properties.
The results show that {\toolname} can manage well the data structures with
sortedness and size properties.

% todo: automatically synthesize the lemma to relate sorted list and list.

\input{impl-table-prog-tree}
\noindent{\bf Tree. } The last set of benchmark on this subsection
show how complex {\toolname} can handle the combination.
As shown in Table \ref{tbl:expr:tree},  {\toolname} can help to verify programs on
very complicated pure properties, e.g.
balanced trees (avl, avlb), complete tree, heaps, perfect tree, red black tree (rb),
and binary sort tree (bstree).
The shape predicates on trees use the following
data structures:
\[ \begin{array}{l|l}
\code{data}~ \code{c_{2a}~\{{int ~val;~c_{2a} ~ l;~c_{2a} ~ r};\}} &
\code{data}~ \code{c_{2b}~\{{int ~val;~int~color;~c_{2b} ~ l;~c_{2b} ~ r};\}} \\
\code{data}~ \code{c_{3}~\{{c_3 ~n_1;~c_3 ~ n_2;~c_3 ~ n_3};\}} &
\code{data}~ \code{c_{4}~\{{c_4 ~n_1;~c_4 ~ n_2;~c_4 ~ n_3;~c_4 ~ n_4};\}} \\
\end{array}
\]


==> impl-veri.tex <==


\begin{table}[tb]
 \vspace{-5pt} %%\savespace
%\begin{small}
%\scriptsize
\begin{center}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
\begin{tabular}[t]{|c | c | c|}
\hline
 Example & Synthesized Lemmas  & Time  \\
%% \multicolumn{3}{|c|}{Singly-linked List}\\
\hline
 dll-append-tail &  & \\
sll-sum          &  & \\
sll-get-kth      &  & \\
sll-get-last     &  & \\
sll-insert-last  &  & \\
bubble-sort      &  & \\
\hline
\end{tabular}

\end{center}
\caption{Enhanced Program Verification using Lemma Synthesis}
\label{tbl:expr-veri}
%\end{small}
\end{table}


==> infer.tex <==
Computation of predicate invariant on separation logic without structural properties;
 the pure formula restricted to pointer equality/inequality.
was presented in \cite{Brotherston:LISC:14}. In this section, we enhance the algorithm to 
include structural properties; the pure formula includes not only pointer equality/inequality
but numerical and set/bag constraints.

\noindent{\bf Predicate Dependent Graph. }
{Predicate Dependency: }
If definition of predicate \code{P_1} contains a summary predicate of predicate \code{P_2}, we say \code{P_1} depends on \code{P_2}.

Based on the dependency, we can build a cyclic direct graph of predicate dependency,
i.e. if predicate \code{P_1} depends on predicate \code{P_2},
\code{P_2} is lower in the graph.
The set of predicates is classified into groups of mutual recursive predicates.
Predicate invariant is computed in modular and bottom-up manner.

In this section, we present the algorithm to compute invariant of
a group of mutual recursive predicates \code{\mr}, and
a set of predicates \code{\dep} whose invariants are computed already and
 there is at least one predicate in
 \code{\mr} depends on.

loop
\begin{itemize}
\item parameters closure: find closure on parameters. fixpoint
\item inv on each closure: fixpoint for each groups of parameters
\item combine 
\end{itemize}
until all parameters are examined

invariant store
\[
\inv = \PName \rightarrow \overline{\Var} \rightarrow \Pow(\bag ~{\times}~ \pure )
\]

store for dependent predicates
$\inv_{\dep}$

accumulated store: combined of accumulated closures
$\inv_{\mr}^{acc}$

current iteration store
 $\inv_{\mr}^k$

\hide{\subsection{Exact Invariant Inference}
\input{infere}

\subsection{Necessary Invariant Inference}}



==> infere.tex <==
We present a practical way to compute predicate invariant by
 extending the algorithm in \cite{Brotherston:LISC:14}
to pure properties.



\hide{
Over-Approximate Analysis

\begin{verbatim}
ordering: (b1,p1) << (b2,p2) iff b2 \subset b1 and
 norm((b2,p2)) \form{\implies} norm((b1,p1))

\end{verbatim}

\begin{verbatim}

D = Baga * D_eq * D_num


\bot = ([], false, false)
\top = ([all_pointers], true, true)

normal form: closure on baga
given an abstraction \alpha = (\B, \eq, \num). \alpha is in normal form if
 - for_all (v \in \B): \eq ==> v!=\null
 - for_all (v1,v2 \in \B): \eq ==> v1 != v2
 - for_all (v1,v2,v3 \in SV: if \eq ==> v1 = v2 && \eq ==> v2 = v3 then  \eq ==> v1 = v3)

-meet
 (B_1, \pure_1) meet (B_2, \pure_2) =
 (B_1 (\cap) B_2, \pure_1 \meet (/\) \pure_2)

-join
 (B_1, \pure_1) \join (B_2, \pure_2) =
 (B_1 \cap (\cup) B_2, \pure_1 \join (\/) \pure_2)


extract(svs, \h_ptos /\ \pure) ---> (\baga,  \neq_null /\ \eq, \num)

\norm: alpha --> alpha

  \neq_null = /\ (for_all p \in \B: p != null)
  \neq = /\ (for_all p1,p2 \in \B: p1 != p2)
  \eq_1 = \eq /\ \neq_null /\ \neq
  \alpha1 =  (\B, \eq_1, \num)
  \alpha2 = if \reduce(\alpha1) ==> false then \bot else \alpha1
  --------------------------------
  norm(\B, \eq, \num) --> \alpha2


\reduce: alpha --> pure formula

inv-o = over approximation invariant
inv-u = under approximation invariant
==================================================
inv-u(svs, \alpha, f): find subset models of \alpha in svs and satisfies f.
 - svs: visible variables
 - \alpha: upper bound models
 - f: symbolic formula is being computed


extract: ptrs * (ptos * pure) --> alpha

 \baga = extract_ptros(h_ptos)
 \neq_null = abs(h_ptos)
 \eq = \cup (extract_eq(\pure)) \cup (extract_ptros (h_ptos))
 \num = slice(\pure, svs)
--------------------------------------------------------------
\end{verbatim}}


==> intro-old.tex <==

%\noindent{\bf Context}
 Separation logic \cite{Ishtiaq:POPL01,Reynolds:LICS02}
 has been well established in reasoning
 of heap-manipulating programs.
With the spatial conjunction (${\sep}$),
separation logic allows users to precisely and locally
specify facts of disjoint heaps.In particular, a spatial conjunction (i.e. \form{\heap_1 {\sep}\heap_2}) asserts that a given heap
can be %% split 
decomposed into two disjoint regions in which the
formulas, \form{\heap_1} and \form{\heap_2} hold,
respectively and separately for the two regions of memory.
In this work, we constrain our interest in a practical fragment of separation logic
with 
points-to assertions ($\pto$),
user-defined (\ud) predicate instances \code{P(\setvars{v})},
and constraints on pure (non-heap) domains, i.e. integer arithmetic,
bag/set domains.
The point-to predicate $\sepnodeF{x}{c}{f_i:v_i}$
 expresses a concrete heap cell bound with
an allocated data type \code{c}, pointed-to by
the variable \form{x} and linked with
downstream pointers \form{v_i} via the fields \code{f_i}.
The {\ud} predicate instance expresses a abstract heap, set of (unbounded)
 heap cells.

 To support deductive-style program verification,
 a large number of entailment procedures
 has been studied
in the last decade \cite{Berdine:APLAS05,Nguyen:VMCAI07,Madhusudan:POPL:2012,Piskac:CAV:2013,DBLP:conf/cade/IosifRS13}.
The key challenges there have been
 how to support an expressive fragment \cite{Nguyen:VMCAI07},
  automatic frame inference \cite{Berdine:APLAS05},
 backwards abductive analysis \cite{Cristiano:POPL:09},
and induction proving \cite{Brotherston:CADE:11}.

%\locsay{relation of modular analysis and frame rule and scalability}

\paragraph{\bf Expressiveness.} The most expressive fragment
has been supported is the combination of user-defined predicates
and constraints on pure properties \cite{Nguyen:VMCAI07,Madhusudan:POPL:2012,Piskac:CAV:2013}.
The capability of handling combinations shape
 with other decidable first-order theories for reasoning about data is essential
 for proving functional correctness
properties .




%% Our research question is what good decision procedures for separation logic are.

%% We argue that a decision procedure should be powerful and practical.
%% By powerful, we stress on the expressiveness that procedure can support.
%% By practical, we emphasize on
%%  services it can provide,i.e.
%% frame inference, to its users (verification systems).



\paragraph{\bf Frame Inference.}
One of the distinguished features of separation logic is the frame rule \cite{Reynolds:LICS02}.
 The use of frame rule has enabled automated modular verification
 for heap-based programs against
 user-supplied specifications.
Except entailment procedures
in  \cite{Berdine:APLAS05,Nguyen:VMCAI07,Madhusudan:POPL:2012,Piskac:CAV:2013},
other systems (like \cite{Brotherston:CADE:11,DBLP:conf/cade/IosifRS13})
are not clear how to support this feature. Thus,
 it is not easy to adopt
 them in a composionally reasoning system.
%% In a modular verification system,
%% decision procedure is invoked to discharge verification conditions
%% at {\em function calls} and {\em exit points}.
%% At the former points, verification conditions are generated for proving
%% callee's pre-conditions. The frame inference capability helps to
%% determining residual heaps in order for accumulating into post-states of the calls.
%% At the latter points, verification conditions generated for proving post-condition.
%% The frame inference capability helps to detect leak memory errors;
%% if the residual frame of a post-condition proving at any exit point is not empty heap,
%% the program does not release all memory it has allocated.
%% To enhance program verification,
%% a entailment procedure on separation logic should be capable of
%%  inferring residual heap of entailment checks.
%
%% The entailment procedures presented in \cite{Brotherston:CADE:11,Radu:ATVA:2014} could
%%  be considered as powerful.
%% However, they have not supported frame inference yet.% They are not practical, therefore.
%% And thus, it is not efficient to adopt them
%% to a modular verification system.
%% The entailment procedures presented in
%% \cite{Berdine:FMCO05,Nguyen:VMCAI07,Piskac:CAV:2013}
%% are considered as practical.
%% However, they have not supported the highest level
%% of generic. And thus, it is not effective to adopt
%% them to discharge entailment checks involving
%% multiple shape predicates.

\paragraph{\bf Abduction Reasoning.}

\paragraph{\bf Induction Proving.}


\paragraph{\bf Our approach. } In this work, we propose a powerful and practical entailment
procedure that supports the highest level of the generic
on shape predicates and the combination with pure domains.
The procedure is able to prove both valid and
invalid for entailment checks and empowered
with frame inference capability.
The proposed procedure has several interesting features.
First, like \cite{Nguyen:VMCAI07}, it matches up structural heap chains
of LHS and RHS until the heap in RHS is empty.
After that it reduces the remain heap in LHS following
an implication of first-order logic formulas.
While the reduction in \cite{Nguyen:VMCAI07} is over-approximate,
 our reduction, inspired by James et. al. \cite{Brotherston:LISC:14},
is exact; thus invalid entailment checks would be confirmed.
Second, it enhances completeness by proving a set
of inference rules to handle segment shape predicates.
While inference rules in \cite{pldi:PerezR11}
is hard-wired to list segment, our rules are designed
for general segment shape predicates, e.g.
list segment, tree segment, skip lists, nested lists.
Third, it provides induction proving via
a new lemma mechanism. While lemma application in
\cite{Nguyen:CAV08} makes use a semantics approach
(via an entailment check)
to infer a cut in LHS of entailment,
our mechanism makes use a syntactic approach (via rewrite).
While the former one may be more general,
it would limit the lemma mechanism into 
the entailment procedure capability;
As long as an entailment the procedure can not check,
the lemma would fail.
The latter one will separate the lemma mechanism from
the entailment procedure and improve the induction proving.

\hide{
SL provides several distinguished features to facilitate program verification.
For instance, concise and precise predicates to express heaps:
$\pto$ predicate to express a singleton heap, $\sep$ predicate to express two disjoint heaps; allows user to define general inductive predicate \cite{Brotherston:CADE:11,Chin:SCP:12,Qiu:PLDI:2013,Radu:ATVA:2014} for more effective reasoning;
 frame rule \cite{} for modular verification.

Features of a decision procedures for SL
\begin{itemize}
\item support shape predicate? hard-fixed, soft-fixed, user-defined
\item sat and entailment (for verification)
\item frame inference (for verification)
\item abduction: second-order variables \cite{Trinh:APLAS:2013,Loc:CAV:2014}
\end{itemize}

Decision procedure has been well studied in literature \cite{Berdine:FMCO05,pldi:PerezR11,Cook:CONCUR:2011,Piskac:CAV:2013,Chin:SCP:12,Brotherston:CADE:11,Qiu:PLDI:2013,Radu:ATVA:2014}.

For a expressive reasoning, verification on real programs requires a  fragment of separation logic with
general inductive predicates.
Challenging of decision procedure is at the inductive predicates that unbound data and heap.

The majority of decision procedure for separation logic can be classified into two main categories.

To deal with this challenging, two groups:

for fixed-defined predicate: \cite{Berdine:FMCO05,pldi:PerezR11,Cook:CONCUR:2011,Piskac:CAV:2013},

user-defined predicates: \cite{Chin:SCP:12,Brotherston:CADE:11,Qiu:PLDI:2013,Radu:ATVA:2014}


\noindent{\bf What? define key words}


\noindent{\bf How}
\noindent{\bf Significance, Application, Scope}

issues/changelings:

for fixed-defined predicate: \cite{Berdine:FMCO05,pldi:PerezR11,Cook:CONCUR:2011,Piskac:CAV:2013},

user-defined predicates: \cite{Chin:SCP:12,Brotherston:CADE:11,Qiu:PLDI:2013}

Tree automata \cite{Radu:ATVA:2014}: inefficient for verification
}

Our primary contributions are summarized as follows:
\begin{itemize}
\item We propose a entailment procedure
% to check entailment and satisfiability
 for separation logic with
user-defined predicates.
Our procedure supports both valid and invalid proving.
% We propose exact invariant as exact model of the predicates
% to transform separation logic.
% into a decidable first-order logic, thus we reduce the  entailment and satisfiability problems
% of separation logic to first-order logic.
%\item inference of exact and necessary invariants.
%\item To facility performance, we propose necessary invariant mechanism + sufficient analysis.
\item We introduce a set of inference rules on segment
 shape predicates for more complete entailment checks.
\item We present a new lemma mechanism for induction proving.
\item We have implemented the proposal and evaluated it on
sets of benchmarks. %%Our tool supports SMT2 format
\end{itemize}

The remainder of our paper is organized as follows.
Sec. \ref{sec:spec} describes the fragment
of separation logic and definitions on shape predicates.
Sec. \ref{sec:sat} summarizes a procedure
for satisfiability check via a reduction from
separation logic formula to decidable fragment of first-order logic.
The inference rules of the entailment procedure will
be presented in Sec. \ref{sec:ent.exact}.
Sec. \ref{sec.exp} presents the implementation
and evaluation.
Finally, Sec. \ref{sec.related} discusses related work
and concludes the work.


==> intro-old2.tex <==
%\noindent{\bf Context}
 Separation logic (SL) \cite{Ishtiaq:POPL01,Reynolds:LICS02}
 has been well established for reasoning
 about heap-based
 programs.
%% quantifiers are
%% near the heart of all the essential difficulties
%% This language
%% has two characteristic features: it provides 1) a
%% spatial conjunction
%% operator that decom-
%% poses the heap into disjoint regions, each of which can be reasoned about independently
%% (this enables an elegant treatment of pointer aliasing); and 2)
%% inductive spatial predi-
%% cates
%% that describe the shape of unbounded linked data structures such as lists, trees, etc.
%% SL assertions give rise to the so-called
%% frame rule
%% , a Hoare-logic proof rule that enables
%% compositional verification of heap-manipulating programs.
Frame rule in SL enables
  modular (compositional) reasoning
in the presence of the heap
and is essential for scalability \cite{Jacobs:NFM:2011,CAV08:Yang,Cristiano:POPL:09}.
%%  It allows us to reason about
%% the effect a program on {\em local} heap, the portions of heap it accesses, and
%% reuse that specification in any bigger (global) heap.
In the last decade,
%% with
 a large number of proof systems for SL
  have been studied
 \cite{Berdine:APLAS05,Brotherston:CADE:11,Cristiano:POPL:09,DBLP:conf/cade/IosifRS13,Chin:SCP:12,Madhusudan:POPL:2012}. %%,Piskac:CAV:2013
Generally speaking, the key challenges of these systems are
  to support 
bi-abduction (automated frame inference \cite{Berdine:APLAS05,Chin:SCP:12} and
 logical abduction \cite{Cristiano:POPL:09,Loc:CAV:2014,Trinh:APLAS:2013}),
and automated induction proving \cite{Brotherston:CADE:11}
in SL fragments with inductive predicates.
While the use of inductive predicates attains expressive power,
% these systems carry with them two key issues:
%
%{\bf Inductive Reasoning.}
entailment checks of inductive predicates normally require
induction.
For an indirect solution,
existing works employed
lemmas that are consequences of induction.
These lemmas were either hardwired for a set of predefined predicates
(i.e. lists \cite{Berdine:APLAS05}),
%% or user-supplied \cite{Nguyen:CAV08,Distefano:2008:OOPSLA},
or automatically generated (for normalization of shape analysis \cite{Loc:CAV:2014},
or for some predefined classes of predicates \cite{EneaSW:ATVA:15}).
 While these lemma approaches can handle
 induction reasoning for some specific predicates,
they could not support induction in general proofs.
%% For a fragment of lists and trees,
%% Berdine et. al. introduce an
%%  indirect solution with hardwired
%% rules that are consequences of induction \cite{Berdine:APLAS05}.
%% \cite{EneaSW:ATVA:15}
%
 Brotherston et. al. make an important step
towards automating general induction reasoning in SL with cyclic entailment proofs \cite{Brotherston:CADE:11,Brotherston:APLAS:12}.
Recently, authors in \cite{Chu:PLDI:2015} managed induction by a %% cyclic-based
framework with historical proofs.
%%  While these cyclic proof techniques can automatically solve a range
%% of inductive reasoning problems for
%%  user-defined predicates,
As induction step naturally requires exactly matching between current
sequent with induction hypothesis,
 %%  with shape \cite{Brotherston:CADE:11}
 %% or numerical \cite{Brotherston:APLAS:12} property,
%% is not ready-to-use in {\em compositional} verification systems based on separation logic:
  these techniques %% did
%% not consider
could not handle
frame inference. Thus, these proof systems \cite{Brotherston:CADE:11,Chu:PLDI:2015}
provide limited support
 % which facilities %% enables
%% application of
for the frame rule 
as well as {\em modular} verification.
%% in a symbolic execution framework
%% as well as detection of leaked memory errors in a
%%  programming language without garbage collector;
%% it does not support quantifiers and arithmetic operations
%% (which are often required for automated verification on functional correctness and termination); and
%%  it only supports
%% limited {\em user-supplied} lemmas.
%% via cut rule
 %% instead of
%% and is unable to automatically generate
% auxiliary lemmas during proof derivation.

%%  is crucial for
 %% modular reasoning ; %% \cite{Berdine:APLAS05,Chin:SCP:12};
%% Additionally, it does not support quantifiers and arithmetic operations
%% (which are often required for automated verification on functional correctness and termination);
%% and it only supports
%% limited {\em user-supplied} lemmas %% via cut rule
%%  %% instead of
%% and is unable to automatically generate
%% auxiliary lemmas during proof derivation.
%%  \cite{Brotherston:APLAS:12}.

\hide{{\bf Completeness.} Past works %% in SL
introduce decision procedures for SL decidable fragments
including
 hardwired lists \cite{Berdine:APLAS05,Bouajjani:ATVA:2012,Cook:CONCUR:2011,pldi:PerezR11}, or even
user-defined predicates with some syntactic restrictions \cite{DBLP:conf/cade/IosifRS13}.
However, the SL fragment with (arbitrary) user-defined predicates
(and arithmetic constraints) is, in general, undecidable.
Entailment procedures for this general fragment
typically trade off completeness for expressiveness \cite{Brotherston:CADE:11,Chin:SCP:12,Distefano:2008:OOPSLA,Madhusudan:POPL:2012}.
To enhance the completeness of program verification,
there have been efforts of exploring relations between predicates via {\em user-supplied}
 lemmas 
 \cite{Berdine:APLAS05,Brotherston:CADE:11,Brotherston:APLAS:12,Distefano:2008:OOPSLA,Jacobs:NFM:2011,Nguyen:CAV08}.
While such a static approach puts creative control back into the users' hands, it is not fully automatic
and is infeasible to support inductive proofs relying on
auxiliary
lemmas of %% that relate
dynamically synthesized predicates (like those in \cite{Brotherston-Gorogiannis:SAS:14,Loc:CAV:2014}).}

%\noindent{\bf Our approach. }
In this work, we propose an approach to lemma synthesis
%%  which is able to support the
%% reasoning for predicates
%% with several induction properties, e.g. singly-linked list
%%  with size property.
%% Our aim is
%% to enhance
for frame inference %% automation and completeness
of inductive proofs in a SL fragment with user-defined predicates
and Presburger arithmetic.
Our technical starting point is an entailment procedure
 for user-defined predicates (i.e. those procedures
in the spirit of \cite{Chin:SCP:12}).
%combined with second-order bi-abduction \cite{Loc:CAV:2014}.
We then extend %% the capability of
 this proof system with a new mechanism
where lemmas are automatically generated, proven
 and systematically applied.
Finally, we introduce lemma synthesis
 into
%% automated inductive reasoning and
 theorem exploration.

 Lemmas in our system can include
universally quantified guards  %% variables
 and unknown predicates.
We will use the notation \form{\D[\setvars{v}]} to stand for a formula
with free variables \form{\setvars{v}}.
Our lemmas with universal guards
\footnote{
We will refer lemma with universal guard as universal lemma.}
 have the form \form{\forall \setvars{v} \cdot H(\setvars{v}) {\wedge} G(\setvars{v}) \rightarrow B(\setvars{v})}
whereas universal guard \form{G} and body \form{B} may include unknown predicates whose definitions
 need to be inferred.
While guards over universal variables make our mechanism very expressive,
 %% inference of
 unknown predicates enable us to synthesize generic lemmas i.e. those with weak(est) guards
and strong(est) bodies.
The meaning of lemmas is interpreted in classic semantics \cite{Ishtiaq:POPL01} i.e. for the lemma above \form{\forall \setvars{v} \cdot H(\setvars{v}) {\wedge} G(\setvars{v}) \models B(\setvars{v})}; the LHS exactly entails the RHS (with empty heap in residue).
Our lemma proving is based on the principle of cyclic proof \cite{Brotherston:CADE:11,Brotherston:APLAS:12},
and can support induction proving.
 Automatically synthesizing
as well as soundly applying universal lemmas to support
induction proofs is nontrivial.
Given the entailment check
 \form{\exists \setvars{e} {\cdot} \D_a{\wedge}G(\setvars{e})  ~{\ent}~ \D_c}, we would generate the lemma
\code{lemma ~ l_1} \form{\forall \setvars{e} {\cdot} \D_a {\wedge} \code{P}(\setvars{e})  ~ {\rightarrow}~ \D_c}, whereas \code{P}
is a newly-inferred predicate. We then employ the lemma \code{l_1}
to prove the initial check (see Sec. \ref{mov-pure-simp}).

%% Application of those lemmas are soundly reduced to corresponding instantiated lemmas.

%% inductive entailment
%% \begin{enumerate}
%% \item infer existing residue
%% \item infer unknown recursive residue
%% \item infer instantiation of rhs pointers
%% \end {enumerate}

Frame inference has been studied in SL entailment procedures like \cite{Berdine:APLAS05,Chin:SCP:12,Piskac:CAV:2013}. Intuitively, these systems prove
 validity of an entailment \form{\D_a \ent \D_c} by unfolding user-defined predicates, subtracting heap predicates
% and 
% instantiating universal variables in
% the consequent with variables in
%the antecedent.
% These systems
until
 halting at sequents
 with {\em empty} heap (i.e. the \form{\emp} predicate in SL) in the consequent,
 such that \form{\D_{\code{f}} {\ent} \textcolor{blue}{{\emp}}{\wedge}\pure_r} and then,
 conclude the entailment is valid with the frame \form{\D_{\code{f}}}, denoted by \form{\D_{a} {\ent}\D_c \yields \D_{f}}.
 However, these systems did not provide a direct solution for general induction proofs.
%% did not present how to combine such frames in proofs with case splits
%%  (i.e. proofs with unfolding recursive predicates in antecedents).
%% Moreover, supporting frame inference for
%% induction reasoning
% and
% instantiating universal variables
%% which do not appears in antecedents
%%  is challenging.

%% Our core contribution is the capable of inferring
%% heap frame and
%% instantiating
%%  {\em free} (universal) variables in
%% consequent of an inductive entailment check
%% with a novel lemma synthesis mechanism.
%In this paper, 
We tackle the aforementioned challenging
%%with lemma synthesis.
with a new approach to frame inference for inductive entailment proofs.
Our key insight is that the entailment check \form{\D_a {\ent} \D_c {\yields}\D_f}
is semantically
equivalent to the check \form{\D_a {\ent} \D_c {\sep}\D_f {\yields}\emp}.
To infer frame for inductive entailment checks like the former, we will
prove the latter check inductively while inferring frame \form{\D_f} abductively.
Concretely, we assume frame as an unknown predicate \code{U}, construct
the conjecture \form{\code{lemma~l_2{:}}\D_a {\rightarrow} \D_c {\sep} \code{U}}, and
finally inductively prove this lemma and abductively %% .
%% The abduction feature helps to 
infer a definition of the predicate \code{U}.
The benefit of the use of lemma synthesis in our approach is twofold.
First, our proposed approach is easily integrated into existing proof systems
with lemma mechanism i.e. \cite{Nguyen:CAV08,Distefano:2008:OOPSLA}  (see Sec. \ref{mov-frame}).
%%
%%  Given
%% the entailment check
%%  \form{\forall \setvars{v} {\cdot} \D_a(\setvars{t})  {\ent} \D_r(\setvars{w}){\sep}\D_c}
%%  (where \form{\setvars{v}{=}\setvars{t}{\cup}\setvars{w}}), we speculate the 
%% %% following
%% conjecture:
%% \code{lemma ~ l_2} \form{\forall \setvars{v} \cdot \D_l(\setvars{t}) ~ {\rightarrow}~ \D_r(\setvars{w}){\sep} \code{U}(\setvars{v})}
%% %% and \code{lemma ~l_2} \form{\forall \setvars{w} \cdot \D_l(\setvars{w})  ~ {\rightarrow}~ \D_c(\setvars{v}){\sep} \code{U}(\setvars{w})}
%%  whereas
%% %% \form{\D_l} is either a subformula of \form{\D_a} or \form{\D_a}, and
%% %% \code{P},
%% \code{U} is a new unknown predicate.
%% Here the spatial conjunction
%%  \form{\sep} asserts that
%%  \form{\D_r(\setvars{w})} and \form{\D_c} cover
%%  disjoint portions of heap.
%% Definition of %% \code{P} and
%%  \code{U} would be synthesized
%% while proving the conjecture \code{l_2}.
%%
%% and \code{l_2}, respectively.
%% While \code{P} helps to generate lemmas with universal guards over pure properties,
%%  (see Sec. \ref{mov-pure-simp}),
 %% \code{U}
%% helps to infer frames of induction proofs %% with case splits
%% (see Sec. \ref{mov-frame}).
%% Finally,
%% for example, the proven lemma \code{l_2} %% and \code{l_2} 
%% could be applied as
% auxiliary inference rules
% intelligent cuts in a general entailment check %%  to
%% prove the initial entailment check
%% .
%% For example, the lemma \code{l_2} is applied
%as intelligent cuts
%% as follow (see Sec. \ref{mov-frame}): %% (Here, for simplicity, we discarded some substitutions.):
%% \[
%% \renewcommand{\arraystretch}{1.2}
%% \begin{array}[t]{c}
%% \form{ \D_a(\setvars{t})  {\ent} \D_l(\setvars{t})
%% {\yields}\emp{\wedge}\pure_{1}}
%% \quad
%%  \form{ \D_r(\setvars{w}){\sep} \code{U}(\setvars{v}){\wedge}\pure_{1}  {\ent} \D_r(\setvars{w}){\yields} \code{U}(\setvars{w}){\wedge}\pure_{2}}
%% \quad \form{ \code{U}(\setvars{v}){\wedge}\pure_{2}  {\ent} \D_c{\yields}\D_f}
%% \\
%% \hline
%% \form{\forall \setvars{v} \cdot \D_a(\setvars{t})
%%  ~{\ent}~  \D_r(\setvars{w}){\sep}\D_c ~{\yields}~ \D_f}
%% \end{array}
%% \]
%
%% \begin{center}
%% \def\defaultHypSeparation{\hskip 5pt}
%% \def\labelSpacing{1pt}
%% \AxiomC{$\begin{array}{l}
%% \form{\code{lemma ~ l_2{:}} \form{ \D_a  ~ {\rightarrow}~ \D_c{\sep}\code{U}} }
%% \quad
%%  \form{ \code{U}  ~{\ent}~ \D_c'~{\yields}~\D_3}
%% \end{array}$}
%% \LeftLabel{\scriptsize LSYN}\RightLabel{\scriptsize $\FV({\D_c})\cap\FV({\D_c'}){=}\emptyset$}
%% \UnaryInfC{$\begin{array}{l}
%% \form{ \D_a
%%  ~{\ent}~  \D_c{\sep}\D_c' ~{\yields}~ \D_{3}}
%% \end{array}$}
%% \DisplayProof
%% \end{center}
%% $\FV$ returns free variables of a formula. (Proof is derived bottom-up while frame is obtained top-down.);
Second, the synthesized lemmas (i.e. \code{l_3}) are accumulated for reuse in
proof systems.

Our predicate inference mechanism is based on
 the principle of second-order bi-abduction ({\sobd}), for shape domain \cite{Loc:CAV:2014} and for pure (non-shape)
domains \cite{Trinh:APLAS:2013},
which is an extension of bi-abduction \cite{Cristiano:POPL:09} to user-defined predicates.
 A {\sobd} %% second-order bi-abductive
entailment procedure takes two SL formulas \form{\D_{ante}} and \form{\D_{conseq}}
as inputs. It infers missing hypotheses \form{\RA?}
and residual frame \form{\D_{frm}?}. %%  such that:
%% \form{\RA? {\wedge} {\D_{ante}} ~{\models}~ {\D_{conseq}} {\sep} \D_{frm}?}.
%%\locsay{need to define \form{\sep}}.
%% Here the spatial conjunction
%% \form{\sep} asserts that
%% \form{\D_{conseq}} and \form{\D_{frm}?} cover
%% disjoint portions of heap.
\form{\RA?} is a set of Horn clause-based constraints %% relational assumptions
 over unknown
variables of \form{\D_{ante}} and \form{\D_{conseq}}.
 %% Relational assumptions
These constraints
 have the form of logical implication
 i.e. \form{\D_L {\imply} \D_R}.
 The set \form{\RA?} can be solved
to obtain definitions of the unknown predicates by the 
algorithms in \cite{Loc:CAV:2014,Trinh:APLAS:2013}.

In inductive reasoning, theory exploration is a
 technique for automatically generating
 and proving useful lemmas for sets of given functions, constants and datatypes  \cite{Claessen:2013:CADE,Johansson:2011:AR,Roy:2007}.
In our context, theory exploration is meant for discovering
useful lemmas for a set of given user-defined predicates.
In SL, this technique was indeed presented %% manually
\cite{Berdine:APLAS05,EneaSW:ATVA:15}.
%%  To build
%% theorems for SL fragment with lists and trees,
%% Berdine et. al. introduced a fixed set of lemmas which
%% is fundamental for the completeness of the fragment.
Like \cite{EneaSW:ATVA:15} and unlike
\cite{Berdine:APLAS05}, our approach is automation-based. %% ;
 %% we propose to synthesize lemmas for
 %% predicate relation exploration.
Different from these, %% inductive theorem provers \cite{Claessen:2013:CADE,Johansson:2011:AR,Roy:2007},
our technique is capable of generating lemmas with newly-inferred user-defined predicates
 i.e. those that are synthesized while proving the lemmas.
%% as a first step in developing new theory.

%% Discovering auxiliary lemmas needed for an entailment proof can be viewed
%% as intelligently chosen {\em CUT} (generalization) steps.
%% This technique has been studied
%% in inductive theorem provers like IsaPlanner \cite{Ireland:1996} and Zeno \cite{Sonnex:2012:TACAS}.
%% ,
%% and
%% cyclic provers \cite{Brotherston:CADE:11,Brotherston:APLAS:12,Rosu:2012:OOPSLA}.
%% While conjecture (over non-heap domain) suggested by these provers
%% is based on simply replacing subterm in a stuck entailment
%% by a variable,
%% our conjecture (over combination of heap and pure domains) is formed by extracting 
%% LHS and RHS of a stuck entailment that cover the same reachable heaps.
%%
%% While these provers focus only on pure (non-heap) domains, our technique
%% targets a combination of heap and pure domains.
%%
%% Moreover, our lemma proving process not only certifies the validity of the lemma
%% but also %% is able to 
%% infers guards of to-be-generated
%% lemmas %% automatically
%% via second-order bi-abduction.
%%
%% Moreover, our mechanism is empowered with 
%% able to infer guards of to-be-generated lemmas via 
%% second-order bi-abduction
%%
%%{\sobd} for generating generic lemmas. %% including
%%
%% newly-inferred predicates. %% during the course of lemma proving.
%% while certifying the lemmas.
%% Such inference helps to generate lemmas with generic guards.
%%
 %% Such lemmas, in turn,
 %% can be applied into a wider range of entailment proofs.

%% The novelty of the proposed induction reasoning
%%  is the capability of synthesizing lemmas which capture
%% induction reasoning
%%  on those predicates with several induction properties over heap
%% and pure domains; these lemmas are synthesized
%% by inductively reasoning on shape property,
%% %(like cyclic proof \cite{Brotherston:CADE:11}),
%% and
%%  (induction) pure properties (i.e. size)
%% are abductively analysed via {\sobd}, simultaneously.
%% Although we believe that it is able to extend
%%  cyclic proofs \cite{Brotherston:05,Brotherston:CADE:11,Brotherston:APLAS:12} to
%% directly reason on a fragment of predicates with several induction properties,
%%  we are not aware any such formal discussion
%% (including \cite{Chu:PLDI:2015}).

The novelty of our proof system is the lemma synthesis
with predicate inference. %% Without this inference, our lemma mechanism is only expressive
%% as the
%% cyclic proof system \cite{Brotherston:05,Brotherston:CADE:11,Brotherston:APLAS:12}.
%With the inference capability, our system is more
%expressive and applicable.
Our primary contributions are summarized as follows:
\begin{itemize}\savespace
\item We propose a new mechanism %% with second-order bi-abduction 
where %% that can support
 universal lemmas %% variables
are soundly synthesized and systematically applied.
\item We synthesize lemmas to support  inductive proofs together with frame inference and theorem exploration.
\item We have implemented the proposal in an entailment procedure, called {\toolname},
and integrated {\toolname} into a modular verification.
%and enhanced this system with incremental specification inference.
Our experiments on
sophisticated inductive proofs show that our approach is promising for advancing
state-of-the-art in automated verification of heap-manipulating programs.
{\toolname} and benchmarks are available at
{\toollink}.
\end{itemize}

%% The remainder of our paper is organized as follows.
%% Sec. \ref{sec:spec} describes the fragment
%% of separation logic and definitions on shape predicates.
%% Sec. \ref{sec:sat} summarizes a procedure
%% for satisfiability check via a reduction from
%% separation logic formula to decidable fragment of first-order logic.
%% The inference rules of the entailment procedure will
%% be presented in Sec. \ref{sec:ent.exact}.
%% Sec. \ref{sec.exp} presents the implementation
%% and evaluation.
%% Finally, Sec. \ref{sec.related} discusses related work
%% and concludes the work.


==> lem-proving.tex <==
\begin{table*}[tb]
 \vspace{-5pt} %%\savespace
%\begin{small}
%\scriptsize
\begin{center}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
\begin{tabular}[t]{|c | c | c| c |}
\hline
No. & Lemma  & {\toolname} & {\cyctool}  \\
%% \multicolumn{3}{|c|}{Singly-linked List}\\
\hline
1 &  & & \\
2      &    &  & \\
3      & &  & \\
4     &  & & \\
5  &  & & \\
6      &  & & \\
\hline
\end{tabular}

\end{center}
\caption{Experimental Results}
\label{tbl:expr}
%\end{small}
\end{table*}


==> ll-append-bk.tex <==
\subsection{Modular Verification with Incremental Specification Inference}\label{mov.veri}
\input{mov-append}
Like Distefano et. al. \cite{Distefano:2008:OOPSLA},
in order to minimize the burden of
program verification we pursue a compositional verification of programs whose
specifications are partially supplied.
Concretely, the user is only required to provide specifications
 of pre/post conditions
for critical methods whereas
specifications of the rest and loop invariants
are inferred automatically.
This specification inference has been
implemented incrementally for the combined domains such that
 shape-only specifications are inferred first
 and then constraints over pure domains are additionally synthesized.
 In the context of manipulating-programs,
recursive specifications and loop invariants normally relate
to recursive predicates; consequently, compositionally verifying these specifications
  requires
 inductive reasoning. Our proposed approach aims to bring the best support for
such inductive reasoning.

 For illustration, consider the method \code{append}
in Fig. \ref{fig.mov.append} which appends a list pointed by \code{y}
to the end of a list pointed by \code{x}.
 The user provides the predicates \code{lln}, \code{lsegn} above
and
\code{append}'s specification. Our system
uses existing
inference techniques
(like \cite{Brotherston-Gorogiannis:SAS:14,Loc:CAV:2014} for shape
and \cite{Trinh:APLAS:2013} for numerical domains)
 to generate
invariant for
 the \code{while} loop  (of pre/post condition).
Our verification is bottom-up
 (i.e. verifying the \code{while} loop before the method \code{append})
and incremental (i.e. analyzing {\em shape} and then {\em size} property
for the loop invariant inference).
Concretely, to infer shape specification of the loop invariant
the system first generates specification with two unknown shape predicates
as follows: 
%\savespace\[\savespace
 \form{\requires ~ \code{U_{pre}}(x) \quad \ensures ~ \code{U_{post}}(x,x')},
%\]
whereas \form{x'} is the value of \form{x} after the loop.

\noindent Using the {modular} shape analysis in \cite{Loc:CAV:2014},
%% definitions of
the predicate \code{U_{pre}} and \code{U_{post}} are synthesized as
\savespace\[\savespace
\begin{array}{ll}
 \seppred{\code{U_{pre}}}{\self} & {\equiv}~ \exists q{\cdot}\sepnode{\code{\self}}{c_1}{q} {\sep} 
 \seppred{\code{U_{1}}}{q} \\
\form{\seppred{\code{U_{post}}}{\self{,}l}} & \equiv~
\form{\sepnode{\code{\self}}{c_1}{\nil}} {\wedge} \form{\code{\self}{=}l} ~~ {\vee} \form{~\exists ~q {\cdot}~ \sepnode{\code{\self}}{c_1}{q} {\sep} \seppred{\code{U_{post}}}{q{,}l} {\wedge}\self{\neq}l} \\
\form{\seppred{\code{U_1}}{\self}} & \equiv~
\form{\emp} {\wedge} \form{\code{\self}{=}\nil} ~~ {\vee} \form{~\exists ~q {\cdot}~ \sepnode{\code{\self}}{c_1}{q} {\sep} \seppred{\code{U_1}}{q} }
\end{array}
\]
whereas \code{U_1} is an auxiliary predicate.
Whenever receiving these predicate definitions,
 our theorem exploration
component will generate new lemmas
to study interesting properties of these predicates.
In this example, our system generate the following lemmas
to explicate the separation between two parameters
of the predicate \code{U_{post}}:
\savespace\[\savespace
\begin{array}{l}
 \seppred{\code{lemma~consep~} \code{U_{post}}}{\self{,}l} ~ {\leftrightarrow}~  
 \seppred{\code{U_{2}}}{\self{,}l} {\sep} \sepnode{\code{l}}{c_1}{\nil}\\
\form{\seppred{\code{U_2}}{\self{,}s}} ~ {\equiv}~
\form{\emp} {\wedge} \form{\code{\self}{=}s} ~~ {\vee} \form{~\exists ~q {\cdot}~ \sepnode{\code{\self}}{c_1}{q} {\sep} \seppred{\code{U_2}}{q{,}s} {\wedge}\self{\neq}s}
\end{array}
\]
whereas \form{A{\leftrightarrow}B}, referred as two-way lemma,
 is a short form
of two reverse lemmas: \form{A{\rightarrow}B} and \form{B{\rightarrow}A}.
We then form the shape invariant as follows: 
\savespace\[\savespace \form{\requires ~ \exists q{\cdot}\sepnode{\code{x}}{c_1}{q} {\sep} 
 \seppred{\code{U_{1}}}{q} \quad \ensures ~ \seppred{\code{U_{2}}}{x{,}x'} {\sep} \sepnode{\code{x'}}{c_1}{\nil}}
\]
To extend the above shape invariant with the size property,
we first use predicate extension \cite{Trinh:APLAS:2013}
to automatically
 append the size property into \code{U_1} (\code{Un_1})
 and \code{U_2} (\code{Un_2})\savespace
\[\savespace
\begin{array}{ll}
 \form{\seppred{\code{Un_1}}{\self{,}n}} & \equiv~
\form{\emp} {\wedge} \form{\code{\self}{=}\nil{\wedge}n{=}0} ~~ {\vee} \form{~\exists ~q {\cdot}~ \sepnode{\code{\self}}{c_1}{q} {\sep} \seppred{\code{Un_1}}{q{,}n{-}1} }\\
\form{\seppred{\code{Un_2}}{\self{,}s{,}n}} & \equiv~
\form{\emp} {\wedge} \form{\code{\self}{=}s{\wedge}n{=}0} ~~ {\vee} \form{~\exists ~q {\cdot}~ \sepnode{\code{\self}}{c_1}{q} {\sep} \seppred{\code{Un_2}}{q{,}s{,}n{-}1}{\wedge}\self{\neq}s }
\end{array}
\]
Our theorem exploration, again, generates
two lemmas %%, among other,
 to match \code{Un_1}
with \code{lln} and \code{Un_2} with \code{lsegn}
as: \form{\seppred{\code{Un_1}}{\self{,}n} {\leftrightarrow} \seppred{\code{lln}}{\self{,}n}} and \form{\seppred{\code{Un_2}}{\self{,}s{,}n} {\leftrightarrow} \seppred{\code{lsegn}}{\self{,}s{,}n}}.
After that,
we generate specification with unknown pure predicates \code{P_2}, \code{P_3}:
\savespace\[\savespace
\form{\requires ~ \exists q{\cdot}\sepnode{\code{x}}{c_1}{q} {\sep} 
 \seppred{\code{lln}}{q{,}i}{\wedge}\code{P_2}(i) ~~ {\ensures} ~ \seppred{\code{lsegn}}{x{,}x'{,}j} {\sep} \sepnode{\code{x'}}{c_1}{\nil} {\wedge}\seppred{\code{P_3}}{i{,}j}}
\]
Using {\sobd} for pure properties inference \cite{Trinh:APLAS:2013},
the following definitions are synthesized:
\form{\seppred{\code{P_2}}{i}{\equiv}i{\geq}0}
and \form{\seppred{\code{P_3}}{i{,}j}{\equiv}j{=}i}.
Finally,
loop invariant is inferred as:

\noindent\form{\requires ~ \exists q{\cdot}\sepnode{\code{x}}{c_1}{q} {\sep} 
 \seppred{\code{lln}}{q{,}i}{\wedge}i{\geq}0 \quad \ensures ~ \seppred{\code{lsegn}}{x{,}x'{,}j} {\sep} \sepnode{\code{x'}}{c_1}{\nil} {\wedge}{j{=}i}}.

\noindent This loop invariant is now used in the verification of
 the main method \code{append}.
To verify the correctness and memory safety (no null-dereference and no leakage) of \code{append}, our system generates
 and successfully proves
the following three verification conditions as:
\begin{small}\savespace
\[\savespace
\begin{array}{ll}
\code{VC_1}. & \seppred{\code{lln}}{x{,}n}{\sep}\seppred{\code{lln}}{y{,}m} {\wedge}n{>}0
~{\ent}_{\lemstore}~  {\exists} q{\cdot}\sepnode{\code{x}}{c_1}{q} {\sep} 
 \seppred{\code{lln}}{q{,}i}{\wedge}i{\geq}0 \\
& ~ {\yields}
 (\true,\seppred{\code{lln}}{y{,}m}{\wedge}x{\neq}\nil{\wedge}n{=}i{-}1{\wedge}n{>}0
{\wedge}i{\geq}0) \qquad  \text{// pre-condition (of loop)}\\
\code{VC_2}. & \seppred{\code{lsegn}}{x{,}x'{,}j}{\sep}\sepnode{\code{x'}}{c_1}{\nil} 
{\sep}\seppred{\code{lln}}{y{,}m} {\wedge}{i{=}j} {\wedge}x{\neq}\nil{\wedge}n{=}i{-}1{\wedge}n{>}0 ~{\ent}_{\lemstore}~  \sepnode{\code{x'}}{c_1}{\_}\\
& ~{\yields}
(\true,\seppred{\code{lsegn}}{x{,}x'{,}j}{\sep} \seppred{\code{lln}}{y{,}m} {\wedge}{i{=}j} {\wedge}x{\neq}\nil{\wedge}n{=}i{-}1{\wedge}n{>}0) ~~ \text{// no null-dereference} \\
\code{VC_3}. & \seppred{\code{lsegn}}{\res{,}x'{,}j}{\sep}\sepnode{\code{x'}}{c_1}{y} 
{\sep}\seppred{\code{lln}}{y{,}m} {\wedge}{i{=}j} {\wedge}x{\neq}\nil{\wedge}n{=}i{-}1{\wedge}n{>}0 ~{\ent}_{\lemstore}~ \seppred{\code{lln}}{\res{,}m{+}n} \\
& ~  {\yields}
(\true,\textcolor{blue}{\emp}{\wedge}x{\neq}\nil{\wedge}n{=}i{-}1{\wedge}n{>}0
{\wedge}i{\geq}0) \qquad \qquad  \text{// post-condition, \textcolor{blue}{no leakage}}
\end{array}
\]
\end{small}
whereas \form{\lemstore} is the set of lemmas either supplied by user
or generated by our system (i.e. to explore predicate relations like the \code{conseq} lemmas above).

\noindent We highlight two advantages achieved from our proposed approach.
First, if the two-way lemma \code{consep} was not synthesized,
the condition \code{VC_2} would be generated as: \form{\code{U_{post}}({x{,}x'}){\sep}\seppred{\code{lln}}{y{,}m} {\wedge}{i{=}j} {\wedge}x{\neq}\nil{\wedge}n{=}i{-}1{\wedge}n{>}0 ~{\ent}_{\lemstore}~  \sepnode{\code{x'}}{c_1}{\_}}.
We are not aware any proof systems that are capable of
discharging such obligation and inferring the residual frame, simultaneously.
%%  except cyclic prover \cite{Brotherston:CADE:11}.
%% However, cyclic technique currently does not infer frame;
%%  thus we can not immediately apply
%%  the cyclic prover in a compositional verification.
Second, simultaneously automated proving \code{VC_3} and inferring its residual heap \form{\emp}
(to confirm no memory is leaked)
require nontrivial inductive reasoning which is not supported
by most existing SL entailment procedures.


==> mov-append-bk.tex <==
\begin{figure}
%% \begin{wrapfigure}{l}{0.47\textwidth}\savespace
\begin{center} 
\savespace
\begin{minipage}{0.47\textwidth} \savespace
\begin{frameit} \savespace \savespace \savespace
%% \begin{minipage}[h]{\linewidth}
%%	\lstinputlisting[language=C,label={append}]{./append.c}
\begin{small}\savespace \[
\begin{array}{ll}
1 & \code{struct ~node{\sep}~append(struct ~node{\sep}~x,} \\
  & \quad \quad \quad \qquad \code{struct ~node{\sep}~y)} \\
 & \form{\requires ~ \seppred{\code{lln}}{x{,}n}{\sep}\seppred{\code{lln}}{y{,}m}{\wedge}n{>}0} \\
 & \form{\ensures~ \seppred{\code{lln}}{\res{,}m{+}n}}\\
2&\code{\{ } \\
3 & \code{\quad struct ~node{\sep}x{=}creat\_list(n);}  \\
3 & \code{\quad struct ~node{\sep}y{=}creat\_list(m);}  \\
3 & \code{\quad struct ~node{\sep}tmp{=}x;}  \\
4 & \code{\quad while(tmp{\der}next)~ tmp{=}tmp{\der}next;} \\
%%  & \code{\small //\seppred{\code{lsegn}}{x{,}x'{,}j}{\sep}\sepnode{\code{x'}}{c_1}{\nil} 
%% {\sep}\seppred{\code{lln}}{y{,}m} {\wedge}{i{=}j} {\wedge}x{\neq}\nil{\wedge}n{=}i{-}1{\wedge}n{>}0 } \\
5 & \code{\quad tmp{\der}next{=}y;} \\
6 & \code{\quad return~x};\}
\end{array}
\]\savespace 
\end{small}\savespace 
\end{frameit}
\end{minipage} \savespace
\caption{Code of method \code{append}.}
\label{fig.mov.append}
\end{center}\savespace %%\savespace
\end{figure}
%%\end{wrapfigure}


==> mov-assert.tex <==
\begin{figure}
%% \begin{wrapfigure}{l}{0.47\textwidth}\savespace
\begin{center} 
%\savespace
\begin{minipage}{0.9\textwidth} %\savespace
\begin{frameit}  \savespace \savespace %% \savespace
%% \begin{minipage}[h]{\linewidth}
%%	\lstinputlisting[language=C,label={append}]{./append.c}
\begin{small}\savespace \[
\begin{array}{ll}
1 & \code{void~main(int~n, ~int~ m)\{} \\
2 & \code{~~node{\sep}~x{=} create\_list(n);}\\
3  &  \code{~~node{\sep}~y{=} create\_list(m);}\\
4 & \code{~~ while(x)~}\\
5 & \code{\quad\{ assert ~(x{\der}val{\geq}0);}\\
6 & \code{\quad x{=}x{\der}next \}}; \\
\end{array}
\qquad
\begin{array}{ll}
6 & \code{node{\sep}~create\_list(int~s)\{} \\
7 & \code{~~if(s{\leq}0) ~return~\nil;}\\
8 & \code{~~else~\{}\\
9 & \code{\quad node{\sep}~ p{=}malloc(node); p{\der}val{=}s;}\\
10 & \code{\quad p{\der}next{=}create\_list(s{-}1);} \\
11 & \code{\quad return ~p \}}; \\
\end{array}
\]
\end{small}\savespace 
\end{frameit}
\end{minipage} \savespace
\caption{Illustrative Example.}
\label{fig.mov.assert}
\end{center}\savespace %%\savespace
\end{figure}
%%\end{wrapfigure}
%% Like Distefano et. al. \cite{Distefano:2008:OOPSLA},
In order to minimize the burden of
program verification, we pursue a compositional verification of programs whose
specifications are partially supplied.
Concretely, the user is only required to provide specifications
 of pre/post conditions
for critical methods and loop invariants whereas
specifications of the rest
 are inferred automatically.
%% This specification inference has been
%% implemented incrementally for the combined domains.
%% such that
 %% shape-only specifications are inferred first
 %% and then constraints over pure domains are additionally synthesized .
 In the context of heap-manipulating programs,
recursive specifications and loop invariants normally relate
to recursive predicates; consequently, compositionally verifying these specifications
  requires
 inductive reasoning. Our proposed approach %% aims to
 brings the best support for
such inductive reasoning.

Consider the code fragment
in Fig. \ref{fig.mov.assert}. This program first
 creates a singly-linked list of decreasing values
pointed by \code{x} using the method \code{create\_list}. Then
it iterates through the list by the loop at line 4 and asserts that
the data element of each node of the list is \form{\geq 0}.
We assume that
the method \code{create\_list} (while loop) has been supplied with
the \form{s_1} (\form{s_2}, resp.) specification as:
{\small \form{(s_1){~} \requires ~\emp{\wedge}\true~ \ensures~ \seppred{\code{lld}}{\res,s};}
\form{(s_2){~}\requires ~\seppred{\code{llgZ}}{x}~ \ensures~ \seppred{\code{llgZ}}{x}{\wedge}x'{=}\nil;}}
 whereas the data structure and the predicates \code{lld}, \code{llgZ} are defined as:
\code{struct ~node\{int~val;node{\sep}~next;\}}
\begin{small}
\savespace
 \[\savespace
\begin{array}{lr}
\begin{array}{l}
\form{\defpred~ \seppred{\code{lld}}{\self{,}s}} {\equiv}
\form{\emp} {\wedge} \form{\code{\self}{=}\nil {\wedge} s{\leq}0} \\
~ {\vee} \form{~\exists ~q {\cdot}~ \sepnode{\code{\self}}{\code{node}}{s,q} {\sep}
\seppred{\code{lld}}{q{,}s{-}1} {\wedge} s{>}0};  \\
\end{array}
 ~& ~
\begin{array}{l}
\form{\defpred~\seppred{\code{llgZ}}{\self}} {\equiv}
\form{\emp} {\wedge} \form{\code{\self}{=}\nil } \\
~ {\vee} \form{~\exists ~d{,}q {\cdot}~ \sepnode{\code{\self}}{\code{node}}{d{,}q} {\sep}
\seppred{\code{llgZ}}{q} {\wedge} \form{d{\geq}0}}; \\
\end{array}
\end{array}
\]
\end{small}
As a (bottom-up) modular verification,
the  method \code{create\_list} and the loop are verified prior to
the verification of the method \code{main}; and the correctness of a method
is reduced to the validity of appropriate verification conditions generated.
Our system generates verification conditions to ensure absence of memory
errors (no null dereference, no double free and no memory leak),
 validity of  functional calls/loops via  compositional pre-/post- conditions
 and post-conditions holding.
 For illustrating the proposed induction reasoning,
we focus on the verification condition that was generated before 
the loop at line 4 (to prove that the current context can imply the loop invariant):
\form{(\code{VC_0})~\seppred{\code{lld}}{x',n}{\sep}\seppred{\code{lld}}{y',m} ~{\ent}~ \seppred{\code{llgZ}}{x'}}.
\code{VC_0} involves two different predicates (\code{lld} and \code{llgZ}) over the combined
domains of shape and number. Hence, this entailment is beyond
the capability of most existing verification systems based on separation logic (like \cite{Nguyen:CAV08,Chin:SCP:12,Madhusudan:POPL:2012,Piskac:CAV:2013}).
Our system is able to prove the validity of this entailment (and
infer the residual heap \form{\seppred{\code{lld}}{y',m}}),
by synthesizing the following auxiliary lemma:
 \form{\seppred{\code{lld}}{\self,n} ~{\rightarrow}~ \seppred{\code{llgZ}}{\self}}.

 For more automation, we integrated the proposed
proof system into S2 \cite{Loc:CAV:2014}, a specification inference system.
Simultaneously, we enhanced S2 beyond the shape domain.
With the illustrative example above, the enhanced S2
can verify both its memory safety and the user-supplied assertion at line
5  {\em without} the 
supplied specifications \code{s_1}
and \code{s2}.


==> mov-pure-simp.tex <==

To illustrate the lemma synthesis, consider the following entailment check \code{E_1}
\savespace \[\savespace 
\exists k{\cdot}\seppred{\code{lln}}{x,n} %% {\sep} \seppred{\code{lln}}{y,m}
{\wedge}
n{\geq}k {\wedge}k{\geq}0{\wedge}i{=}k{\wedge}j{=}n{-}k~{\ent}_{\emptyset}~ {\exists} p {\cdot} \seppred{\code{lsegn}}{x{,}p{,}i} {\sep}
\seppred{\code{lln}}{p,j}
\]
%% To the best of our knowledge, automatically proving and frame inferring
%% for the entailment \code{E_1} above are beyond capability of existing proof
%% systems in SL.
We define the \code{lln} (\code{lsegn}) predicate to describe an
 acyclic singly-linked list
\form{\nil}-terminated (segment, respectively) over the data type \code{c_1}
 with size property \code{n} as follows:\savespace
\begin{small}\[\savespace
\begin{array}{lr}
\begin{array}{l}
\form{\defpred~ \seppred{\code{lln}}{\self{,}n}} {\equiv}
\form{\emp} {\wedge} \form{\code{\self}{=}\nil {\wedge} n{=}0} \\
~ {\vee} \form{~\exists ~q {\cdot}~ \sepnode{\code{\self}}{c_1}{q} {\sep}
\seppred{\code{lln}}{q{,}n{-}1} };  \\
 %% \quad \invtext{:}~ (\{~\}, \code{\self{=}s} \wedge \code{n{=}0}) \vee (\{\self\}, \self{\neq}s \wedge \code{n{\geq}1})\\
%% \quad  \invtext~ n{\geq}0;
\end{array}~&~
\begin{array}{l}
\form{\defpred~\seppred{\code{lsegn}}{\self{,}s{,}n}} {\equiv}
\form{\emp} {\wedge} \form{\code{\self}{=}s {\wedge} n{=}0} \\
~ {\vee} \form{~\exists ~q {\cdot}~ \sepnode{\code{\self}}{c_1}{q} {\sep}
\seppred{\code{lsegn}}{q{,}s{,}n{-}1} {\wedge} \form{\self{\neq}s}}; \\
 %% \quad \invtext{:}~ (\{~\}, \code{\self{=}s} \wedge \code{n{=}0}) \vee (\{\self\}, \self{\neq}s \wedge \code{n{\geq}1})\\
%% \quad \invtext~ n{\geq}0;
\end{array}
\end{array}
\]
\end{small}
 whereas
  \form{\code{struct~ c_1\{{c_1{\sep} ~ next};\}}}.
In these predicate definitions, we use basic SL notations
to express heaps, e.g. %% .
%% A heap formula includes
 empty predicate (i.e. \form{\emp}),
points-to predicate (i.e. $\sepnodeF{\self}{c_1}{p}$
  asserts a concrete heap cell bound with
 an allocated data type \code{c_1}, pointed-to by
 the variable \form{\self} and linked with
 downstream pointer \form{p} via the field \code{next}).
%% One important notation of SL is spatial conjunction (${\sep}$).
%% The spatial conjunction
%%  allows users to precisely and locally
%% specify facts of disjoint heaps. In particular,  \form{\heap_1 {\sep}\heap_2}
%%  asserts that a given heap
%% can be %% split 
%% decomposed into two disjoint regions in which the
%% formulas, \form{\heap_1} and \form{\heap_2} hold,
%% respectively and separately for the two regions of memory.


\code{E_1} verifies that the list \form{x} can be split into two smaller list segments.
%% (The list y is the residue.)
We propose to derive a proof for
\code{E_1} through two phrases as follows.
First,
 we automatically generates
the following {\em universal} lemma \code{sp} while proving \code{E_1}:
 \savespace\[\savespace
\code{lemma} ~\code{sp}~ {\forall} n{,}a{,}b {\cdot}
  \seppred{\code{lln}}{\self,n} {\wedge} n{=}a{+}b
{\wedge}n{\geq}b{\wedge}b{\geq}0
\rightarrow
\exists p \cdot \seppred{\code{lsegn}}{\self{,}p{,}a} {\sep}
 \seppred{\code{lln}}{p,b}
\]
(We present the detail of this lemma synthesis in App. \ref{mov-pure}.)

Second, we apply the lemma \code{sp} to prove
\code{E_1} via three steps (see Sec. \ref{ent.lemsyn}): (i) skolemizing \code{E_1};
(ii) generating an instantiation of \code{sp} wrt. the skolemized \code{E_1};
(iii) applying the instantiated lemma into the  skolemized \code{E_1} .


==> pldi15-sound.tex <==
In the experiment section,
authors in \cite{Chu:PLDI:2015} made an effort towards an inductive reasoning for inductive predicates
with both shape and pure properties.
However, it is hard to reproduce proofs
of entailment checks for predicates with several induction properties i.e.,
linked lists with size (len in their term) property.
Concretely, consider the following entailment check
 (the eighth lemma in Table 1 of \cite{Chu:PLDI:2015}):
\form{\seppred{\code{ls1}}{x,y,len_1} {\sep} \seppred{\code{list1}}{y,len_2} \models \seppred{\code{list1}}{x,len_1{+}len_2}}.
 This entailment check requires
inductive proving on both shape and size properties.
The technique presented in \cite{Chu:PLDI:2015} might only perform
an induction reasoning on shape property (using IA-2 in Fig.6) and
did not care induction of size property.  In the following,
we reproduce proofs of the eighth lemma above using proof system presented in \cite{Chu:PLDI:2015}.
(The following proof is similar to the proof in Fig. 11 of \cite{Chu:PLDI:2015}, except
that \form{len_1} and \form{len_2} variables are included.)
%% and assumption A is discarded for simplicity
%
%% \begin{verbatim}
%%                            True
%% (CP) -------------------------------------------------------------------
%%      x!=y,LEN1'=LEN1'+1,L1=t|->y*L3,list1(y,LEN2,L2),L1*L2 
%%            \models list1(t,LEN2,L4),L3*L4=L1*L2
%% (IA-2) ---------------------------------------------------------------------
%%      x!=y,LEN1'=LEN1+1,L1=t|->y*L3,ls1(x,t,LEN1',L3),list1(y,LEN2,L2),L1*L2
%%            \models list1(x,LEN1+LEN2,L),L=L1*L2
%% (LU) ----------------------------------------------------------------------------
%%      ls1(x,y,LEN1,L1)*list1(y,LEN2,L2),L1*L2 \models list1(x,LEN1+LEN2,L),L=L1*L2

%% \end{verbatim}
%
\begin{center}
\begin{small}
\AxiomC{$\code{True}$}
\LeftLabel{CP}\RightLabel{}
\UnaryInfC{$ \begin{array}{l} \{A\} \ent x{\neq}y{,}len_1'{=}len_1'{+}1{,}
L_1{\bumpeq}\sepnode{t}{\code{node}}{y} {\sep} L_3 {,}
 \seppred{\code{list1}}{y,len_2,L_2}{,} \\
  \quad \qquad L_1{\sep}L_2 \models \seppred{\code{list1}}{t,len_2,L_4}, L_3{\sep}L_4{\bumpeq}L_1{\sep}L_2
\end{array} $}
\LeftLabel{IA-2}\RightLabel{}
\UnaryInfC{$ \begin{array}{l} \{A\} \ent x{\neq}y{,}len_1'{=}len_1{+}1{,}
L_1{\bumpeq}\sepnode{t}{\code{node}}{y} {\sep} L_3{,} \seppred{\code{ls1}}{x,t,len_1',L_3} {,}
 \seppred{\code{list1}}{y,len_2,L_2}{,} \\
  \quad \qquad L_1{\sep}L_2 \models \seppred{\code{list1}}{x,len_1{+}len_2,L}, L{\bumpeq}L_1{\sep}L_2
\end{array} $}
\LeftLabel{LU}\RightLabel{}
\UnaryInfC{$\emptyset \ent \seppred{\code{ls1}}{x,y,len_1,L_1} {,} \seppred{\code{list1}}{y,len_2,L_2}
{,}L_1{\sep}L_2 \models \seppred{\code{list1}}{x,len_1{+}len_2,L}, L{\bumpeq}L_1{\sep}L_2$}
\DisplayProof
\end{small}\end{center}
whereas
\[
\begin{array}{l}
\form{A{\equiv}\langle \seppred{\code{ls1}}{x,y,len_1,L_1} {,} \seppred{\code{list1}}{y,len_2,L_2}
{,}L_1{\sep}L_2  \models \seppred{\code{list1}}{x,len_1{+}len_2,L}, \\\qquad L{\bumpeq}L_1{\sep}L_2 ;
\seppred{\code{ls1}}{x,y,len_1}
\rangle }
\end{array}
\]
After (IA-2) rule, the matching between RHS of
the current proof obligation with the RHS of the induction hypothesis
requires $\theta$ to rename y to t and \form{len_1} to \form{len_1'} so that 
\form{\seppred{\code{ls1}}{x,t,len_1'} {\equiv} \seppred{\code{ls1}}{x,y,len_1}\theta}.
 This renaming introduces
the constraint \form{len_1'{=}len_1'{+}1} (which is equivalent to false) in LHS.
This false constraint accidentally terminates the proof.
Such reasoning may produce unsound proofs for inductive predicates
without base cases.
For instance, \cite{Chu:PLDI:2015} may classify the following lemma as validity:

\noindent \form{\seppred{\code{odd\_lsegn}}{x,z,len_1}{\sep} \seppred{\code{odd\_lsegn}}{z,\nil,len_2} \models
\seppred{\code{odd\_lsegn}}{x,\nil,len_1{+}len_2\textcolor{red}{{+}2}}}
whereas \code{odd\_lsegn} and \code{even\_lsegn} are defined as
%
%% \begin{verbatim}
%% pred odd_lsegn<p,size> == self::node<q> * q::even_lsegn<p,size-1>.
%% pred even_lsegn<p,size> == emp/\self=p/\size=0 or self::node<q> * q::odd_lsegn<p,size-1>.
%% \end{verbatim}
%
\[
\begin{array}{l}
\form{\defpred~\seppred{\code{odd\_lsegn}}{\self{,}p{,}len}} ~{\equiv}~
\sepnode{\code{\self}}{\code{node}}{q} {\sep}\seppred{\code{even\_lsegn}}{q{,}p{,}len{-}1} \\
\form{\defpred~\seppred{\code{even\_lsegn}}{\self{,}p{,}len}} ~{\equiv}~
\form{\emp} {\wedge} \form{\code{\self}{=}p {\wedge} len{=}0} \\
\quad \form{\sepnode{\code{\self}}{\code{node}}{q} {\sep}\seppred{\code{odd\_lsegn}}{q{,}p{,}len{-}1}} \\
\end{array}
\]

Therefore, we are not convinced that
the proof system in \cite{Chu:PLDI:2015} is sound 
for reasoning on predicates
with several induction properties over the combined domains.

We believe that it
is straight forward to extend the reasoning in \cite{Chu:PLDI:2015},
 (and cyclic instantiations for separation logic \cite{Brotherston:CADE:11})
to handle some fragment of
predicates including one-inductive properties with pure constraints.
For example, \cite{Chu:PLDI:2015}
(and a simple extension on syntax to cyclic proof \cite{Brotherston:CADE:11}) could handle
such entailment checks like \form{zero\_list(x) \models list(x)},
whereas \form{zero\_list(x)} - list of zero numbers.
For \cite{Chu:PLDI:2015}, handling predicates
with several induction properties over the combined domains
 requires further study.


==> related-old.tex <==

\locsay{fixed Predicates}

There are large number of entailment procedures for separation logic.
We have discussed most of them on Sec. \ref{sec:intro}.
We now highlight some prominent solvers in the literature.
Smallfoot \cite{Berdine:APLAS05} is the first and practical
 entailment procedure for separation logic.
This solver was hard-wired on variants of linked list,
supports frame inference, but induction proving.
Some optimization on segment feature for the same fragment
of \cite{Berdine:APLAS05} was presented
in \cite{Cook:CONCUR:2011} (using graph technique),
 \cite{pldi:PerezR11} (using superposition calculus), and \cite{Navarro:APLAS:2013} (using SMT reduction).
 However, those proposals did not show how
 to infer frame like in \cite{Berdine:APLAS05}
and thus is not practical for modular-based verification
 on heap manipulating programs.
Furthermore, while those solvers fixed their interest
in list segment only, ours can support general segment predicates.
%(and Slayer\cite{Berdine:CAV11}
More general, GRASS-based decision procedures support
all shape predicates that can be reduced to some special
predicates in GRASS logic,
e.g. SLL$\mathds{B}$ for list segment \cite{Piskac:CAV:2013},
GRIT for tree data structures \cite{Piskac:CAV:2014}.
This reduction approach is promising; it can check both
valid and invalid entailment, support frame inference,
abduction and combination of shape and pure properties. However, this approach has not supported
induction proving yet and limited to entailment
checks with level 2 shape predicate, therefore.
Furthermore, to handle the combination of heap and pure domains,
GRASS-based approaches make use of the combination capability of SMT-solvers (i.e. Z3 \cite{TACAS08:Moura}),
{\toolname} employs proof slicing technique \cite{Chanh:ICFEM:2013}.
 As SMT-solver based solution is more modular, it is interesting to exploit this feature
in {\toolname} in future.


\locsay{tree automata} \cite{Enea:APLAS:2014}

\locsay{without pure}



For more expressive predicates, the decision procedures presented
in \cite{Nguyen:VMCAI07,Qiu:PLDI:2013,Radu:ATVA:2014} perform a good try to enhance
the power of separation logic solvers. While solvers presented in \cite{Nguyen:VMCAI07,Qiu:PLDI:2013}
support the combination with pure, they are not complete.
Conversely, solver presented in \cite{Radu:ATVA:2014} considered completeness
but the combination.

\hide{Natural Proofs for Structure, Data, and Separation \cite{Qiu:PLDI:2013}

Automata: Tree automata \cite{Radu:ATVA:2014},
high complexity, hard to support data constraints and frame inference.}

The cyclic prover \cite{Brotherston:CADE:11} described how
to employ induction hypothesis for entailment procedure on separation logic.
This prover can support the most expressive shape predicates among all the tools in
separation logic.
It did support neither the pure constraints show nor frame inference.
Hence, the cyclic technique is not applicable for program verification.

\paragraph{\bf Expressiveness.}

 The expressiveness of a decision procedure
in separation logic relies on (i) the expressiveness of  predicates and
 (ii) combination of
heap and pure (non-hap) domains (like \cite{Nguyen:VMCAI07,Madhusudan:POPL:2012,Qiu:PLDI:2013,Piskac:CAV:2013}).
For the former,
we classifies decision procedures into four levels based on the inductive shape predicates:
\begin{itemize}
\item hard-fixed predicate (level 1): decision procedure
 syntactically hard-wires one kind of shape predicate
i.e. it specializes inference rules for only that kind of predicate.
For example,
 decidable fragment with list segment predicate is
well supported in many separation logic solvers,
 e.g.  \cite{Berdine:APLAS05,pldi:PerezR11,Cook:CONCUR:2011,Navarro:APLAS:2013}.
\item soft-fixed predicates (level 2): decision procedure supports
a set of shape predicates via a intermediate representative, e.g.
 higher-order predicates \cite{Berdine:CAV11} or predicates in reduced logic \cite{Piskac:CAV:2013,Piskac:CAV:2014}.
To check entailment, those decision procedures provide two ingredients:
(i) a reduction from separation logic formulas to the intermediate forms;
and (ii) entailment procedure on the intermediate.
\item user-defined one-predicates (level 3):
 This fragment is proved as undecidable \cite{Cristiano:aplas:01,Timos:FOSSACS:2014}.
 Entailment procedures for this fragment, e.g. \cite{Nguyen:VMCAI07,Qiu:PLDI:2013},
 support general shape predicates,
but allows only one kind of predicate in each entailment check.
\item user-defined predicates (level 4): This fragment is also undecidable
 \cite{Cristiano:aplas:01,Timos:FOSSACS:2014}.
induction proving \cite{Brotherston:CADE:11}
entailment procedure based on automata
and restricted in tree width \cite{Radu:ATVA:2014}.
 %and decision procedure for satisfiability problem \cite{Brotherston:LISC:14}
\end{itemize}

\paragraph{\bf Frame Inference.}

\paragraph{\bf Abduction Inference.}

\cite{Cristiano:POPL:09,Loc:CAV:2014}

\paragraph{\bf Induction Proving.}

\cite{Brotherston:CADE:11,Nguyen:CAV08}

\hide{
SAT \cite{Brotherston:LISC:14}
\begin{verbatim}
 - support user-defined predicates
 - exact invariant
 - sat procedure only
\end{verbatim}

Entailment:


\begin{verbatim}
 - unfold inductive predicates to appropriate abstraction
that combined of shape and pure domains.

\end{verbatim}
}

\hide{ in shape analysis

Relational inductive shape analysis \cite{POPL08:Chang}: introduce a fixed lemma unfolding.

necessary analysis is helpful for \cite{Loc:NFM:2013}.

STRAND \cite{Madhusudan:POPL:2011}: convert constraints on structural heap into data constraints??
}



==> sl-sem-fig.tex <==
Concrete heap models assume  a fixed finite collection {\Dns},
a fixed finite collection {\Flds},
a disjoint set {\Locations} of locations (heap addresses),
a set of non-address values {\Val}, with \form{\nil ~{\in}~ {\Val}}
and {\Val} \form{\cap} {\Locations}  = \form{\emptyset}.
With this, we define:
\[
\begin{array}{lcl}
{\Store}  & {\defsym} &  {\Locations} {\rightharpoonup_{fin}} ({\Dns} ~{\rightarrow}~ \Flds ~{\rightarrow}~ \Val \cup \Locations) \}  \\
{\Stack} & {\defsym} &  {\Var} ~{\rightarrow}~ \Val \cup \Locations
\end{array}
\]

\noindent where \form{dom(f)} returns the domain of function \form{f}.
\form{\emptyheap} is the empty heap that is undefined everywhere.

The semantics is given by a forcing relation:
\form{\sstack,\sheaps ~\force~ \constr}
that forces the stack \form{\sstack} and heap \form{\sheaps} to satisfy the constraint
 \form{\constr}
 where \form{\sheaps \in {\Store} }, \form{\sstack \in {\Stack}},
and \form{\constr} is a separation logic formula.

%% In our system, pure domains include integer domain (\code{Ints}), bag of \form{\Val} ($2^{\code{\Val}}$),
%%  and boolean.
%% The evaluation for pure expressions are determined by valuations as follows:
%% \[
%% \begin{array}{ccc}
%% {\sstack}(\a) ~{\in}~ \code{Ints} & \qquad {\sstack}(\bag) ~{\in}~ 2^{\code{\Val}} & \qquad {\sstack}(\myit{b}) ~{\in}~ \{\true,\false\}
%% \end{array}
%% \]

The semantics is presented as in Figure \ref{fig.sl.sem}.

\begin{figure}[bth]
%\begin{center}
%\begin{minipage}{0.98\textwidth}
%\begin{frameit} %\savespace % \savespace \savespace
\[
\begin{array}{lcl}
 \form{\sstack} \force \pure_1 {\wedge} \pure_2 & \iffs &
 \form{\sstack} \force \pure_1 \text{ and }
 \form{\sstack}\force \pure_2 \\
\form{\sstack} \force \pure_1 {\vee} \pure_2 & \iffs &
 \form{\sstack} \force \pure_1 \text{ or }
 \form{\sstack}\force \pure_2 \\
 \form{\sstack} \force v_1{\oslash}v_2 & \iffs & \force {\sstack}(v_1)~{\oslash}~ {\sstack}(v_2) \text{, where }
 \oslash \in \{=,\neq\}
  \\
 \form{\sstack} \force {\a_1}{\oslash}{\a_2} & \iffs & \force {\sstack}(\a_1)~{\oslash}~ {\sstack}(\a_2) \text{, where }
 \oslash \in \{=,\leq\}
  \\
  \form{\sstack} \force {\bag_1}{\oslash}{\bag_2} & \iffs & \force {\sstack}(\bag_1)~{\oslash}~ {\sstack}(\bag_2) \text{, where }
  \oslash \in \{\in,=,{\bagsubsume},  {\bagunion},{\bagintersect},{\bagsubtract} \}
   \\
 \end{array}
 \]
 \[
 \begin{array}{lcl}
\form{\sstack},\form{\sheaps} \force \emp &
\iffs & \sheaps {=} \emptyset\\
\form{\sstack},\form{\sheaps} \force \sepnodeF{v}{c}{f_i:v_i} &
\iffs &  l {=}\sstack(v), \sheaps {=}\{l \rightarrow r \} 
\mbox{ and } r(c,f_i){=} \sstack({v_i})\\
\form{\sstack},\form{\sheaps} \force \seppredF{\code{P}}{\setvars{v}} &
\iffs & (\form{\sstack(\setvars{v}),}\form{\sheaps}) \in \text{\textlbrackdbl} \seppredF{\code{p}}{\setvars{v}} \text{\textrbrackdbl} \\
      \form{\sstack},\form{\sheaps} \force \seppredF{\code{U}}{\setvars{v}} &
      \iffs & \mbox{always}\\
%\end{array}
%&
%\begin{array}{lcl}
\form{\sstack},\form{\sheaps} \force  \heap_1 \sep \heap_2 &
\iffs & \exists \sheaps_1,\sheaps_2 \cdot \sheaps_1 {\#} \sheaps_2 \mbox{ and }
 \sheaps{=}\sheaps_1 {\cdot} \sheaps_2 \mbox{ and }\\
& & \sstack,\sheaps_1 \force \heap_1 \mbox{ and } \sstack,\sheaps_2 \force \heap_2\\
%%%%%%%%%%%
%% \form{\sstack},\form{\sheaps} \force  \heap_1 \wedge \heap_2 &
%% \iffs & \sstack,\sheaps \force \heap_1 \mbox{ and } \sstack,\sheaps \force \heap_2\\
%%%%%%%%%%%%%%%%
%\end{array}
%% \end{array}
%% \]
%% \[
%% %% \begin{array}{ll};
%% \begin{array}{lcl}
\form{\sstack},\form{\sheaps} \force \true &
\iffs & \mbox{always}\\
\form{\sstack},\form{\sheaps} \force \false &
\iffs & \mbox{never}\\
\form{\sstack},\form{\sheaps} \force \exists {v_1},{...},{v_n} {\cdot}(\heap{\wedge}\pure) &
\iffs & \exists {\alpha_1}...{\alpha_n} \cdot {\sstack}(v_1 \pto {\alpha_1} {\sep} ... {\sep} v_n \pto {\alpha_n}),\form{\sheaps} \force {\heap} \\
 & & \text{ and } {\sstack}(v_1 \pto {\alpha_1} {\sep} ... {\sep} v_n \pto {\alpha_n}) \force {\pure} \\
\form{\sstack},\form{\sheaps} \force \neg \constr &
\iffs & \form{\sstack},\form{\sheaps} \nforce \constr \\
\form{\sstack},\form{\sheaps} \force  \constr_1 \vee \constr_2 &
\iffs & \sstack,\sheaps \force \constr_1 \mbox{ or } \sstack,\sheaps \force \constr_2\\
\end{array}
\]
%\end{frameit}
%\vspace{-15pt}
%\end{minipage}
\caption{Semantics}
\label{fig.sl.sem}
%\end{center}
%%\savespace \savespace
\end{figure}

Note that
%\form{dom(\sheaps)}
 \form{\sheaps_1 {\#} \sheaps_2} denotes that heaps $h_1$ and $h_2$ are disjoint, i.e.
\form{\text{dom}(\sheaps_1) \cap \text{dom}(\sheaps_2) = \emptyset};
  \form{\sheaps_1 \cdot \sheaps_2} denotes the union of two disjoint heaps.

%% As pure formula is independent from heap, semantics of pure formula only depends on stack valuations.
%% Shape predicate is interpreted as least model semantics.
%% its greatest fixpoint set \cite{Brotherston:LISC:14}



\hide{\begin{verbatim}

\eval

\inv^0(lsegn) = \emptyset
\inv^1(lsegn) = \inv^0(lsegn) \vee \eval[(\constr)](\inv^0(lsegn))
               = \emptyset \vee ({(p,p,0,{\emptyheap}) | p \in \val} \vee \emptyset)
                      = {(p,p,0,{\emptyheap}) | p \in \val}
\inv^2(lsegn) = \inv^1(lsegn) \vee \eval[(\constr)]_{\inv^1(lsegn)} = \inv^1 \vee ()
              = {(p,p,0,{\emptyheap}) | p \in \val} \vee
                {(p,p,0,{\emptyheap}) | p \in \val}
                 \vee {(x,p,n,[x->(v,q)]) | x in val, p \in val,
                  n\in val, v,q\in val and x\neq p and n=1 }
\end{verbatim}
}


==> sobd.tex <==
\subsection{Second-Order Bi-Abduction (SOBD)}
Calcagno et. al \cite{Calcagno:2009:POPL}
 presented the {\em bi-abduction} mechanism to empower inference capability in
 a fragment of separation logic with lined-lists.
Authors in \cite{Loc:CAV:2014,Trinh:APLAS:2013} introduced {\em second-order bi-abduction}
to introduce the inference of more general user-defined predicates.
The second-order bi-abductive entailment is formalised as follows
\[
\entailSA{\setvars{P}}{\D_{\code{ante}}}
{\D_{\code{conseq}}} {\RA}{\D_{\code{frame}}}
\]
\form{\D_{\code{ante}}} and \form{\D_{\code{conseq}}} may contains
 second-order variables (unknown predicates) whose definition need to be inferred.
The entailment outputs a pair of a typical residue heaps \form{\D_{\code{frame}}}
and a set of relational constraints (on unknowns) of the form \sm{ \form{\RA {=}
\bigwedge^{n}_{i=1} (\D_l^{i} \imply
\D_r^i})} \footnote{For simplicity, we discard the guard formula.}
such that 
\begin{small}
\form{\RA ~{\wedge}~\D_{\code{ante}}
\vDash \D_{\code{conseq}} {\sep} \D_{
\code{frame}}.
}\end{small}
%% for the validity of the entailment.% is valid when the set has a valid solution;
%% Sematically, the 
 %% a solution is a set of definition of the unknown predicates.
The residual heap \form{\D_{\code{frame}}}
 is inferred during proof search
by looking up proofs with empty heap in the RHS, like \form{\D_{\code{frame}} \ent {\emp}{\wedge}\pure}
 (see \cite{Berdine:APLAS05,Chin:SCP:12}).
The set of constraints \form{\RA} is solved by
derivation algorithms presented
 in \cite{Loc:CAV:2014} (\cite{Trinh:APLAS:2013})
  for shape domain
 (for numeric and bag/set domains, respectively).
We will discuss the use of this {\sobd} technique
 to infer unknown predicates of lemmas in the next section.


==> symmod.tex <==

To interpreter separation logic formula, we propose ${\xpure}$ reduction
from separation logic formula into a first-order logic formula.
This reduced formula captures exactly both constraints on heap structure (size of heap, separation) and
 data.
 The transformation is a composition of  $\reduce$ reduction and $\reduceg$ reduction :
(i) $\reduce$ transforms separation logic formula into a set of
pairs of bag of heap locations and pure formula, referred as {$\baga$} formula,
 an extension of pure formula with bag of heap locations;
(ii) $\reduceg$ transforms {$\baga$} formula into first order logic formula.
\[
\begin{array}[t]{c}
\reduce: \constr \rightarrow \Pow(\bag \sep \pure) \qquad \qquad
\reduceg: \Pow(\bag \sep \pure)  \rightarrow \pure
\end{array}
\]
\[
\begin{array}[t]{c}
  \xpure: {\constr}  \rightarrow \pure \\
  \xpure = \reduceg \circ \reduce
\end{array}
\]

\noindent{\bf $\reduce$ Reduction. }
Formula in $\baga$ domain is a pair ($\bag$,$\pure$):
$\bag$ is a bag of (symbolic) heap locations and ,$\pure$ is a pure formula to express stack constrains.
This domain has the least element ${\bot}$ = $(\{ ~ \},\false)$ and
the greatest element ${\top}$ = $\{ (\Var, \true) \}$.

To define the  $\reduce$ reduction, we will employ the following auxiliary functions:
(1) $\constr \subst{\setvars{t}}{\setvars{v}}$ is a substitution over separation logic formula and
overlapped for the pair of $\baga$ formula (the substitution is defined pointwise over tuples);
(2) \code{\invtext(P,\setvars{v})} returns invariant of a predicate
 formula with substitution  $\subst{\setvars{v}}{\setvars{t}}$
with $\setvars{t}$ is formal parameters of the predicate \code{P}.
(3) disjoint union over two $\baga$ formulas $\uplus$ is defined as


\[ \uplus((\code{b_1}, \pure_1),  (\code{b_2}, \pure_2)) = \left\{
  \begin{array}{l l}
    \bot & \quad \text{if \code{b_1}  {=} \{ \}  \& } \pure_1 {=} \false \\
    \bot & \quad \text{if \code{b_2}  {=} \{ \}  \& } \pure_2 {=} \false \\
    \bot & \quad \text{if $\code{b_1} {\cap} \code{b_2} {\not=} \emptyset$ }\\
    (\code{b_1} {\cup} \code{b_2}, \pure_1 {\wedge} \pure_2) & \quad \text{otherwise}
  \end{array} \right.\]

And disjoint union over two sets of $\baga$ formulas $\biguplus$ is defined as
\[
\begin{array}{l}
\biguplus(\{(\code{b_i}, \pure_i) \mid i \in 1...n \}, 
 \{(\code{b_j}, \pure_j) \mid j \in 1...m\}) {=} \\
 \qquad \quad \{ \uplus ((\code{b_i}, \pure_i),(\code{b_j}, \pure_j))  \mid i \in 1...n
 \text{ \& } j \in 1...m \}
\end{array}
\]

The  $\reduce$ reduction is defined inductively on separation logic formula $\constr$ as follows:
\[
\begin{array}[t]{c}
\reduce(\emp) {=} \{ (\{\}, \true) \}
\end{array}
\qquad 
\begin{array}[t]{c}
\reduce(\sepnodeF{v}{c}{f_i:v_i}) {=} \{ (\{v\}, \true) \}
\end{array}
\]
\[
\begin{array}[t]{c}
\reduce(\seppredF{\code{P}}{\setvars{v}}) {=} \invtext(\code{P}, \code{\setvars{v}})
\end{array}
\quad
%
\begin{array}[t]{c}
\reduce(\heap_1 \sep \heap_2) {=} \reduce(\heap_1) \biguplus \reduce(\heap_2)
\end{array}
\quad
\begin{array}[t]{c}
\reduce(\heap \wedge \pure) {=} \reduce(\heap) \biguplus \{ (\{ \}, \pure) \}
\end{array}
\]
\[
\begin{array}[t]{c}
\reduce(\exists \setvars{v} \cdot \D) {=} \project{\reduce(\D)}{\setvars{v}}
\end{array}
\qquad
\begin{array}[t]{c}
\reduce(\D_1 \vee \D_2) {=} \reduce(\D_1) \cup \reduce(\D_2)
\end{array}
\]

The definition of the project function $\Pi$ is deferred to after the discussion of $\reduceg$ reduction.

\noindent{\bf $\reduceg$ Reduction. } This reduction explicates the constraints on heap:
(i) for each symbolic heap location \form{v}, we add a heap-allocated constraint \form{v{\not=}\nil};
(ii) for each pair of any two each symbolic heap locations \form{v_1} and \form{v_2},
we add a separation constraint \form{v_1{\not=}v_2}.
\[
\begin{array}[t]{c}
\reduceg(\{ \setvars{v} \}, \pure) {=}  \bigwedge \{v_i \neq \nil \mid v_i \in \setvars{v} \} \wedge
 \bigwedge\{v_i \neq v_j \mid v_i,v_j \in \setvars{v} \text{ and } v_i \neq v_j \} \wedge \pure
\end{array}
\]


The project function over a $\baga$ formula \projectp{(\code{b}, \pure)}{\setvars{w}} is defined as
\[
\projectp{(\code{b}, \pure)}{\setvars{w}} {=} (\code{b} {-} \setvars{w}, \elim{\reduceg(\code{b}, \pure)}{\setvars{w}} )
\]
with \code{elim} is a function to eliminate existential quantifiers on pure formulas \cite{Pugh:CACM}.

The project function \form{\Pi} over a set of $\baga$ formulas is extended straight forward.

\noindent{\bf Satisfiability Check. }
Now, the satisfiability check for a separation logic formula ($\sat{\constr}$) is reduced to
satisfiability check of the first-order logic formula ($\satp{\pure}$):
\[
 \sat{\constr}{=}\satp{\xpure(\constr)}
\]

\noindent Technically, the satisfiability on the first-order logic is implemented through two steps.
First, the formula is purified into separate domain-based sub-formulas. (We implemented this step by proof slicing
technique \cite{Chanh:ICFEM:2013}.)
After that, each such sub-formula is discharged by
corresponding SMT-solvers and theorem provers like
 Z3 \cite{TACAS08:Moura}, Omega \cite{Pugh:CACM} for arimethic domain, Mona \cite{klarlund-mona} for bag/set domain.


==> table-impl-3.tex <==
\begin{table}[tb]
% \vspace{-5pt}
\begin{center}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
\begin{tabular}[t]{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Programs & LOC & LOS & \#Proc.& \#Ver. & \#Fault & \code{\mustF} & \code{\mayF^*} & \code{\mayF} & LOE & time(s) \\
\hline
tcas           & 173    & 48   & 9   & 41  & 48  & 31 & 14  & 3  & 3.48  & 3.06 \\
schedule2      & 374    & 108  & 16  & 10  & 10  & 5  &  0  & 3  & 3     & 8.25 \\
%schedule2      & 374    & 108  & 16  & 10  & 8  & 5  &  0  & 3  & 3     & 8.25 \\
schedule1a     & 412    & 50   & 18  & 10  & 16  & 15 &  0  & 1  & 4.38  & 18.13 \\
schedule1b     & 413    & 50   & 18  &  9  & 8   & 7  &  0  & 1  & 4.25  & 32.29  \\
replace       & 564   & 73    & 21  & 24  & 24  & 18 &  0  & 6  & 4.21  & 17.89 \\
%update % of summary of must/may1/may2
print\_tokens2 & 570    & 64   & 19  & 10  & 10  & 7  &  0 &  1  & 4.88  & 20.42 \\
%print\_tokens2 & 570    & 64   & 19  & 10  & 8  & 7  &  0 &  1  & 4.88  & 20.42 \\
print\_tokens  & 726    & 87   & 18  & 7   & 9   & 8  &  0  & 1  & 3.67  & 6.73 \\
\hline
%Total/(Average) & 2668  & 407  & 98  & 87  & 101 & 73 & 14 & 10  & (3.94)\hide{23.65} & (14.81)\hide{272.67} \\
Total/(Average) & 3232  & 480  & 119  & 111  & 125 & 91 & 14 & 16  & (3.98)\hide{23.65} & (15.25)\hide{272.67} \\
%Total/(Average) & 3232  & 480  & 119  & 111  & 121 & 91 & 14 & 16  & (3.98)\hide{23.65} & (15.25)\hide{272.67} \\
\hline
\end{tabular}
%\end{minipage}
%}
\end{center}
\caption{Program Verification: Exact Invariant vs. }
\label{tbl:siemens}
%\vspace{-22pt} %%\savespace
\end{table}


==> ud-seg.tex <==


\noindent{\bf Segment Shape Predicate. } We define segment shape predicate
syntactically through {\em point-to heap chain} as follows.

A formula is a point-to heap chain if it is of the form
\[
\form{\exists \setvars{w} \cdot~ \sepnode{r_1}{c}{\setvars{v}_{2}} {\sep}
 \sepnode{r_2}{c}{\setvars{v}_{3}} {\sep} ... {\sep}
 \sepnode{r_{n-1}}{c}{\setvars{v}_{n}} ~{\wedge}~ \pure}
\] with \form{n\geq2}
and \form{ \pure \implies r_{i+1} \in \setvars{v}_{i}} for all \form{i>1 ~\wedge~ i<n}.

We call \form{r_1} the root pointer and
 \form{\setvars{v_n}} are segment pointers of the chain.
For example, the
\form{\sepnode{v_1}{c_1}{v_2} {\sep} \sepnode{v_2}{c_1}{v_3}} formula
 is a point-to heap chain with root \form{v_1} and segment \form{v_3}.

\begin{defn}[Segment Shape Predicate]
A shape predicate \code{SP} is segment if given a summary predicate
 \form{\seppred{\code{SP}}{\setvars{v}}}
and integer \form{k, ~ k{\geq}1}, all disjuncts of
 \code{\unfoldc^k(\seppred{\code{SP}}{\setvars{v}}, \code{SP}, \setvars{v})}
 are point-to heap chains.
\end{defn}

The predicate parameter corresponds to root (segment pointers)
 of heap chains is called root parameter (segment parameters, respectively).

Without loss of generality, parameters of segment predicates are ordered:
root, segment, and remains.

We fix segment predicate symbols over $\segpred$ ($\segpred \subseteq \PName $).

We now give a definition of heap chain which forms the 
essential of proposed entailment procedure.
\begin{defn}[Heap Chain]
Given the formula \form{\D} as follows:
\[
\exists \setvars{w} \cdot~ \heap_1 {\sep}
 \heap_2 {\sep} ... {\sep} \heap_n ~{\wedge}~ \pure
\] with \form{n\geq2}

\form{\D} is a heap chain if
\begin{enumerate}
\item $\heap_i$ is either a point-to predicate $\sepnode{r_{i-1}}{c}{\setvars{v}_{i}}$
 or a summary predicate $\seppred{\code{SP}}{r_{i-1}{,}\setvars{v_i}}$ with
 $\code{SP} \in \segpred$ for all $1{<}i{<}n$
\item \form{ \pure \implies r_{i+} \in \setvars{v}_{i}} for all \form{1{<}i{<}n}
\end{enumerate}

\form{r_1} is called the root and \form{\setvars{v_n}} are the segment pointers (may be \form{\nil}).
\end{defn}

\noindent For example, the following formula is a heap chain with the root \form{x_0}
and segment \form{\nil}:
\[
\sepnode{x_0}{c_1}{x_1}~{\sep}~ \seppred{\code{lsegn}}{x_1{,}x_2{,}3}~{\sep}
\seppred{\code{lsegn}}{x_2{,}\nil{,}n} 
\]

%% {\bf Predicate Normal Form} parameters
%% \begin{verbatim}
%%  - pure parameters are constrained within every rules
%%  - pointers parameters: segment or allocated in every rules
%% \end{verbatim}

%% \noindent{\bf Implicit Heap Constraints. }
%% Our language does not allows dereference pointers on pure constraints, e.g.
%% \form{x.p\neq \nil}, \form{\seppred{\code{lsegn}}{x,\nil,n} {\wedge} x.p\neq \nil}.
%% This kind of pure constraints implicitly includes constraints on heaps.
%% We require the explicit form, e.g.
%%  \form{\sepnode{x}{c_1}{p} \wedge p\neq \nil},
%%  \form{\seppred{\sepnode{x}{c_1}{p} {\sep} \code{lsegn}}{p,\nil,n_1} {\wedge} p\neq \nil {\wedge} n_1{=}n{-}1}.

